Online Binary Models are Promising for Distinguishing Temporally Consistent Computer Usage Profiles

This paper investigates whether computer usage profiles comprised of process-, network-, mouse-, and keystroke-related events are unique and consistent over time in a naturalistic setting, discussing challenges and opportunities of using such profiles in applications of continuous authentication. We collected ecologically-valid computer usage profiles from 31 MS Windows 10 computer users over 8 weeks and submitted this data to comprehensive machine learning analysis involving a diverse set of online and offline classifiers. We found that: (i) profiles were mostly consistent over the 8-week data collection period, with most (83.9%) repeating computer usage habits on a daily basis; (ii) computer usage profiling has the potential to uniquely characterize computer users (with a maximum F-score of 99.90%); (iii) network-related events were the most relevant features to accurately recognize profiles (95.69% of the top features distinguishing users were network-related); and (iv) binary models were the most well-suited for profile recognition, with better results achieved in the online setting compared to the offline setting (maximum F-score of 99.90% vs. 95.50%).

==> 6-results.tex <==
This section describes the study results testing computer usage profiles uniqueness (\textbf{RQ1}) and temporal consistency (\textbf{RQ2}).

% ===========================
% Profile Uniqueness
% ===========================

%\textbf{Computer Usage Profiles Uniqueness} 
\subsection{Computer Usage Profiles Uniqueness} 

Tables~\ref{tab:acc_multi_sc1} and~\ref{tab:acc_one_sc1} present the F-scores resulted from the multi-class and one-class classifiers, respectively, used to distinguish among the computer usage profiles. %for Scenario 1 (considering all processes). Similarly, Tables~\ref{tab:acc_multi_sc2} and~\ref{tab:acc_one_sc2} report the F-scores for Scenario 2 (considering only common processes). 
Both tables also display the average F-score for each model (computed across conditions) and condition (computed across models). For the one-class results, we reported the average values computed among the individual F-scores obtained per user. The individual results per user are given in Tables \ref{tab:oneclass_per_user_sv} and \ref{tab:oneclass_per_user_if} for the one-class SVM and Isolation Forest, respectively.

%The individual results per user are given in Appendix~\ref{sec:oneclass_per_user}.


%Multi-class classification accuracies in the first experimental scenario
\begin{table}[t]
\caption{Multi-class classification F-scores. %for Scenario 1 (considering all processes used by the users).
}
\label{tab:acc_multi_sc1}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Condition} & \multicolumn{5}{c|}{F-score (\%)} \\ \cline{2-6} 
 & SVM & \begin{tabular}[c]{@{}c@{}}Random\\ Forest\end{tabular} & \begin{tabular}[c]{@{}c@{}}Decision\\ Tree\end{tabular} & LSTM & \begin{tabular}[c]{@{}c@{}}Avg.\end{tabular} \\ \hline
1 week  &83.7&93.9&81.9&77.6&\textbf{84.3} \\ \hline
2 weeks &93.6&86.7&72.7&90.9&\textbf{86.0} \\ \hline
3 weeks &89.1&75.2&70.1&88.1&\textbf{80.6} \\ \hline
\begin{tabular}[c]{@{}c@{}}Avg.\end{tabular} & {\bf 88.8} & {\bf 85.3} & {\bf 74.9} & {\bf 85.5} & - \\ \hline
\end{tabular}
}
% \vspace{-2em}
\end{table}

%One-class classification accuracies in the first experimental scenario
\begin{table}[t]
\caption{One-class classification F-scores. %for Scenario 1 (considering all processes used by the users).
}
\label{tab:acc_one_sc1}
\small
% \resizebox{.75\columnwidth}{!}{
\centering

\begin{tabular}{|c|c|c|c|}
\hline
\multirow{2}{*}{Condition} & \multicolumn{3}{c|}{F-score (\%)} \\ \cline{2-4} 
 & SVM & Isolation Forest & \begin{tabular}[c]{@{}c@{}}Avg.\end{tabular} \\ \hline
1 week & 45.7 & 24.5 & {\bf35.1} \\ \hline
2 weeks & 54.0 & 22.1 & {\bf38.0} \\ \hline
3 weeks & 52.6 & 16.9 & {\bf34.8} \\ \hline
\begin{tabular}[c]{@{}c@{}}Avg.\end{tabular} & {\bf50.8} & {\bf21.2} & - \\ \hline
\end{tabular}
% }
% \vspace{-3em}
\end{table}


\begin{table}[ht]
\caption{Classification F-scores per study participant for one-class SVM.}
\label{tab:oneclass_per_user_sv}
\centering
\footnotesize
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{\multirow{2}{*}{}} & \multicolumn{3}{c|}{F-score (\%)} \\ \cline{2-4} 
\multicolumn{1}{|l|}{} & \begin{tabular}[c]{@{}c@{}}1 week of data\end{tabular} & \begin{tabular}[c]{@{}c@{}}2 weeks of data\end{tabular} & \begin{tabular}[c]{@{}c@{}}3 weeks of data\end{tabular}       \\ \hline
User-01 & 55.6 & 61.2 & 44.3 \\ \hline
User-02 & 37.2 & 27.8 & 33.1 \\ \hline
User-03 & 73.1 & 60.5 & 55.4 \\ \hline
User-04 & 32.3 & 29.4 & 28.5 \\ \hline
User-05 & 37.2 & 45.5 & 34.8 \\ \hline
User-06 & 40.7 & 15.6 & 95.4 \\ \hline
User-07 & 78.2 & 72.3 & 50.9 \\ \hline
User-08 & 84.4 & 73.9 & 86.6 \\ \hline
User-09 & 51.5 & 57.6 & 49.7 \\ \hline
User-10 & 5.7 & 88.6 & 76.1  \\ \hline
User-11 & 36.6 & 67.2 & 74.8 \\ \hline
User-12 & 37 & 63.7 & 41     \\ \hline
User-13 & 47.3 & 68.9 & 65.9 \\ \hline
User-14 & 20.3 & 43 & 43.1   \\ \hline
User-15 & 41.5 & 57.7 & 46.1 \\ \hline
User-16 & 9.4 & 28.2 & 24    \\ \hline
User-17 & 88.5 & 56.8 & 44.4 \\ \hline
Average & 45.7 & 54 & 52.6   \\ \hline

\end{tabular}
\end{table}

\begin{table}[ht]
\caption{Classification F-scores per study participant for Isolation Forest.}
\label{tab:oneclass_per_user_if}
\centering
\footnotesize
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{\multirow{2}{*}{}} & \multicolumn{3}{c|}{F-score (\%)} \\ \cline{2-4} 
\multicolumn{1}{|l|}{} & \begin{tabular}[c]{@{}c@{}}1 week of data\end{tabular} & \begin{tabular}[c]{@{}c@{}}2 weeks of data\end{tabular} & \begin{tabular}[c]{@{}c@{}}3 weeks of data\end{tabular} \\ \hline
User-01 & 39.5 & 20.5 & 19.9 \\ \hline
User-02 & 11.2 & 7.2 & 5.1 \\ \hline
User-03 & 26.9 & 18.9 & 20.6 \\ \hline
User-04 & 12.3 & 14.5 & 15.7 \\ \hline
User-05 & 16.4 & 12.9 & 9.3 \\ \hline
User-06 & 36.7 & 73.2 & 23.5 \\ \hline
User-07 & 13.1 & 9 & 13.2 \\ \hline
User-08 & 26.3 & 19.6 & 20.6 \\ \hline
User-09 & 19.6 & 20.1 & 18.6 \\ \hline
User-10 & 6.5 & 15.5 & 27.8 \\ \hline
User-11 & 19.2 & 16.9 & 17.3 \\ \hline
User-12 & 37.5 & 36.2 & 27.1 \\ \hline
User-13 & 29.1 & 14 & 17.3 \\ \hline
User-14 & 12.2 & 10.3 & 8.2 \\ \hline
User-15 & 16.3 & 16.8 & 16.5 \\ \hline
User-16 & 19.2 & 9.9 & 6.8 \\ \hline
User-17 & 75.1 & 59.7 & 20.7 \\ \hline
Average & 24.5 & 22.1 & 16.9 \\ \hline

\end{tabular}
\end{table}


%Multi-class classification accuracies in the second experimental scenario
% \begin{table}[t]
% \centering
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Condition} & \multicolumn{5}{c|}{F-score (\%)} \\ \cline{2-6} 
%  & SVM & \begin{tabular}[c]{@{}c@{}}Random\\ Forest\end{tabular} & \begin{tabular}[c]{@{}c@{}}Decision\\ Tree\end{tabular} & LSTM & \begin{tabular}[c]{@{}c@{}}Avg.\end{tabular} \\ \hline
% 1 week &18.3&30.1&32.8&27.3&\textbf{27.1} \\ \hline
% 2 weeks &48.4&32.5&25.7&47.8&\textbf{38.6} \\ \hline
% 3 weeks &44.1&27.5&32.2&43.5&\textbf{36.8} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Avg.\end{tabular} & {\bf36.9} & {\bf30.0} & {\bf30.2} & {\bf39.5} & - \\ \hline
% \end{tabular}
% }
% \caption{Multi-class classification F-scores for Scenario 2 (considering only common processes among users).}
% \label{tab:acc_multi_sc2}
% \vspace{-2em}
% \end{table}

% %One-class classification accuracies in the second experimental scenario.
% \begin{table}[t]
% \centering
% \small
% %\resizebox{\columnwidth}{!}{
% \begin{tabular}{|c|c|c|c|}
% \hline
% \multirow{2}{*}{Condition} & \multicolumn{3}{c|}{F-score (\%)} \\ \cline{2-4} 
%  & SVM & Isolation Forest & \begin{tabular}[c]{@{}c@{}}Avg.\end{tabular} \\ \hline
% 1 week & 10.0 & 12.5 & {\bf11.2} \\ \hline
% 2 weeks & 15.2 & 12.8 & {\bf14.0} \\ \hline
% 3 weeks & 14.9 & 12.3 & {\bf13.6} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Avg.\end{tabular} & {\bf13.3} & {\bf12.5} & - \\ \hline
% \end{tabular}
% %}
% \caption{One-class classification F-scores for Scenario 2 (considering only common processes among users).}
% \label{tab:acc_one_sc2}
% \vspace{-3.5em}
% \end{table}

%In terms of classifiers' performance, the highest average accuracy rates were achieved with the multi-class models for Scenario 1 ($M = 86.3\%$, $SD = 4.1\%$), followed by the one-class models also for Scenario 1 ($M = 73.4\%$, $SD = 5.9\%$). Scenario 2 yielded worse results, especially with the multi-class models, with average accuracies lower than 50\% ($M = 39.5\%$, $SD = 1.5\%$). With the one-class models, although above 50\%, the average accuracies did not reach promising levels ($M = 59.1\%$, $SD = 0.3\%$). In addition, in Appendix~\ref{sec:appendix_confmat}, we provide the confusion matrices obtained with the multi-class SVM in both Scenarios (confusion matrices from the other classifiers exhibited qualitatively similar results), which also show that the predictions were consistently more accurate for Scenario 1 compared to Scenario 2. When comparing classification approaches, for Scenario 1, the multi-class models outperformed the one-class models in accuracy by 12.9\% on average (86.3\% versus 73.4\%, respectively). On the other hand, for Scenario 2, the one-class models outperformed the multi-class models in accuracy by 19.6\% on average (59.1\% versus 39.5\%, respectively). \linebreak 
%Lastly, when comparing results among experimental conditions, one can observe a decrease in the average accuracy over conditions for Scenario 1 with the multi-class models (see Table~\ref{tab:acc_multi_sc1}), but a oscillation over conditions in all other cases (see Tables \ref{tab:acc_one_sc1}-\ref{tab:acc_one_sc2}), with worse results for 1 week of data, better results for 2 weeks, and intermediate results for 3 weeks. 

In summary, the multi-class models yielded an overall average F-score of 83.6\% ($SD = 5.2\%$) while the one-class models produced an overall average F-score of 36.0\% ($SD = 14.8\%$). In other words, the multi-class approach significantly outperformed the one-class approach, with a difference of 47.6 percentage points in the overall average F-score.


% The highest overall average F-score was achieved with the multi-class models %for Scenario 1 
% ($M = 83.6\%$, $SD = 5.2\%$) followed by the one-class models %also for Scenario 1 
% ($M = 36.0\%$, $SD = 14.8\%$). %, then by the multi-class models for Scenario 2 ($M = 34.2\%$, $SD = 4.1\%$), and finally by the one-class models also for Scenario 2 ($M = 12.9\%$, $SD = 0.4\%$). 
% In other words, %our results show that predictions were more accurate for Scenario 1 (considering all processes used by the users) compared to Scenario 2 (considering only common processes among users). In terms of approach, 
% the multi-class models significantly outperformed the one-class models, %for both scenarios, 
% with a difference in the overall average F-score of 47.6 percentage points. \\ %(83.6\% versus 36.0\%). \\ %for Scenario 1 and of 21.3 percentage points (34.2\% versus 12.9\%) for Scenario 2. \\



% ===========================
% Profile Consistency
% ===========================

%\textbf{Computer Usage Profiles Consistency}
\subsection{Computer Usage Profiles Consistency}

%Figure~\ref{fig:fake_data} presents the SOM images per week and the classification curves resulted from our approach for the categorization of temporal changes in profiles for the synthetic test data used to simulate the four existing types of concept drift (see Figure~\ref{fig:drift_types}) plus absence of drift.
As previously explained, before using our approach for the categorization of temporal changes in computer usage profiles to analyze the data of our study participants, we first tested the approach using synthetic data with known types of temporal changes embedded to check whether the results were reliable. Figure \ref{fig:fake_data} presents the SOM images per week and the classification curves resulted for the synthetic test datasets, which simulated absence of drift, presence of sudden drift, presence of recurring concepts, presence of gradual drift, and presence of incremental drift. As expected, the SOM visualizations changed over weeks for the four types of concept drifts simulated, and remained unaffected when simulating absence of drift. Accordingly, the classification curves exhibited patterns of variability consistent with the type of concept drift simulated (see Figure \ref{fig:drift_types}), and an uniform behavior when simulating drift absence.


%Accordingly, the classification curves presented variability in all simulations of drift, and an uniform behavior for the absence of drift.

Table~\ref{tab:drift_per_user} exhibits the type of drift assigned to each study participant with our approach when temporal changes in profile were detected. Examples of SOM images and classification curves are displayed in Figure~\ref{fig:real_data} for some users. %For both Scenarios, 
We found an inter-rater reliability Kappa = 1.0, which means perfect agreement between coders when deciding presence and type of temporal changes in profiles for all study participants. In summary, %for both scenarios,
14 users (82.4\%) presented some identifiable pattern of temporal changes (with a higher prevalence of incremental drift and a lower prevalence of gradual drift), one user (5.9\%) did not present temporal changes, and two users (11.8\%) exhibited unidentifiable patterns of temporal changes, 
%it was observed a higher prevalence of incremental drift (35.3\% of the users), a lower prevalence of gradual drift (11.8\% of the users), one user (5.9\%) with no temporal changes detected, and two users (11.8\%) with unidentified changes in profile, 
where the SOM visualizations among weeks suggested changes in profile but the classification curves suggested the opposite (Figure~\ref{fig:unable_identify_drift}). %Further, 13 users (76.5\%) were assigned the same type of drift in both scenarios while four (23.5\%) were assigned different types between scenarios (Table~\ref{tab:drift_per_user}).

%Examples of SOM images and classification curves are displayed in Figure~\ref{fig:real_data} for some users.%\footnote{Due to space limitations, SOM visualizations and classification curves for all users are shown in Appendix~\ref{sec:appendix_drift}}. 



%%%%% FAKE DATA %%%%%
\begin{figure}[t]
    \centering
    \begin{minipage}{0.475\columnwidth}
        \centering
        % \hfill
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 1}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_nodrift_crop_week01-cropped-1.png}
            %\caption{W1.}
            %\label{fig:fake_nodrift1}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 2}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_nodrift_crop_week01-cropped-1.png}
            %\caption{W2.}
            %\label{fig:fake_nodrift2}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 3}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_nodrift_crop_week01-cropped-1.png}
            %\caption{W3.}
            %\label{fig:fake_nodrift3}
        \end{subfigure}
        % \hfill
        \par\smallskip
        \centering
        \begin{subfigure}[b]{\columnwidth}
            % \includegraphics[width=\columnwidth]{figs/new_version/curves/fake_data/fake_nodrift_svm_concept_drift_scenario_1_new-cropped.pdf}
            \includegraphics[width=\columnwidth]{figs/new_version/curves/fake_data/fake_no_drift_smaller-cropped.pdf}
            \caption{Absence of drift.}
            \label{fig:fake_nodrift_curve}
        \end{subfigure}
    
        % \caption{\hl{No drift (similar behaviors) artificial data results}.}
        % \label{fig:fake_data_nodrift}
    \end{minipage}
    \hfill
    \centering
    \begin{minipage}{0.475\columnwidth}
        \centering
        % \hfill
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 1}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_sudden_crop_week01-cropped-1.png}
            % \caption{W1.}
            % \label{fig:fake_sudden_drift1}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 2}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_sudden_crop_week02-cropped-1.png}
            %\caption{W2.}
            %\label{fig:fake_sudden_drift2}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 3}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_sudden_crop_week03-cropped-1.png}
            %\caption{W3.}
            %\label{fig:fake_sudden_drift3}
        \end{subfigure}
        % \hfill
        \par\smallskip
        \centering
        \begin{subfigure}[b]{\columnwidth}
            % \includegraphics[width=\columnwidth]{figs/new_version/curves/fake_data/fake_sudden_svm_concept_drift_scenario_1_new-cropped.pdf}
            \includegraphics[width=\columnwidth]{figs/new_version/curves/fake_data/fake_sudden_drift_smaller-cropped.pdf}
            \caption{Sudden drift.}
            \label{fig:fake_sudden_drift_curve}
        \end{subfigure}
    
        %\caption{\hl{Sudden drift artificial data results}.}
        %\label{fig:fake_data_sudden_drift}
    \end{minipage}
    \par\bigskip
    \centering
    % \hfill
    \centering
    \begin{minipage}{0.475\columnwidth}
        \centering
        % \hfill
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 1}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_recurring_crop_week01-cropped-1.png}
            % \caption{Week 1.}
            % \label{fig:fake_recurring_drift1}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 2}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_recurring_crop_week02-cropped-1.png}
            % \caption{Week 2.}
            % \label{fig:fake_recurring_drift2}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 3}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_recurring_crop_week03-cropped-1.png}
            % \caption{Week 3.}
            % \label{fig:fake_recurring_drift3}
        \end{subfigure}
        % \hfill
        \par\smallskip
        \centering
        \begin{subfigure}[b]{\columnwidth}
            % \includegraphics[width=\columnwidth]{figs/new_version/curves/fake_data/fake_recurring_svm_concept_drift_scenario_1_new-cropped.pdf}
            \includegraphics[width=\columnwidth]{figs/new_version/curves/fake_data/fake_rec_drift_smaller-cropped.pdf}
            \caption{Recurring concepts.}
            \label{fig:fake_recurring_drift_curve}
        \end{subfigure}
    
        %\caption{\hl{Recurring concept artificial data results}.}
        %\label{fig:fake_data_recurring_drift}
    \end{minipage}
    % \hfill
    \hfill
    % \par\bigskip
    \centering
    \begin{minipage}{0.475\columnwidth}
        \centering
        % \hfill
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 1}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_gradual_crop_week01-cropped-1.png}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 2}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_gradual_crop_week02-cropped-1.png}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 3}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_gradual_crop_week03-cropped-1.png}
        \end{subfigure}
        % \hfill
        \par\smallskip
        \centering
        \begin{subfigure}[b]{\columnwidth}
            % \includegraphics[width=\columnwidth]{figs/new_version/curves/fake_data/fake_gradual_svm_concept_drift_scenario_1_new-cropped.pdf}
            \includegraphics[width=\columnwidth]{figs/new_version/curves/fake_data/fake_grad_drift_smaller-cropped.pdf}
            \caption{Gradual drift.}
            \label{fig:fake_gradual_drift_curve}
        \end{subfigure}
    
        % \caption{\hl{Recurring concept artificial data results}.}
        % \label{fig:fake_data_recurring_drift}
    \end{minipage}
    \par\bigskip
    \centering
    \begin{minipage}{0.475\columnwidth}
        \centering
        % \hfill
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 1}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_incremental_crop_week01-cropped-1.png}
            % \caption{Week 1.}
            % \label{fig:fake_recurring_drift1}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 2}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_incremental_crop_week02-cropped-1.png}
            % \caption{Week 2.}
            % \label{fig:fake_recurring_drift2}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 3}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_incremental_crop_week03-cropped-1.png}
            % \caption{Week 3.}
            % \label{fig:fake_recurring_drift3}
        \end{subfigure}
        % \hfill
        \par\smallskip
        \centering
        \begin{subfigure}[b]{\columnwidth}
            % \includegraphics[width=\columnwidth]{figs/new_version/curves/fake_data/fake_incremental_svm_concept_drift_scenario_1_new-cropped.pdf}
            \includegraphics[width=\columnwidth]{figs/new_version/curves/fake_data/fake_inc_drift_smaller-cropped.pdf}
            \caption{Incremental drift.}
            \label{fig:fake_incremental_drift_curve}
        \end{subfigure}
    \end{minipage}
    \caption{SOM visualizations over weeks and classification curves for synthetic test datasets simulating computer usage with    (\subref{fig:fake_nodrift_curve}) absence of drift, (\subref{fig:fake_sudden_drift_curve}) presence of sudden drift, (\subref{fig:fake_recurring_drift_curve}) presence of recurring concepts, (\subref{fig:fake_gradual_drift_curve}) presence of gradual drift, and (\subref{fig:fake_incremental_drift_curve}) presence of incremental drift.}
    \label{fig:fake_data}
    % \vspace{-1.5em}
\end{figure}

% \begin{figure*}[t]
%     \centering
%     \begin{minipage}{0.325\textwidth}
%         \centering
%         % \hfill
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 1}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_nodrift_crop_week01-cropped-1.png}
%             %\caption{W1.}
%             %\label{fig:fake_nodrift1}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 2}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_nodrift_crop_week01-cropped-1.png}
%             %\caption{W2.}
%             %\label{fig:fake_nodrift2}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 3}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_nodrift_crop_week01-cropped-1.png}
%             %\caption{W3.}
%             %\label{fig:fake_nodrift3}
%         \end{subfigure}
%         % \hfill
%         \par\smallskip
%         \centering
%         \begin{subfigure}[b]{\columnwidth}
%             % \includegraphics[width=\columnwidth]{figs/new_version/curves/fake_data/fake_nodrift_svm_concept_drift_scenario_1_new-cropped.pdf}
%             \includegraphics[width=\columnwidth]{figs/new_version/curves/fake_data/fake_no_drift_smaller-cropped.pdf}
%             \caption{Absence of drift.}
%             \label{fig:fake_nodrift_curve}
%         \end{subfigure}
    
%         % \caption{\hl{No drift (similar behaviors) artificial data results}.}
%         % \label{fig:fake_data_nodrift}
%     \end{minipage}
%     \hfill
%     \centering
%     \begin{minipage}{0.325\textwidth}
%         \centering
%         % \hfill
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 1}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_sudden_crop_week01-cropped-1.png}
%             % \caption{W1.}
%             % \label{fig:fake_sudden_drift1}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 2}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_sudden_crop_week02-cropped-1.png}
%             %\caption{W2.}
%             %\label{fig:fake_sudden_drift2}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 3}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_sudden_crop_week03-cropped-1.png}
%             %\caption{W3.}
%             %\label{fig:fake_sudden_drift3}
%         \end{subfigure}
%         % \hfill
%         \par\smallskip
%         \centering
%         \begin{subfigure}[b]{\columnwidth}
%             % \includegraphics[width=\columnwidth]{figs/new_version/curves/fake_data/fake_sudden_svm_concept_drift_scenario_1_new-cropped.pdf}
%             \includegraphics[width=\columnwidth]{figs/new_version/curves/fake_data/fake_sudden_drift_smaller-cropped.pdf}
%             \caption{Sudden drift.}
%             \label{fig:fake_sudden_drift_curve}
%         \end{subfigure}
    
%         %\caption{\hl{Sudden drift artificial data results}.}
%         %\label{fig:fake_data_sudden_drift}
%     \end{minipage}
%     \hfill
%     \centering
%     \begin{minipage}{0.325\textwidth}
%         \centering
%         % \hfill
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 1}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_recurring_crop_week01-cropped-1.png}
%             % \caption{Week 1.}
%             % \label{fig:fake_recurring_drift1}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 2}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_recurring_crop_week02-cropped-1.png}
%             % \caption{Week 2.}
%             % \label{fig:fake_recurring_drift2}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 3}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_recurring_crop_week03-cropped-1.png}
%             % \caption{Week 3.}
%             % \label{fig:fake_recurring_drift3}
%         \end{subfigure}
%         % \hfill
%         \par\smallskip
%         \centering
%         \begin{subfigure}[b]{\columnwidth}
%             % \includegraphics[width=\columnwidth]{figs/new_version/curves/fake_data/fake_recurring_svm_concept_drift_scenario_1_new-cropped.pdf}
%             \includegraphics[width=\columnwidth]{figs/new_version/curves/fake_data/fake_rec_drift_smaller-cropped.pdf}
%             \caption{Recurring concepts.}
%             \label{fig:fake_recurring_drift_curve}
%         \end{subfigure}
    
%         %\caption{\hl{Recurring concept artificial data results}.}
%         %\label{fig:fake_data_recurring_drift}
%     \end{minipage}
%     % \hfill
%     \par\bigskip
%     \centering
%     \begin{minipage}{0.325\textwidth}
%         \centering
%         % \hfill
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 1}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_gradual_crop_week01-cropped-1.png}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 2}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_gradual_crop_week02-cropped-1.png}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 3}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_gradual_crop_week03-cropped-1.png}
%         \end{subfigure}
%         % \hfill
%         \par\smallskip
%         \centering
%         \begin{subfigure}[b]{\columnwidth}
%             % \includegraphics[width=\columnwidth]{figs/new_version/curves/fake_data/fake_gradual_svm_concept_drift_scenario_1_new-cropped.pdf}
%             \includegraphics[width=\columnwidth]{figs/new_version/curves/fake_data/fake_grad_drift_smaller-cropped.pdf}
%             \caption{Gradual drift.}
%             \label{fig:fake_gradual_drift_curve}
%         \end{subfigure}
    
%         % \caption{\hl{Recurring concept artificial data results}.}
%         % \label{fig:fake_data_recurring_drift}
%     \end{minipage}
%     ~% \hfill
%     \centering
%     \begin{minipage}{0.325\textwidth}
%         \centering
%         % \hfill
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 1}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_incremental_crop_week01-cropped-1.png}
%             % \caption{Week 1.}
%             % \label{fig:fake_recurring_drift1}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 2}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_incremental_crop_week02-cropped-1.png}
%             % \caption{Week 2.}
%             % \label{fig:fake_recurring_drift2}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 3}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/fake_data/user03_id11003_fake_incremental_crop_week03-cropped-1.png}
%             % \caption{Week 3.}
%             % \label{fig:fake_recurring_drift3}
%         \end{subfigure}
%         % \hfill
%         \par\smallskip
%         \centering
%         \begin{subfigure}[b]{\columnwidth}
%             % \includegraphics[width=\columnwidth]{figs/new_version/curves/fake_data/fake_incremental_svm_concept_drift_scenario_1_new-cropped.pdf}
%             \includegraphics[width=\columnwidth]{figs/new_version/curves/fake_data/fake_inc_drift_smaller-cropped.pdf}
%             \caption{Incremental drift.}
%             \label{fig:fake_incremental_drift_curve}
%         \end{subfigure}
%     \end{minipage}
%     \caption{SOM visualizations over weeks and classification curves for artificial usage data simulating (\subref{fig:fake_nodrift_curve}) absence of drift, (\subref{fig:fake_sudden_drift_curve}) sudden drift, (\subref{fig:fake_recurring_drift_curve}) recurring concepts, (\subref{fig:fake_gradual_drift_curve}) gradual drift, and (\subref{fig:fake_incremental_drift_curve}) incremental drift.}
%     \label{fig:fake_data}
%     \vspace{-1.5em}
% \end{figure*}


%Table~\ref{tab:drift_summary} summarizes the total amount of participants categorized in each type of concept drift. As shown, in both Scenarios, we found presence of drift for 14 study participants (82.4\%) and absence of drift for a single participant (5.9\%). Accordingly, results from the first experiment also exhibit temporal inconsistency in profiles when comparing the average accuracies among conditions. More specifically, one can observe a decrease in this average accuracy over the conditions for Scenario 1 with the multi-class models (see Table~\ref{tab:acc_multi_sc1}), and a oscillation over conditions in all other cases (see Tables~\ref{tab:acc_one_sc1}-\ref{tab:acc_one_sc2}), with worse results for 1 week of data, better results for 2 weeks, and intermediate results for 3 weeks. Finally, our approach could not properly identify concept drift for two participants (11.8\%) in both scenarios. In these cases, as exemplified in Figure~\ref{fig:unable_identify_drift}, the SOM visualizations among weeks were considered to suggest temporal changes in profiles, but the classification curves were considered to suggest the opposite. \linebreak


%%% REAL DATA %%%
\begin{figure}[t]
    % user 03
    \centering
    \begin{minipage}{0.475\columnwidth}
        \centering
        % \hfill
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 1}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/user03_week01-cropped-1.png}
            %\caption{W1.}
            %\label{fig:fake_nodrift1}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 2}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/user03_week02-cropped-1.png}
            %\caption{W2.}
            %\label{fig:fake_nodrift2}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 3}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/user03_week03-cropped-1.png}
            %\caption{W3.}
            %\label{fig:fake_nodrift3}
        \end{subfigure}
        % \hfill
        \par\smallskip
        \centering
        \begin{subfigure}[b]{\columnwidth}
            % \includegraphics[width=\columnwidth]{figs/new_version/curves/user03_no_drift-cropped.pdf}
            \includegraphics[width=\columnwidth]{figs/new_version/curves/real_data/real_no_drift_smaller-cropped.pdf}
            \caption{Absence of drift (User-03).}
            \label{fig:real03_nodrift_curve}
        \end{subfigure}

        % \caption{\hl{No drift (similar behaviors) artificial data results}.}
        % \label{fig:fake_data_nodrift}
    \end{minipage}
    \hfill
    % user 06
    \centering
    \begin{minipage}{0.475\columnwidth}
        \centering
        % \hfill
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 1}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user06_week01-cropped-1.png}
            % \caption{W1.}
            % \label{fig:fake_sudden_drift1}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 2}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user06_week02-cropped-1.png}
            %\caption{W2.}
            %\label{fig:fake_sudden_drift2}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 3}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user06_week03-cropped-1.png}
            %\caption{W3.}
            %\label{fig:fake_sudden_drift3}
        \end{subfigure}
        % \hfill
        \par\smallskip
        \centering
        \begin{subfigure}[b]{\columnwidth}
            % \includegraphics[width=\columnwidth]{figs/new_version/curves/user06_sudden-cropped.pdf}
            \includegraphics[width=\columnwidth]{figs/new_version/curves/real_data/real_sudden_drift_smaller-cropped.pdf}
            \caption{Sudden drift (User-06).}
            \label{fig:real06_sudden_drift_curve}
        \end{subfigure}
    
        %\caption{\hl{Sudden drift artificial data results}.}
        %\label{fig:fake_data_sudden_drift}
    \end{minipage}
    \par\bigskip
    % user 09
    \begin{minipage}{0.475\columnwidth}
        \centering
        % \hfill
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 1}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user09_week01-cropped-1.png}
            % \caption{Week 1.}
            % \label{fig:fake_recurring_drift1}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 2}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user09_week02-cropped-1.png}
            % \caption{Week 2.}
            % \label{fig:fake_recurring_drift2}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 3}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user09_week03-cropped-1.png}
            % \caption{Week 3.}
            % \label{fig:fake_recurring_drift3}
        \end{subfigure}
        % \hfill
        \par\smallskip
        \centering
        \begin{subfigure}[b]{\columnwidth}
            % \includegraphics[width=\columnwidth]{figs/new_version/curves/user09_recurring-cropped.pdf}
            \includegraphics[width=\columnwidth]{figs/new_version/curves/real_data/real_rec_drift_smaller-cropped.pdf}
            \caption{Recurring drift (User-09).}
            \label{fig:real09_recurring_drift_curve}
        \end{subfigure}
    
        %\caption{\hl{Recurring concept artificial data results}.}
        %\label{fig:fake_data_recurring_drift}
    \end{minipage}
    % \hfill
    \hfill
    % user 10
    \centering
    \begin{minipage}{0.475\columnwidth}
        \centering
        % \hfill
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 1}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user10_week01-cropped-1.png}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 2}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user10_week02-cropped-1.png}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 3}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user10_week03-cropped-1.png}
        \end{subfigure}
        % \hfill
        \par\smallskip
        \centering
        \begin{subfigure}[b]{\columnwidth}
            % \includegraphics[width=\columnwidth]{figs/new_version/curves/user10_gradual-cropped.pdf}
            \includegraphics[width=\columnwidth]{figs/new_version/curves/real_data/real_grad_drift_smaller-cropped.pdf}
            \caption{Gradual drift (User-10).}
            \label{fig:real10_gradual_drift_curve}
        \end{subfigure}
    
        % \caption{\hl{Recurring concept artificial data results}.}
        % \label{fig:fake_data_recurring_drift}
    \end{minipage}
    \par\bigskip
    % user 05
    \centering
    \begin{minipage}{0.475\columnwidth}
        \centering
        % \hfill
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 1}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user05_week01-cropped-1.png}
            % \caption{Week 1.}
            % \label{fig:fake_recurring_drift1}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 2}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user05_week02-cropped-1.png}
            % \caption{Week 2.}
            % \label{fig:fake_recurring_drift2}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 3}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user05_week03-cropped-1.png}
            % \caption{Week 3.}
            % \label{fig:fake_recurring_drift3}
        \end{subfigure}
        % \hfill
        \par\smallskip
        \centering
        \begin{subfigure}[b]{\columnwidth}
            % \includegraphics[width=\columnwidth]{figs/new_version/curves/user05_incremental-cropped.pdf}
            \includegraphics[width=\columnwidth]{figs/new_version/curves/real_data/real_inc_drift_smaller-cropped.pdf}
            \caption{Incremental drift (User-05).}
            \label{fig:real05_incremental_drift_curve}
        \end{subfigure}
    \end{minipage}
    % user 11, problematic
    \hfill
    \begin{minipage}{0.475\columnwidth}
        \centering
        % \hfill
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 1}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/user11_week01-cropped-1.png}
            %\caption{W1.}
            %\label{fig:fake_nodrift1}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 2}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/user11_week02-cropped-1.png}
            %\caption{W2.}
            %\label{fig:fake_nodrift2}
        \end{subfigure}
        \begin{subfigure}[b]{.315\columnwidth}
            \caption*{week 3}
            % \vspace{-.5em}
            \includegraphics[width=\columnwidth]{figs/new_version/som/user11_week03-cropped-1.png}
            %\caption{W3.}
            %\label{fig:fake_nodrift3}
        \end{subfigure}
        % \hfill
        \par\smallskip
        \centering
        \begin{subfigure}[b]{\columnwidth}
            % \includegraphics[width=\columnwidth]{figs/new_version/curves/scenario1/user11_id12001_svm_concept_drift_scenario_1-cropped.pdf}
            \includegraphics[width=\columnwidth]{figs/new_version/curves/real_data/real_unable_identify_smaller-cropped.pdf}
            \caption{Unable to identify (User-11).}
            % \label{fig:real11_unable_curve}
            \label{fig:unable_identify_drift}
        \end{subfigure}

        % \caption{\hl{No drift (similar behaviors) artificial data results}.}
        % \label{fig:fake_data_nodrift}
    \end{minipage}
    \caption{SOM images over weeks and classification curves for six study participants whose computer usage profiles were considered to present (\subref{fig:real03_nodrift_curve}) absence of drift, (\subref{fig:real06_sudden_drift_curve}) sudden drift, (\subref{fig:real09_recurring_drift_curve}) recurring concepts, (\subref{fig:real10_gradual_drift_curve}) gradual drift, (\subref{fig:real05_incremental_drift_curve}) incremental drift, and (\subref{fig:unable_identify_drift}) drift unable to identify.}
    \label{fig:real_data}
    % \vspace{-1.5em}
\end{figure}

% \begin{figure*}[t]
%     % user 03
%     \centering
%     \begin{minipage}{0.325\textwidth}
%         \centering
%         % \hfill
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 1}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user03_week01-cropped-1.png}
%             %\caption{W1.}
%             %\label{fig:fake_nodrift1}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 2}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user03_week02-cropped-1.png}
%             %\caption{W2.}
%             %\label{fig:fake_nodrift2}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 3}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user03_week03-cropped-1.png}
%             %\caption{W3.}
%             %\label{fig:fake_nodrift3}
%         \end{subfigure}
%         % \hfill
%         \par\smallskip
%         \centering
%         \begin{subfigure}[b]{\columnwidth}
%             % \includegraphics[width=\columnwidth]{figs/new_version/curves/user03_no_drift-cropped.pdf}
%             \includegraphics[width=\columnwidth]{figs/new_version/curves/real_data/real_no_drift_smaller-cropped.pdf}
%             \caption{User-03 (Scenario 1): absence of drift.}
%             \label{fig:real03_nodrift_curve}
%         \end{subfigure}

%         % \caption{\hl{No drift (similar behaviors) artificial data results}.}
%         % \label{fig:fake_data_nodrift}
%     \end{minipage}
%     \hfill
%     % user 06
%     \centering
%     \begin{minipage}{0.325\textwidth}
%         \centering
%         % \hfill
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 1}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user06_week01-cropped-1.png}
%             % \caption{W1.}
%             % \label{fig:fake_sudden_drift1}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 2}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user06_week02-cropped-1.png}
%             %\caption{W2.}
%             %\label{fig:fake_sudden_drift2}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 3}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user06_week03-cropped-1.png}
%             %\caption{W3.}
%             %\label{fig:fake_sudden_drift3}
%         \end{subfigure}
%         % \hfill
%         \par\smallskip
%         \centering
%         \begin{subfigure}[b]{\columnwidth}
%             % \includegraphics[width=\columnwidth]{figs/new_version/curves/user06_sudden-cropped.pdf}
%             \includegraphics[width=\columnwidth]{figs/new_version/curves/real_data/real_sudden_drift_smaller-cropped.pdf}
%             \caption{User-06 (Scenario 1): sudden drift.}
%             \label{fig:real06_sudden_drift_curve}
%         \end{subfigure}
    
%         %\caption{\hl{Sudden drift artificial data results}.}
%         %\label{fig:fake_data_sudden_drift}
%     \end{minipage}
%     \hfill
%     % user 09
%     \begin{minipage}{0.325\textwidth}
%         \centering
%         % \hfill
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 1}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user09_week01-cropped-1.png}
%             % \caption{Week 1.}
%             % \label{fig:fake_recurring_drift1}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 2}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user09_week02-cropped-1.png}
%             % \caption{Week 2.}
%             % \label{fig:fake_recurring_drift2}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 3}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user09_week03-cropped-1.png}
%             % \caption{Week 3.}
%             % \label{fig:fake_recurring_drift3}
%         \end{subfigure}
%         % \hfill
%         \par\smallskip
%         \centering
%         \begin{subfigure}[b]{\columnwidth}
%             % \includegraphics[width=\columnwidth]{figs/new_version/curves/user09_recurring-cropped.pdf}
%             \includegraphics[width=\columnwidth]{figs/new_version/curves/real_data/real_rec_drift_smaller-cropped.pdf}
%             \caption{User-09 (Scenario 1): recurring concepts.}
%             \label{fig:real09_recurring_drift_curve}
%         \end{subfigure}
    
%         %\caption{\hl{Recurring concept artificial data results}.}
%         %\label{fig:fake_data_recurring_drift}
%     \end{minipage}
%     % \hfill
%     \par\bigskip
%     % user 10
%     \centering
%     \begin{minipage}{0.325\textwidth}
%         \centering
%         % \hfill
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 1}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user10_week01-cropped-1.png}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 2}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user10_week02-cropped-1.png}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 3}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user10_week03-cropped-1.png}
%         \end{subfigure}
%         % \hfill
%         \par\smallskip
%         \centering
%         \begin{subfigure}[b]{\columnwidth}
%             % \includegraphics[width=\columnwidth]{figs/new_version/curves/user10_gradual-cropped.pdf}
%             \includegraphics[width=\columnwidth]{figs/new_version/curves/real_data/real_grad_drift_smaller-cropped.pdf}
%             \caption{User-10 (Scenario 1): gradual drift.}
%             \label{fig:real10_gradual_drift_curve}
%         \end{subfigure}
    
%         % \caption{\hl{Recurring concept artificial data results}.}
%         % \label{fig:fake_data_recurring_drift}
%     \end{minipage}
%     \hfill
%     % user 05
%     \centering
%     \begin{minipage}{0.325\textwidth}
%         \centering
%         % \hfill
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 1}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user05_week01-cropped-1.png}
%             % \caption{Week 1.}
%             % \label{fig:fake_recurring_drift1}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 2}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user05_week02-cropped-1.png}
%             % \caption{Week 2.}
%             % \label{fig:fake_recurring_drift2}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 3}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/scenario1/user05_week03-cropped-1.png}
%             % \caption{Week 3.}
%             % \label{fig:fake_recurring_drift3}
%         \end{subfigure}
%         % \hfill
%         \par\smallskip
%         \centering
%         \begin{subfigure}[b]{\columnwidth}
%             % \includegraphics[width=\columnwidth]{figs/new_version/curves/user05_incremental-cropped.pdf}
%             \includegraphics[width=\columnwidth]{figs/new_version/curves/real_data/real_inc_drift_smaller-cropped.pdf}
%             \caption{User-05 (Scenario 1): incremental drift.}
%             \label{fig:real05_incremental_drift_curve}
%         \end{subfigure}
%     \end{minipage}
%     % user 11, problematic
%     \hfill
%     \begin{minipage}{0.325\textwidth}
%         \centering
%         % \hfill
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 1}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user11_week01-cropped-1.png}
%             %\caption{W1.}
%             %\label{fig:fake_nodrift1}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 2}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user11_week02-cropped-1.png}
%             %\caption{W2.}
%             %\label{fig:fake_nodrift2}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 3}
%             % \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user11_week03-cropped-1.png}
%             %\caption{W3.}
%             %\label{fig:fake_nodrift3}
%         \end{subfigure}
%         % \hfill
%         \par\smallskip
%         \centering
%         \begin{subfigure}[b]{\columnwidth}
%             % \includegraphics[width=\columnwidth]{figs/new_version/curves/scenario1/user11_id12001_svm_concept_drift_scenario_1-cropped.pdf}
%             \includegraphics[width=\columnwidth]{figs/new_version/curves/real_data/real_unable_identify_smaller-cropped.pdf}
%             \caption{User-11 (Scenario 1): unable to identify.}
%             % \label{fig:real11_unable_curve}
%             \label{fig:unable_identify_drift}
%         \end{subfigure}

%         % \caption{\hl{No drift (similar behaviors) artificial data results}.}
%         % \label{fig:fake_data_nodrift}
%     \end{minipage}
%     \caption{SOM visualizations over weeks and classification curves for real usage data considered to present (\subref{fig:real03_nodrift_curve}) absence of drift, (\subref{fig:real06_sudden_drift_curve}) sudden drift, (\subref{fig:real09_recurring_drift_curve}) recurring concepts, (\subref{fig:real10_gradual_drift_curve}) gradual drift, (\subref{fig:real05_incremental_drift_curve}) incremental drift, and (\subref{fig:unable_identify_drift}) drift unable to identified.}
%     \label{fig:real_data}
%     \vspace{-1.5em}
% \end{figure*}


% \begin{figure*}[t]
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user17_week01-cropped-1.png}
%             \caption{Week 1.}
%             \label{fig:drift_users_17_1}
%         \end{subfigure}
%         ~
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user17_week02-cropped-1.png}
%             \caption{Week 2.}
%             \label{fig:drift_users_17_2}
%         \end{subfigure}
%         ~
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user17_week03-cropped-1.png}
%             \caption{Week 3.}
%             \label{fig:drift_users_17_3}
%         \end{subfigure}
%         \hfill
        
%         \centering
%         \begin{subfigure}[b]{.9\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/curves/user17_svm_drift_es1.pdf}
%             \caption{Accuracy curve.}
%             \label{fig:drift_users_17_curve}
%         \end{subfigure}
    
%         \caption{\hl{User 17 behavior classified as sudden drift}.}
%         \label{fig:drift_users_17}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user08_week01-cropped-1.png}
%             \caption{Week 1.}
%             \label{fig:drift_users_08_1}
%         \end{subfigure}
%         ~
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user08_week02-cropped-1.png}
%             \caption{Week 2.}
%             \label{fig:drift_users_08_2}
%         \end{subfigure}
%         ~
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user08_week03-cropped-1.png}
%             \caption{Week 3.}
%             \label{fig:drift_users_08_3}
%         \end{subfigure}
%         \hfill
        
%         \centering
%         \begin{subfigure}[b]{.9\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/curves/user08_svm_drift_es1.pdf}
%             \caption{Accuracy curve.}
%             \label{fig:drift_users_08_curve}
%         \end{subfigure}
    
%         \caption{\hl{User 08 behavior classified as recurring concepts}.}
%         \label{fig:drift_users_08}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user06_week01-cropped-1.png}
%             \caption{Week 1.}
%             \label{fig:drift_users_06_1}
%         \end{subfigure}
%         ~
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user06_week02-cropped-1.png}
%             \caption{Week 2.}
%             \label{fig:drift_users_06_2}
%         \end{subfigure}
%         ~
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user06_week03-cropped-1.png}
%             \caption{Week 3.}
%             \label{fig:drift_users_06_3}
%         \end{subfigure}
%         \hfill
        
%         \centering
%         \begin{subfigure}[b]{.9\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/curves/user06_svm_drift_es1.pdf}
%             \caption{Accuracy curve.}
%             \label{fig:drift_users_06_curve}
%         \end{subfigure}
    
%         \caption{\hl{User 06 behavior classified as gradual drift}.}
%         \label{fig:drift_users_06}
%     \end{minipage}
% \end{figure*}

% \begin{figure}[t]
%     \centering
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user15_week01-cropped-1.png}
%             \caption{Week 1.}
%             \label{fig:drift_users_15_1}
%         \end{subfigure}
%         ~
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user15_week02-cropped-1.png}
%             \caption{Week 2.}
%             \label{fig:drift_users_15_2}
%         \end{subfigure}
%         ~
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user15_week03-cropped-1.png}
%             \caption{Week 3.}
%             \label{fig:drift_users_15_3}
%         \end{subfigure}
%         \hfill
        
%         \centering
%         \begin{subfigure}[b]{.9\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/curves/user15_svm_drift_es1.pdf}
%             \caption{Accuracy curve.}
%             \label{fig:drift_users_15_curve}
%         \end{subfigure}
%     \end{minipage}
%     \caption{\hl{User 15 behavior classified as incremental drift}.}
%     \label{fig:drift_users_15}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user03_week01-cropped-1.png}
%             \caption{Week 1.}
%             \label{fig:drift_users_03_1}
%         \end{subfigure}
%         ~
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user03_week02-cropped-1.png}
%             \caption{Week 2.}
%             \label{fig:drift_users_03_2}
%         \end{subfigure}
%         ~
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user03_week03-cropped-1.png}
%             \caption{Week 3.}
%             \label{fig:drift_users_03_3}
%         \end{subfigure}
%         \hfill
        
%         \centering
%         \begin{subfigure}[b]{.9\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/curves/user03_svm_drift_es1.pdf}
%             \caption{Accuracy curve.}
%             \label{fig:drift_users_03_curve}
%         \end{subfigure}
%     \end{minipage}
%     \caption{\hl{User 03 behavior classified as no drift (similar behaviors)}.}
%     \label{fig:drift_users_03}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figs/new_version/drift_users.pdf}
%     \caption{SOM images and classification curves for different study participants. \hl{To do: improve the quality of the figure}}
%     \label{fig:drift_users}
% \end{figure}


\begin{table}[t]
\caption{Type of concept drift assigned to study participants. %\\$^{*}$denotes users with different drift types between scenarios.
}
\label{tab:drift_per_user}
\centering
\begin{tabular}{|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}Participant ID (de-identified)\end{tabular} & %\begin{tabular}[c]{@{}c@{}}Scenario 1\end{tabular} &
\begin{tabular}[c]{@{}c@{}}Type of drift assigned\end{tabular} \\ \hline
User-01 & Sudden drift  \\ \hline
User-02 & Unable to identify \\ \hline
User-03 & Absence of drift \\ \hline
User-04 & Recurring concepts \\ \hline
User-05 & Incremental drift \\ \hline
User-06 & Sudden drift \\ \hline
User-07 & Gradual drift \\ \hline
User-08 & Recurring concepts \\ \hline
User-09 & Recurring concepts \\ \hline
User-10 & Gradual drift \\ \hline
User-11 & Unable to identify  \\ \hline
User-12 & Incremental drift \\ \hline
User-13 & Incremental drift \\ \hline
User-14 & Sudden drift \\ \hline
User-15 & Incremental drift \\ \hline
User-16 & Incremental drift \\ \hline
User-17 & Incremental drift \\ \hline
\end{tabular}

% \vspace{-2.5em}
\end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{|c|c|c|}
% \hline
% Drift type & \begin{tabular}[c]{@{}c@{}}Scenario 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}Scenario 2\end{tabular} \\ \hline
% % Incremental & 5 (29.4\%) & 7 (41.2\%) \\ \hline
% % Recurring & 5 (29.4\%) & 5 (29.4\%) \\ \hline
% % Sudden & 3 (17.6\%) & 2 (11.8\%) \\ \hline
% % Gradual & 2 (11.8\%) & 2 (11.8\%) \\ \hline
% % No drift & 1 (5.9\%) & 0 (0.0\%) \\ \hline
% % Unable to identify & 1 (5.9\%) & 1 (5.9\%) \\ \hline
% Incremental & 6 (35.3\%) & 6 (35.3\%) \\ \hline
% Recurring & 3 (17.6\%) & 4 (23.5\%) \\ \hline
% Sudden & 3 (17.6\%) & 2 (11.8\%) \\ \hline
% Gradual & 2 (11.8\%) & 2 (11.8\%) \\ \hline
% Absence & 1 (5.9\%) & 1 (5.9\%) \\ \hline
% Unable to identify & 2 (11.8\%) & 2 (11.8\%) \\ \hline
% \end{tabular}
% \caption{Summary of study users per type of concept drift.}
% \label{tab:drift_summary}
% \vspace{-1.75em}
% \end{table}

%%% REAL UNABLE DATA %%%
% \begin{figure}[t]
%     % user 11
%     \centering
%     \begin{minipage}{0.325\textwidth}
%         \centering
%         % \hfill
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 1}
%             \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user11_week01-cropped-1.png}
%             %\caption{W1.}
%             %\label{fig:fake_nodrift1}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 2}
%             \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user11_week02-cropped-1.png}
%             %\caption{W2.}
%             %\label{fig:fake_nodrift2}
%         \end{subfigure}
%         \begin{subfigure}[b]{.315\columnwidth}
%             \caption*{week 3}
%             \vspace{-.5em}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user11_week03-cropped-1.png}
%             %\caption{W3.}
%             %\label{fig:fake_nodrift3}
%         \end{subfigure}
%         % \hfill
%         \par\medskip
%         \centering
%         \begin{subfigure}[b]{\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/curves/scenario1/user11_id12001_svm_concept_drift_scenario_1-cropped.pdf}
%             \caption{\hl{User 11, First Scenario}}
%             \label{fig:real11_unable_curve}
%         \end{subfigure}

%         % \caption{\hl{No drift (similar behaviors) artificial data results}.}
%         % \label{fig:fake_data_nodrift}
%     \end{minipage}
%     ~%\hfill
%     % user 01, es2
%     % \centering
%     % \begin{minipage}{0.23\textwidth}
%     %     \centering
%     %     % \hfill
%     %     \begin{subfigure}[b]{.315\columnwidth}
%     %         \caption*{week 1}
%     %         \vspace{-.5em}
%     %         \includegraphics[width=\columnwidth]{figs/new_version/som/user01_week01-cropped-1.png}
%     %         % \caption{W1.}
%     %         % \label{fig:fake_sudden_drift1}
%     %     \end{subfigure}
%     %     \begin{subfigure}[b]{.315\columnwidth}
%     %         \caption*{week 2}
%     %         \vspace{-.5em}
%     %         \includegraphics[width=\columnwidth]{figs/new_version/som/user01_week02-cropped-1.png}
%     %         %\caption{W2.}
%     %         %\label{fig:fake_sudden_drift2}
%     %     \end{subfigure}
%     %     \begin{subfigure}[b]{.315\columnwidth}
%     %         \caption*{week 3}
%     %         \vspace{-.5em}
%     %         \includegraphics[width=\columnwidth]{figs/new_version/som/user01_week03-cropped-1.png}
%     %         %\caption{W3.}
%     %         %\label{fig:fake_sudden_drift3}
%     %     \end{subfigure}
%     %     % \hfill
%     %     \par\medskip
%     %     \centering
%     %     \begin{subfigure}[b]{\columnwidth}
%     %         \includegraphics[width=\columnwidth]{figs/new_version/curves/scenario2/user01_id11001_svm_concept_drift_scenario_2-cropped.pdf}
%     %         \caption{\hl{User 01, Second Scenario}}
%     %         \label{fig:real01_unable_curve}
%     %     \end{subfigure}
%     % \end{minipage}
    
%     \caption{SOM images and classification curves that provided contrasting conclusions about presence of concept drift. %in usage profiles: (\subref{fig:real11_unable_curve}) user 11, experimental scenario 1 and (\subref{fig:real01_unable_curve}) user 01, experimental scenario 2.
%     }
%     \label{fig:unable_identify_drift}
%     \vspace{-1.5em}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user11_week01-cropped-1.png}
%             \caption{Week 1.}
%             \label{fig:drift_users_11_1}
%         \end{subfigure}
%         ~
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user11_week02-cropped-1.png}
%             \caption{Week 2.}
%             \label{fig:drift_users_11_2}
%         \end{subfigure}
%         ~
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user11_week03-cropped-1.png}
%             \caption{Week 3.}
%             \label{fig:drift_users_11_3}
%         \end{subfigure}
%         \hfill
        
%         \centering
%         \begin{subfigure}[b]{.9\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/curves/user11_svm_drift_es1.pdf}
%             \caption{Accuracy curve.}
%             \label{fig:drift_users_11_curve}
%         \end{subfigure}
%     \end{minipage}
%     \caption{\hl{User 11 SOM images and classification curves for experimental scenario 1 provided contrasting conclusions about presence of concept drift in usage profiles}.}
%     \label{fig:drift_users_11}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user01_week01-cropped-1.png}
%             \caption{Week 1.}
%             \label{fig:drift_users_01_1}
%         \end{subfigure}
%         ~
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user01_week02-cropped-1.png}
%             \caption{Week 2.}
%             \label{fig:drift_users_01_2}
%         \end{subfigure}
%         ~
%         \begin{subfigure}[b]{.26\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/som/user01_week03-cropped-1.png}
%             \caption{Week 3.}
%             \label{fig:drift_users_01_3}
%         \end{subfigure}
%         \hfill
        
%         \centering
%         \begin{subfigure}[b]{.9\columnwidth}
%             \includegraphics[width=\columnwidth]{figs/new_version/curves/user01_svm_drift_es2.pdf}
%             \caption{Accuracy curve.}
%             \label{fig:drift_users_01_curve}
%         \end{subfigure}
%     \end{minipage}
%     \caption{\hl{User 01 SOM images and classification curves for experimental scenario 2 provided contrasting conclusions about presence of concept drift in usage profiles}.}
%     \label{fig:drift_users_01}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figs/new_version/unable_identify_drift.pdf}
%     \caption{SOM images and classification curves that provided contrasting conclusions about presence of concept drift in usage profiles. \hl{To do: improve the quality of the figure}}
%     \label{fig:unable_identify_drift}
% \end{figure}




==> OLD/ack.tex <==
We thank our study participants. We also thank the anonymous reviewers for their detailed and insightful feedback. \hl{This work was supported (in part) by <include>}.

==> OLD/availability.tex <==
Our de-identified computer usage dataset and profile extracting tool are publicly available at: <link> (to be included upon paper acceptance).




==> OLD/diss.tex <==

\subsection{Summary and Findings}
\subsubsection{User Classification}
% Do computer users have unique computer usage profiles which can be leveraged to successfully distinguish them from other users? Our research answers through addressing these following questions: (i) Do computer users behave routinely different in their daily computer usage activities? (ii) Can these differences be reliably learned using machine learning methods? (iii) How long period do we need to reliably recognize computer users?  

Our research answers validate our assumption from the following three aspects:(i) the existence of identifiable difference among different users (ii) the reliably of learned using machine (iii) the period do we need to reliably recognize computer users.

Our research confirms our hypothesis that computer users do behave differently in their computer usage activities. According to Figure~\ref{fig:som_users} generated with Self Organization Map (SOM), the users exhibit their preference in using the computer.  

Using BA-LSTM, RF-V and SVM, our research demonstrates that the differences among users can be reliably learned using machine learning methods. All the machine learning methods successfully distinguish the different users. Given enough information, the accuracy of the classifiers would reach 90\% with 18 users. These three different classifiers show both similarities and discrepancies. On the one hand, the accuracy shift in a similar trend among the three classifiers; the accuracy increases as the windows length increases and decreases when more users are required to be distinguished. Both the trend on the accuracy change come close to a stop as length of the windows or number of users increases. On the other hand, the accuracy ratios of the different machine learning methods show some differences. BA-LSTM is the most accurate classifier among the three when window length at 5-10 minutes and has low Standard Deviation (STD). RF-V has the highest average accuracy on most window length and number of users in each group. The STD of RF-V remains close to that of BA-LSTM. SVM holds the highest accuracy in the most extreme case where 50 minutes of window are used; the STD of SVM, however, is also higher than the other two classifiers.

% With our evaluation results on BA-LSTM, RF-V and SVM, we could draw the conclusion that longer periods produce preciser classification results. However, this conclusion contradicts with the target of authentication where time need to authenticate an user should be minimized. Thus, in balance of these two contradictory requirements, windows of X-minute(remain to be discussed) of data would be ideal for our current solution.

Although the evaluation results shows that windows of longer length could improve the accuracy of the classifiers, the authentication task requires us to react in a short period of time. Balancing the detection accuracy and reaction time, we consider the window of five minutes would be the sweet spot for our proposed user profiling framework. One the one hand, the classifiers could reach the detection accuracy at 90\% using five minute windows, while further increase of the window length would lead to limited gain in accuracy. On the other hand, five minutes could still be fast enough for authentication tasks.

\subsubsection{Concept Drift on User Behavior}

Concept drift is the situation where the relation between the input data and the target variable changes over time~\cite{Gama2014SCD}. We explore the degree where user behaviors are maintained during the weeks visually, evidencing the presence of concept drifts in our data. To visualize the weekly computer using activities of each participants, we divided each user data in three sets, containing their behaviors for weeks one, two and three, and trained one SOM for each of the weeks with the same parameters as the SOM for the first week. Almost every participants display the sign of variation in their weekly behavior, but the degree of variation different from one participants to another. Figure~\ref{fig:som_week_04} shows very similar behaviors for user four during the tree weeks of the data collected, since there is a common pattern in all figures. On the other hand, when we see Figure~\ref{fig:som_week_06}, user six figures by week indicate that there is a change of concept in his behaviors, since they are very 
different from each other. 

% \begin{figure}

% \begin{multicols}{3}
%     \centering
%     \subcaptionbox{Week 1.\label{fig:user_0401}}[\linewidth][c]{
%     \includegraphics[width=.14\textwidth]{figs/users_week/0401.png}}\par
%     \subcaptionbox{Week 2.\label{fig:user_0402}}[\linewidth][c]{
%     \includegraphics[width=.14\textwidth]{figs/users_week/0402.png}}\par
%     \subcaptionbox{Week 3.\label{fig:user_0403}}[\linewidth][c]{
%     \includegraphics[width=.14\textwidth]{figs/users_week/0403.png}}\par 
% \end{multicols}
% \caption{User 4 (12007) U-matrices for each week indicate that his behavior is very similar as time goes by: figures have a common pattern.}

% \label{fig:som_week_04}
% \end{figure}

% \ToDo{TODO: Different behaviors by week for user 6 in Figure~\ref{fig:som_week_06}.}

% \begin{figure}

% \begin{multicols}{3}
%     \centering
%     \subcaptionbox{Week 1.\label{fig:user_0601}}[\linewidth][c]{
%     \includegraphics[width=.14\textwidth]{figs/users_week/0601.png}}\par
%     \subcaptionbox{Week 2.\label{fig:user_0602}}[\linewidth][c]{
%     \includegraphics[width=.14\textwidth]{figs/users_week/0602.png}}\par
%     \subcaptionbox{Week 3.\label{fig:user_0603}}[\linewidth][c]{
%     \includegraphics[width=.14\textwidth]{figs/users_week/0603.png}}\par 
% \end{multicols}
% \caption{User 6 (11011) U-matrices for each week indicate that his behavior changes a lot as time goes by, problem known as concept drift.}

% \label{fig:som_week_06}

% \end{figure}

\begin{figure}

\begin{multicols}{3}
    \centering
    \subcaptionbox{User 3, week 1.\label{fig:user_0301}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/0301.png}}\par
    \subcaptionbox{User 3, week 2.\label{fig:user_0302}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/0302.png}}\par
    \subcaptionbox{User 3, week 3.\label{fig:user_0303}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/0303.png}}\par
\end{multicols}

\begin{multicols}{3}
    \centering
    \subcaptionbox{User 7, week 1.\label{fig:user_0701}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/0701.png}}\par
    \subcaptionbox{User 7, week 2.\label{fig:user_0702}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/0702.png}}\par
    \subcaptionbox{User 7, week 3.\label{fig:user_0703}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/0703.png}}\par
\end{multicols}

\begin{multicols}{3}
    \centering
    \subcaptionbox{User 16, week 1.\label{fig:user_1601}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/1601.png}}\par
    \subcaptionbox{User 16, week 2.\label{fig:user_1602}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/1602.png}}\par
    \subcaptionbox{User 16, week 3.\label{fig:user_1603}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/1603.png}}\par
\end{multicols}

\caption{Good users.}

\label{fig:good_users}

\end{figure}

\begin{figure}

\begin{multicols}{3}
    \centering
    \subcaptionbox{User 5, week 1.\label{fig:user_0501}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/0501.png}}\par
    \subcaptionbox{User 5, week 2.\label{fig:user_0502}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/0502.png}}\par
    \subcaptionbox{User 5, week 3.\label{fig:user_0503}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/0503.png}}\par
\end{multicols}

\begin{multicols}{3}
    \centering
    \subcaptionbox{User 6, week 1.\label{fig:user_0601}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/0601.png}}\par
    \subcaptionbox{User 6, week 2.\label{fig:user_0602}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/0602.png}}\par
    \subcaptionbox{User 6, week 3.\label{fig:user_0603}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/0603.png}}\par
\end{multicols}

\begin{multicols}{3}
    \centering
    \subcaptionbox{User 13, week 1.\label{fig:user_1301}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/1301.png}}\par
    \subcaptionbox{User 13, week 2.\label{fig:user_1302}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/1302.png}}\par
    \subcaptionbox{User 13, week 3.\label{fig:user_1303}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/1303.png}}\par
\end{multicols}

\caption{Bad users.}

\label{fig:bad_users}

\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figs/confusion_matrix_svm_crop.pdf}
    \caption{SVM confusion matrix.}
    \label{fig:confusion_matrix_svm}
\end{figure}


Drift Detection Method (DDM) \cite{gama2004} and Early Drift Detection Method (EDDM) \cite{baena2006} are the two most popular drift detectors found in the literature and
both are online supervised methods based on sequencial error (prequential) monitoring (i.e., if any classifier starts to miss classify in sequence, it means that something is changing
-- change of concept), which could be used to handle concept drift in users behaviours. 

\ToDo{Address the relation between concept drift and classification accuracy}

% \subsubsection{Computer Left Unused}

% A common situation that we witnessed in the 

% Unused minutes are the time where users left their computer unused. Unused minute is one of the problems we find during our research. Besides the occasions where the participants left their computer unused for a short period of time, we also observes that many participants would left their computer on for whole night. 

% In our evaluation, we found that our machine learning methods yield significantly lower accuracy on three specific users. 
% % According to figure~\ref{fig:conf_matrix}, these three users confused the classifier and lower the average classification accuracy. To find out the cause of the confusion, we analyzed the vector of the minutes where the classifier failed to distinguish and compare the activities with the other computer users.

% Our analysis reveals that the problem lies in the activities records of the minutes where the computer was left idle. Compared with other users, these three users have more idle minutes collected as they tend to left their computer on over night. These three users have idle minute ratios at 33\%, 25\% and 13\% respectively, which are generally higher than the rest users. This results in generating minutes of records with few and similar, if not the same, process and network activities.

% There are a few of solutions to this issue. \ToDo{The solution of the problem}

\subsection{Strength and Limitation}

Our research present a pioneering user profiling framework that creates a multi-dimensional digital user signature based on various system level information and across different layers of abstractions.

We designed and implemented a kernel mode extractor that is transparent to the computer users. On the one hand, operating system keeps the kernel mode extraction system relatively secure and blind to the user. On the other hand, this extraction system has barely noticeable overhead. These features not only increase the usability of our system, but also fulfill the requirements of continuous authentication systems.

In our research, we conducted an ecologically-valid user study using our extraction system. In this study, we collected complicated computer usage information for a relatively long period from participants with different habits. we enrolled both male and female computer users (10 male v.s. 8 female). Among all the participants, we have 7 light computer users, 9 routine computer users and 2 heavy computer users. This user study also guides us in both improving  the usability of data extraction system and simplifying its installation process.

To evaluate our profile method, we experimented comprehensively on multiple machine learning and deep learning methods for user profiling. In our experiments, we intentionally compared multiple categories of machine learning methods: deep learning (BA-LSTM, SOM) vs. traditional machine learning (SVM and Random Forest) and supervised (BA-LSTM, SVM, Random Forest) vs unsupervised (SOM). In conclusion, both the deep learning and machine learning show promising results (up to 98.3\% of accuracy) in classification tasks at distinguishing different users. Although SOM does not produce any prediction, the generated figures proves visually that there are sufficient opportunities for unsupervised methods to generate accurate computer user profiles.

Our research could open a new horizon for continuous authentication. To our best knowledge, this is the first work that seek to profile the user using kernel level information on PC. Our framework adopts kernel based design; thus provides protection against tampering from malware. It exploits human behaviors across different abstraction layers of the computer system to avoid missing any traits of abnormal behaviors. 

% Our research explore a novel method to profile the computer user. We use per-minute process and network activities of the computer users. This differ us from behavioral biometric methods~\cite{Neal2015MDABWUD} that uses long periods (e.g. half a day) of process and network activities and also enable our system to timely respond to abnormal cases. 

% A strength of our research is our join efforts with the psychology department. Using the feedback from 

% Our sample covers various types of computer users. In the user study, we enrolled almost equal number of male and female computer users (10 v.s. 8). Among all the participants, we have 7 light computer users, 9 routine computer users and 2 heavy computer users. The diversity of the participants allows the exploration on the effects of these difference on our profiling method.

Due to the complication of our user study, we have only recruited 18 participants in our user study. The lack of abundant computer usage data from the participants restricts our capability to further exploit how the relation between accuracy and number of user in groups. Also, for certain long-term research targets, e.g., concept drift, that requires months of study of the users, the data acquired from previous user study remains too short. According to the lesson we learned, we preparing for another longer period of user study with more categories of users.

% \subsubsection{Data Collection}
As our current study focus on evaluating the feasibility of our personalized human centric computer usage profile system, we did not include the effects of malware in our current study. In the future, the detection of malware and its effect on alternating normal user behavior will be of our major research points.

\subsection{Recommendation}
Our research could also shed some light on how different deep learning and machine learning methods perform on profile computer users on with their computer usage activities. Also, we envision how a new generation of deep learning method: adversarial learning, could help with this problem.
%Based on our evaluation on BA-LSTM, SVM and RF-V, we would provide the following recommendation.

\subsubsection{BA-LSTM}
\ToDo{Discuss methods pros and cons (and use their results).}


\subsubsection{SVM}

SVM is an ideal machine learning classifier for our profiling problem. SVM can be easily implemented with or without machine learning package. Although SVM needs grid search to find its best parameters, the training on SGD based SVM requires less than 20 minutes to complete. SGD based SVM also retains the capability of updating the model later. Compared with BA-LSTM, SVM remains simple in design and implementation with little performance decrease than BA-LSTM. Compared with RF, SVM has better accuracy and requires less computational resource. SVM remains a good solution for user profiling with network and process information. It well balances the efficiency and accuracy while capable of model retraining. These features make SVM ideal where the user models are frequently updated.

\subsubsection{RF-V}

\ToDo{Fabricio: please discuss methods pros and cons (and use their results).}

Random Forrest 
% The main difference compared to the standard sliding window mechanism is that we do not need to train a new classifier when we change the window size. We just train a single model with every minute individually and change the size of our window in the prediction phase. Consequently, the memory usage is lower since we do not concatenate columns and use only the original data. In addition, it is possible to change the window size on the fly, advancing the prediction in relation to the sliding window mechanism, since the method will require always the same amount of minutes to predict.

% \ToDo{- Best overall accuracy per group when using all users (18)}
\subsubsection{SOM}



\subsubsection{Adversarial Learning}
\ToDo{Heng: please briefly discuss the advantages and challenges of adversarial learning}
Adversarial attacks come in many different forms. One classic example is attacks in image classifier, where carefully designed "noise" is added to the test image, such that the image would looks the same to the human eyes, but will trick the trained classifier. (A example can be found on \url{https://blog.openai.com/adversarial-example-research/}).
The key point is to minimize the amplitude of the noise so it won't be detected by eyes but still enough to trick the classifier. In our application, the attackers would aim for "Getting the job done" without alarming the detection system. "Getting the job done" means some of the features will definitely be "1" in the feature vector. So even though the goal is to trick the classifier in these two scenarios, they have different restrictions, leading to different attack/defend methods.


==> OLD/eval.tex <==


This section  describes the results of the machine learning analysis and to what extent the profiles are consistent over time. The goal of the analysis was to determine whether users exhibit unique behavior-based computer usage profiles. The goal was  not to compare  performance of different machine learning methods.  Therefore, we did not control for performance of each machine learning classifier running on identical machines and in identical environments.

Performance of the classifiers was measured as standard classification tasks and specifically as,  how accurately they classified to which user a window of observation belonged. We tested our classifiers with different user group sizes (i.e., 3, 5, 7, 10 and 18 users), with users randomly assigned to these different group sizes. For each group size, we analyzed classification accuracy for each of the following  window sizes: 1, 2, 5, 10, 15, and 50 minutes. \\

\noindent
{\bf Training.} We trained the classifiers with data collected from the first two weeks of the study period (approximately 2/3 of  each participant's data) and used the last week of collected data (approximately 1/3 of the dataset) for testing. For BA-LSTM and SVM, whose training procedures use non-linear optimization algorithms, 10\% of the training set was separated as validation set~\cite{bishop1995neural} to avoid overfitting. Random Forest-V, however, does not require a validation test because it is less prone to overfitting~\cite{Breiman2001RF}. 
%The training and testing sets were not chosen randomly because we used sliding window with stride of one minute in the pre-processing of the data. 
% , and random selecting will introduce almost identical data across training and testing sets. This setup also simulates the real use cases of profiling where user behaviors are first modeled and then used to identify the user. 
All values in the feature vectors were normalized using min-max normalization, which scales every feature into an interval between 0 and 1~\cite{Gron:2017:HML:3153997}.

We did not employ k-fold cross-validation because of the  temporal nature of our data. 
%K-fold validation basically extends the training time k times 
For a temporal dataset such as ours, where the behavior of the user might slightly change week by week (concept-drift),  behaviors from the future cannot be mixed with behaviors from the past~\cite{DBLP:journals/corr/abs-1807-07838, gregioIEEEBrazil18}. Therefore, k-fold cross-validation was not applicable. 

% BA-LSTM: The BA-LSTM classifier was trained in small batches with batch size of 32 in each iteration. The training process was evaluated on validation set for every 1000 iterations. During the training, the classifier with maximum accuracy on validation set was maintained. The training step would stop if the maximum accuracy was not surpassed after 5 more evaluations.

% SVM: The SVM classifier was trained with the training set while the accuracy on the validation set is evaluated after each iteration. During the training, the classifier with maximum accuracy on the validation set was maintained. The training would stop if the maximum accuracy on are not surpassed by after 8 more iterations.

% RF-V: The Random Forest is trained with the same random seed (to always generate the same trees) and 500 estimators (which was the best parameter found using grid search). 

We trained a different SOM for each user, since each neural network generates a different representation. For training  we used computer usage data from all 21 days for all participants,  leading to a $100\times100$ hexagonal grid of neurons. The network was trained for 30 epochs and its neurons were initialized with Principal Component Analysis (PCA) projections. 

% since each neural network will generate a different representation. We used all the 21-day computer usage activity records of each user to train these networks, which is composed by a $100\times100$ hexagonal grid of neurons. We train the network for 30 epochs and its neurons are initialized with PCA (Principal Component Analysis) projections. 


\subsection{Classification}

{\bf BA-LSTM}. The classifier was implemented  with Tensorflow~\cite{tensorflow2015-whitepaper} and experiments ran on 3 Nvidia K80 GPUs. Table~\ref{tabacclstm} presents the classification accuracy for the test set.  

\begin{table}[hbtp]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 & 3 users & 7 users & 10 users & 18 users & \begin{tabular}[c]{@{}c@{}}Avg. across\\ Window Sizes\end{tabular} \\ \hline
1 min & 96\% & 91.5\% & 90.6\% & 88.2\% & 91.6\% \\ \hline
2 min & 96.3\% & 92\% & 90.9\% & 88.9\% & 92\% \\ \hline
5 min & 96.8\% & 92.5\% & 91.5\% & 89.6\% & 92.6\% \\ \hline
10 min & 97\% & 92.4\% & 92.2\% & 90.1\% & 92.9\% \\ \hline
15 min & 97.2\% & 92.5\% & 92.5\% & 90.6\% & 93.2\% \\ \hline
50 min & 98.3\% & 93.3\% & 93.6\% & 90.8\% & 94\% \\ \hline
\begin{tabular}[c]{@{}c@{}}Avg. across\\ Group Sizes\end{tabular} & 96.9\% & 92.4\% & 91.9\% & 89.7\% & - \\ \hline
\end{tabular}
}
\caption{Classification accuracy for different user group sizes and different observation windows for BA-LSTM.}
\label{tabacclstm}
\end{table}

%\subsection{SVM}

%We evaluate two types of SVM on user profiling: linear SVM and kernel SVM
{\bf SVM}. We implemented a linear SVM classifier on one-versus-rest configuration with the scikit Learn Stochastic Gradient Descent (SGD) classifier tool kit~\cite{scikit-learn}  
%Compared with other SVM solutions, SGD-based SVM uses stochastic gradient descent learning method to optimize the classifier. Compared SGD with traditional methods with quadratic programming solution, the classifier for SGD based SVM can be trained through multiple steps. This feature not only reduces the memory used in training, but also enables retraining the model if user behaviors change substantially. Also, SGD optimization generates classifier with minor differences in their accuracy. For each configuration, we generated three classifiers and used their average accuracy rates as results. 
and ran experiments on a Xeon E5-2695 machine with 128 GB  memory. Each classifier was trained with 20-40 iterations until  it converged (i.e., accuracy stopped increasing). Table~\ref{tab:svm_acc} presents the results.


% \begin{figure}
%     \centering
%     % \includegraphics[width=0.45\textwidth]{figs/SVM_accuracy.pdf}
%     \includegraphics[width=0.45\textwidth]{figs/chart_svm.pdf}
%     \caption{Testing set accuracy results of classification for different sizes of groups of subjects and different window of classification sizes for SVM.}
%     \label{fig:svm_acc}
% \end{figure}


\begin{table}[hbtp]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 & 3 Users & 7 Users & 10 Users & 18 Users & \begin{tabular}[c]{@{}c@{}}Avg. across\\ Window Sizes\end{tabular} \\ \hline
1 min & 93.73\% & 89.72\% & 88.78\% & 87.12\% & 89.84\% \\ \hline
2 min & 94.86\% & 90.22\% & 89.31\% & 87.64\% & 90.51\% \\ \hline
5 min & 95.42\% & 90.25\% & 90.26\% & 87.64\% & 90.89\% \\ \hline
10 min & 96\% & 92.08\% & 91.58\% & 88.53\% & 92.05\% \\ \hline
15 min & 96.30\% & 93.40\% & 92.44\% & 89.06\% & 92.80\% \\ \hline
50 min & 97.92\% & 94.91\% & 94.05\% & 91.80\% & 94.67\% \\ \hline
\begin{tabular}[c]{@{}c@{}}Avg. across\\ Group Sizes\end{tabular} & 95.71\% & 91.76\% & 91.07\% & 88.63\% & - \\ \hline
\end{tabular}
}
\caption{Classification accuracy for different user group sizes and different observation windows for SVM.}
\label{tab:svm_acc}
\end{table}

% Similar to BA-LSTM results, the accuracy of the model increases as the windows of observation increases.  The accuracy for classification decreases, however, as more users are included in each group. 
%Each row of Table~\ref{fig:svm_acc} reflects this phenomenon. According to the results, the accuracy drop becomes less intensive. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figs/users_som/01.pdf}
%     \caption{User 1 component plane representation.}
%     \label{fig:network_coverage}
% \end{figure}


%\subsection{RF-V}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figs/voting.pdf}
%     \caption{Voting mechanism.}
%     \label{fig:voting}
% \end{figure}


{\bf Random Forest-V}. The classifier was implemented with scikit-learn~\cite{scikit-learn} and  experiments ran on a Xeon E5-2620 machine with 64GB of memory.  Table~\ref{tab:rf_acc} presents the results.


\begin{table}[hbtp]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 & 3 Users & 7 Users & 10 Users & 18 Users & \begin{tabular}[c]{@{}c@{}}Avg. across\\ Window Sizes\end{tabular} \\ \hline
1 min & 96.30\% & 90.18\% & 90.84\% & 88.92\% & 91.56\% \\ \hline
2 min & 96.31\% & 90.18\% & 90.91\% & 88.94\% & 91.59\% \\ \hline
5 min & 96.59\% & 90.56\% & 91.33\% & 89.49\% & 91.99\% \\ \hline
10 min & 96.96\% & 90.97\% & 91.80\% & 90.06\% & 92.45\% \\ \hline
15 min & 97.08\% & 91.14\% & 92.05\% & 90.32\% & 92.65\% \\ \hline
50 min & 97.51\% & 91.57\% & 92.50\% & 90.98\% & 93.14\% \\ \hline
\begin{tabular}[c]{@{}c@{}}Avg. across\\ Group Sizes\end{tabular} & 96.79\% & 90.77\% & 91.57\% & 89.79\% & - \\ \hline
\end{tabular}
}
\caption{Classification accuracy for different user group sizes and different observation windows for Random Forest-V.}
\label{tab:rf_acc}
\end{table}

As shown in Tables \ref{tabacclstm}-\ref{tab:rf_acc}, classification accuracy was consistent across machine learning methods, with an accuracy of over 90\% for all methods and user group sizes when the observation windows were greater than 10 minutes. Accuracy for  group size increased as a function of increasing the observation window. However, accuracy decreased as a function of increasing user group size across all observation windows.


% \subsection{Data Extraction Overhead}

% We also analyzed the overhead introduced by our data extractor using three popular benchmarks each measuring different category of computer performance. 
% \begin{itemize}
%     \item PC mark~\cite{pcmark10} simulates the modern office workload including users performing web browsing, document work, skype meeting, digital content creation and etc.
%     \item Cinebench~\cite{maxon_cinebench} is a CPU intensive benchmark using graphic rendering workload. 
%     \item CrystalDiskMark~\cite{crystaldiskmark} is an I/O intensive benchmark measuring the disk performance via measuring the speed on file read and write.
% \end{itemize}
%  %Cinebench\cite{maxon_cinebench} is a CPU intensive benchmark using graphic rendering workload. CrystalDiskMark\cite{crystaldiskmark} is an I/O intensive benchmark measuring the disk performance via measuring the speed on file read and write.

% To identify the overhead of each sub-component of the extractor, we conduct the experiments with different configuration of the the extractor:(i) no extractor, (iii) fully functional extractor, (iii) extractor only collecting processes event, and (iv) extractor only collecting network information. In the overhead evaluation, we use the results form the system without the extractor as standard score. The tests are conducted on a Windows 10 laptop with dual core i7-7Y75, 16GB of RAM and 256GB solid state drive. The test results are shown in Figure~\ref{fig:perf}. Our tests demonstrate that the performance overhead was negligible (less than 5\%). 

% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{figs/performance_loss.pdf}%\vspace{-0.25in}
% \caption{Performance evaluation of extractor. Results for various benchmarks. Labels - Without data extractor = System with Windows OS 10 without the extractor; Full data extractor = Full version of the extractor; Process monitor = Extractor capturing process-related information only; Network monitor= Extractor capturing network-related information only.} 
% \label{fig:perf}
% \end{figure}


\subsection{Self-Organizing Maps}

SOM was implemented with Python module \textit{somoclu}~\cite{somoclu} and  experiments ran on a Xeon E5-2620 machine with 64 GB of memory. Figure~\ref{fig:som_users} shows the SOM  images for all 18 participants across the 21-day study period. 
%SOM creates similarity clusters that reflect the attribute relationship of the input data. 
In our case, similar computer usage activities lead to patterns of similar shape in SOM images. The observed distinctive image patterns in the SOM-generated figures per participant suggested unique usage profiles.


\begin{figure*}[htb]
\begin{multicols}{6}
    \centering
    \subcaptionbox{User 1\label{fig:user_01}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_som/01.png}}\par
    \subcaptionbox{User 2\label{fig:user_02}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_som/02.png}}\par
    \subcaptionbox{User 3\label{fig:user_03}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_som/03.png}}\par 
    \subcaptionbox{User 4\label{fig:user_04}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_som/04.png}}\par 
    \subcaptionbox{User 5\label{fig:user_05}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_som/05.png}}\par 
    \subcaptionbox{User 6\label{fig:user_06}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_som/06.png}}\par 
\end{multicols}
\begin{multicols}{6}
    \subcaptionbox{User 7\label{fig:user_07}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_som/07.png}}\par
    \subcaptionbox{User 8\label{fig:user_08}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_som/08.png}}\par
    \subcaptionbox{User 9\label{fig:user_09}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_som/09.png}}\par 
    \subcaptionbox{User 10\label{fig:user_10}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_som/10.png}}\par 
    \subcaptionbox{User 11\label{fig:user_11}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_som/11.png}}\par 
    \subcaptionbox{User 12\label{fig:user_12}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_som/12.png}}\par 
\end{multicols}
\begin{multicols}{6}
    \subcaptionbox{User 13\label{fig:user_13}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_som/13.png}}\par
    \subcaptionbox{User 14\label{fig:user_14}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_som/14.png}}\par
    \subcaptionbox{User 15\label{fig:user_15}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_som/15.png}}\par 
    \subcaptionbox{User 16\label{fig:user_16}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_som/16.png}}\par 
    \subcaptionbox{User 17\label{fig:user_17}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_som/17.png}}\par 
    \subcaptionbox{User 18\label{fig:user_18}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_som/18.png}}\par 
\end{multicols}
\caption{U-matrix representations extracted from SOM based on training data  collected in our user study. Representations suggests that usage profiles are unique.}
\label{fig:som_users}
\end{figure*}




%Concept drift is a phenomenon in which the relation between the input data and the classification class (e.g., in our case the data belonging to the user) changes over time \cite{Gama2014SCD}. An example of concept drift in our context are natural and benign changes in the user profile, e.g.,  travel and change of responsibilities within the organization. Concept drift can adversely  affect classification accuracy because the training data becomes obsolete.


\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figs/confusion_matrix_svm_crop.pdf}
    \caption{SVM confusion matrix using a window size of 50 minutes.}
    \label{fig:confusion_matrix_svm}
\end{figure}

SOM also allowed determination of concept drift in the user data. Concept drift is a phenomenon in which the relation between the input data and the classification class (e.g., in our case the data of a specific user) changes over time \cite{Gama2014SCD}. An example of concept drift in our context are natural and benign changes in the user profile, e.g., related to travel and change of responsibilities within the organization. Concept drift can adversely  affect classification accuracy because the training data becomes obsolete.

To explore concept shift, we compared user profiles which were based on almost 100\% classification accuracy with  profiles which were based on a lower classification accuracy (< 85\%). Figure \ref{fig:confusion_matrix_svm} illustrates our confusion matrix (for SVM \footnote{The other classification methods presented comparable results.}), where the x-axis represents the predicted label for a user profile (from the classifier) and the y-axis represents the true label. Users are identified by the labels 1 to 18. The matrix shows that the classifier resulted in almost 100\% classification accuracy for Users 3, 7, and 16. It resulted in less than 85\% classification accuracy for Users 5, 6, and 13.  Figures~\ref{fig:good_users} and~\ref{fig:bad_users} present the SOM images for User 7 (high classification accuracy) and User 6 (low classification accuracy) \footnote{Due to space limitations, weekly SOM images for all users are shown in the Appendix.} per week in the study to exemplify the observed concept drift. In particular, these visual depictions suggest that concept drift existed for all users, but was more pronounced for users whose profiles had  lower classification accuracy (e.g., User 6).  While other reasons (e.g., natural similarities between usage profiles) may explain the difficulty the classifiers had with identification of some  profiles, our data highlights that the next generation of continuous authentication tools need to consider concept drift to be effective.


\begin{figure} [htb]

% \begin{multicols}{3}
%     \centering
%     \subcaptionbox{User 3, week 1.\label{fig:user_0301}}[\linewidth][c]{
%     \includegraphics[width=.14\textwidth]{figs/users_week/0301.png}}\par
%     \subcaptionbox{User 3, week 2.\label{fig:user_0302}}[\linewidth][c]{
%     \includegraphics[width=.14\textwidth]{figs/users_week/0302.png}}\par
%     \subcaptionbox{User 3, week 3.\label{fig:user_0303}}[\linewidth][c]{
%     \includegraphics[width=.14\textwidth]{figs/users_week/0303.png}}\par
% \end{multicols}

\begin{multicols}{3}
    \centering
    \subcaptionbox{User 7, week 1.\label{fig:user_0701}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/0701.png}}\par
    \subcaptionbox{User 7, week 2.\label{fig:user_0702}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/0702.png}}\par
    \subcaptionbox{User 7, week 3.\label{fig:user_0703}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/0703.png}}\par
\end{multicols}

% \begin{multicols}{3}
%     \centering
%     \subcaptionbox{User 16, week 1.\label{fig:user_1601}}[\linewidth][c]{
%     \includegraphics[width=.14\textwidth]{figs/users_week/1601.png}}\par
%     \subcaptionbox{User 16, week 2.\label{fig:user_1602}}[\linewidth][c]{
%     \includegraphics[width=.14\textwidth]{figs/users_week/1602.png}}\par
%     \subcaptionbox{User 16, week 3.\label{fig:user_1603}}[\linewidth][c]{
%     \includegraphics[width=.14\textwidth]{figs/users_week/1603.png}}\par
% \end{multicols}

\caption{SOM images, week-by-week, for User 7, with almost 100\% classification accuracy.}
\label{fig:good_users}
\end{figure}

\begin{figure}
% \begin{multicols}{3}
%     \centering
%     \subcaptionbox{User 5, week 1.\label{fig:user_0501}}[\linewidth][c]{
%     \includegraphics[width=.14\textwidth]{figs/users_week/0501.png}}\par
%     \subcaptionbox{User 5, week 2.\label{fig:user_0502}}[\linewidth][c]{
%     \includegraphics[width=.14\textwidth]{figs/users_week/0502.png}}\par
%     \subcaptionbox{User 5, week 3.\label{fig:user_0503}}[\linewidth][c]{
%     \includegraphics[width=.14\textwidth]{figs/users_week/0503.png}}\par
% \end{multicols}

\begin{multicols}{3}
    \centering
    \subcaptionbox{User 6, week 1.\label{fig:user_0601}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/0601.png}}\par
    \subcaptionbox{User 6, week 2.\label{fig:user_0602}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/0602.png}}\par
    \subcaptionbox{User 6, week 3.\label{fig:user_0603}}[\linewidth][c]{
    \includegraphics[width=.14\textwidth]{figs/users_week/0603.png}}\par
\end{multicols}

% \begin{multicols}{3}
%     \centering
%     \subcaptionbox{User 13, week 1.\label{fig:user_1301}}[\linewidth][c]{
%     \includegraphics[width=.14\textwidth]{figs/users_week/1301.png}}\par
%     \subcaptionbox{User 13, week 2.\label{fig:user_1302}}[\linewidth][c]{
%     \includegraphics[width=.14\textwidth]{figs/users_week/1302.png}}\par
%     \subcaptionbox{User 13, week 3.\label{fig:user_1303}}[\linewidth][c]{
%     \includegraphics[width=.14\textwidth]{figs/users_week/1303.png}}\par
% \end{multicols}

\caption{SOM images, week-by-week, for User 6 with less than 85\% classification accuracy.}
\label{fig:bad_users}
\end{figure}



\subsection{Discussion: Summary, Limitations, and Lessons}

We used machine learning methods to test the hypothesis that unique computer usage profiles exist. We also explored in this context, whether such profiles exhibited temporal consistency.    %We propose that these unique user profiles could be efficiently for the development of the next generation of  human-centric,  behavioral-based continuous authentication tools. 
We conducted  an ecologically-valid user study to collect  behavior-based computer usage data from  participants  over a period of 21 days. We applied three distinct machine learning methods to demonstrate robustness of  our findings. Our work suggests that H1 (a) cross-layer, user computer behavior-based profiles are feasible for application in continuous authentication tools, and H1(b) most profiles are temporal consistent, even though we observed concept drift for some users. 

%Our results provide indication that such unique profiles do exist. All machine learning methods provided consistent results with classification accuracy reaching over 90\%  for all groups of users for windows of observation longer than 10 minutes. 


 The classification accuracy decreased with the increase in user group size. For example, for BA-LSTM the accuracy dropped 8\% on average for 50-minute windows when considering 18 compared to 3  users. However, dropped accuracy appeared to converge,  as  the number of users in a group increased. From example, for both a group size increase from 7 to 18 users and a group size increase from 10 to 18 users,  the accuracy (50-minute window, BA-LSTM) dropped approximately 3\%. More research with a larger and more diverse sample is needed to confirm  this trend. Nevertheless, these first findings suggest that the increase in the number of users in a group (e.g., employees in a  corporation) may affect classification accuracy. Also, some users might have naturally similar profiles, which  may pose challenges to  classification. We advocate  the use of a larger and more diverse number of computer usage features, taken from all layers of abstraction that make up a computer system as a way to optimize unique usage profile classification. 

Our  results indicate that continuous authentication tools should primarily be used to distinguish users profiles against anomalies (e.g., Mary using a corporate device vs. an imposter or an APT), rather than differentiating among various users profiles.

%and not to distinguish which user is associated with  a particular computer activity. This angle can potentially be the most suitable for practical and effective applications of continuous authentication tools. 

Our analysis was based on the assumption that user’s systems were not compromised by malware during the 21-day data collection. Presence of malware in the user’s machine during collection of training data can adversely affect the learning models, as malicious behaviors would be considered part of the usage profile. 

One challenge of leveraging computer usage profiles in continuous authentication tools is that the recording and determination of user profiles can be perceived as a {\bf privacy-invasive}. To address this concern,  profile extractors should operate without recording  personally identifiable information, file contents, or keys typed by the user. 
%The extractor presented in this study operates in such manner. 
Nevertheless, some users might still feel uncomfortable with having their system events being recorded. However,  in corporate environments, expectations of privacy are nearly nonexistent. Often, employees are  fully aware that nearly all their  activities inside the organization perimeter are monitored and recorded. For example, many organizations have their employees agree on usage policies, such as  that  corporate email is to be used only for business purposes and that  employers have the right to monitor employees' email and computer usage \cite{privacy}. 


User profiles might change with time ({\bf concept drift}) and we observed such phenomenon for some users in our sample. While concept drift presents challenges for machine learning classification, the literature discusses methods to handle it: Drift Detection Method (DDM) \cite{gama2004} and Early Drift Detection Method (EDDM) \cite{baena2006}. These are online supervised methods based on sequential error monitoring (i.e., if a classifier starts misclassifying, this might be an indication of concept drift), which could be used to early detect and counter concept drift. Another approach is to employ user assistance.
%in the model about changes in profile and need of retraining.
For example, upon changing responsibilities in an organization, an employee might configure (or request an administrator to configure) a need to retrain his profile. 

Our analysis also operated on the assumption that the collected training data was generated from the natural computer usage behavior of the user. The training data collection  can be tampered with  {\bf adversarial examples} \cite{christian2013DBLP}. For instance, during training, a user could craft noise to confuse the classifier in a semi-honest (e.g., to protect privacy) or malicious way (e.g., to disguise actions as a malicious insider). As the current version of the profile extractor uses plain text files to store logs, the data in the log files can also be tampered by the user before they are uploaded onto the server.

Without constant access to the internet, the profile extractor generates logs offline and uploads all of them to the server when an active internet connection is found. This may burden the CPU and network on rare occasions such as when a user has generated huge amounts of log files while being offline, and then connect to the internet.

The tasks scheduled on Windows, such as a scheduled Dropbox sync, are not differentiated from the tasks explicitly opened by the user. All such tasks are counted toward user activity and cannot be a distinguishing factor when an adversary uses this system.

Some limitations are caused by the restrictions set by the operating system. For example, Windows kernel callbacks provide capabilities only for capturing destination IPs. The destination hostnames are resolved later using reverse DNS lookups. These reverse lookups are not always successful, and also may not always return the exact domain name.


Our results suggest that behavior-based continuous authentication is feasible in that users do exhibit, in general, distinct and distinguishable computer usage profiles, which repeat weekly. %While  continuous authentication systems are promising in profiling users, they should always be part of a multi-factor authentication and anomaly-detection framework inside organizations, which should also include traditional mechanisms such as passwords and anti-malware solutions. 
Such tools can complement traditional security solutions  (e.g., passwords, anti-malware solutions) in corporate environments and represent a game-changer to flag stealthy, long-duration attacks, such as insider attacks, APTs, and intruders. 

In sum, we recommend (i) the use of cross-layer, fine-grained, hyper-dimensional computer events recorded in a continuous fashion, (ii) the development of classifiers  resilient to concept drift and adversarial noise,   (iii) consideration of usability by  recording of user profiles  in a user-transparent fashion and respectful of user privacy, and (iv) combination of continuous authentication tool with traditional security mechanisms.
%, as the performance of the classifiers for all groups of users reached over 90\% accuracy for windows of observation longer 10 minutes. 

%In other words, using a behavioral based continuous authentication system to flag a fast operating  malware or exploit would only be advisable if the tool is combined with traditional anti-malware approaches such as an antivirus.





==> OLD/experiments_old.tex <==
% ===========================
% EXPERIMENTS SECTION
% ===========================
This section first present our feature engineering approach to streamline the learning process. Then, it reports the experiments that we have designed to test our hypotheses:

\textbf{H1}: Computer users have unique usage profiles, like unique signatures that can be distinguished from one another.

\textbf{H2}: Profile uniqueness increases with observation time, as more computer usage data become available.

\textbf{H3}: Profiles are consistent over weeks, that is, repeated weekly.

Briefly, our analysis has involved a diverse set of machine learning tools, including deep learning and traditional learning classifiers that we used to distinguish among users (H1) and weeks (H2). We also used Self-Organizing Maps (SOM) to introduce a novel approach for detection and categorization of concept drift in the usage behaviors over the study period (H2).

% ===========================
% Feature Engineering
% ===========================
\subsection{Feature Engineering}

Feature engineering is the process of using domain knowledge to determine the most appropriate features for machine learning analysis \hl{[ref]}. This usually involves making trade-offs regarding data representation. We converted the data of each user into a feature matrix, that is, a collection of feature vectors stacked. In this matrix, each vector (line) represented one-minute of process and network activity on a given study day linked with the respective temporal information (Table~\ref{tab:matrix_template}). Each vector included 10 temporal features, 100 process features, and 454 network features, which we discuss in the following subsections. In other words, each user was represented by a matrix containing a set of vectors, one per minute of activity, with 564 features each.
\todo[inline]{include reference}

\begin{table*}[!ht]
\caption{An example of the matrix with popular app features}
\label{tab:matrix_template}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}Minute\\ in day\end{tabular} & Sunday & ... & Saturday & Month & Day & \begin{tabular}[c]{@{}c@{}}Other\\ app\end{tabular} & \begin{tabular}[c]{@{}c@{}}Popular\\ app 1\end{tabular} & ... & \begin{tabular}[c]{@{}c@{}}Popular\\ app 99\end{tabular} & \begin{tabular}[c]{@{}c@{}}Popular\\ website 1\end{tabular} & ... & \begin{tabular}[c]{@{}c@{}}Popular\\ website 200\end{tabular} & \begin{tabular}[c]{@{}c@{}}Country level\\ domain 1\end{tabular} & ... & \begin{tabular}[c]{@{}c@{}}Country level\\ domain 253\end{tabular} & \begin{tabular}[c]{@{}c@{}}Other\\ website\end{tabular} \\ \hline
0 & 0 & ... & 1 & 7 & 27 & 1 & 0 & ... & 0 & 0 & ... & 0 & 0 & ... & 0 & 0 \\
... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
6 & 0 & ... & 1 & 7 & 27 & 3 & 1 & ... & 0 & 1 & ... & 1 & 1 & ... & 0 & 0 \\ \hline
... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... \\
1436 & 0 & ... & 1 & 7 & 27 & 0 & 0 & ... & 1 & 1 & ... & 1 & 0 & ... & 0 & 2 \\
... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
\end{tabular}
}
\end{table*}


\subsubsection{Temporal Information}

We included the following temporal features: the minute in day (numerical, ranging from 1 to 1440) at which a process and/or network activity was detected, the respective day in week, month (numerical, ranging from 1 to 12), and day in month (numerical, ranging from 1 to 31). In the first feature, '1' marks the first minute of the day (that is, 00:00 AM) while '1440' indicates the last minute of the day (that is, 11:59 PM). For the second information, we used seven binary features, one for each day in week, where '0' means 'inactive' and '1' means 'active'. The example showed in Table~\ref{tab:matrix_template} illustrates the situation where an event was logged on July 27, Saturday, at 00:05 am.


\subsubsection{Process Information}

The first feature engineering trade-off we made was related to the list of processes executed by a user. If we build feature vectors that consider all software used by all users, we would have to choose one of the following alternatives: (i) enumerate all software that a user could use and consider this complete list as features for all users, or (ii) create personalized feature vectors for each user containing information about the specific software used by them. The first alternative would lead to an exhaustive list of processes, thus producing sparse feature matrices that could impose memory and CPU overheads while possibly resulting in overfitting of the learning models. The second alternative is not ideal either because, under this condition, the learning model would need to be updated every time a new user enters the group (e.g., a new employee is hired) or a new software is executed. 

Therefore, we opted for a simplified version of the first alternative by considering a finite and common set of process features comprising 99 widely used Windows 10 applications (e.g., Avast, MS Word, WinZip) selected from publicly available lists~\cite{fblq2018office,pcmagBackup2018,best23backup,valve2018,G2bestCS,fblq2018music,DT2018Media,fossMedia2017,G2bestIDE,quora10IDE,best13RA,bestRAS2018,BestAntiV,10antimalware,filehippo2018,CBS2018,muo2018,ninite2018,G2bestoffice}. These feature were binary, where '0' means 'inactive' while '1' means 'active'. For example, if the user was using a particular popular application in a given minute, the respective feature would contain '1', while the features related to the other popular applications unused at that minute would contain '0'. We also included a numerical feature called “other applications” to count the usage of any software other than the 99 popular processes. Table~\ref{tab:matrix_template} illustrates the situation where the user used a single popular process and three other applications at a given minute.


Importantly, our process features only covered user-initiated applications. Any other processes generated by the OS were not taken into account once they do not reflect the user's profile, and therefore may provide misleading results. For instance, consider the situation where Alice's computer checks for new Windows updates every morning at 10:00 AM while Bob's computer does the same task every afternoon at 3:00 PM. This might create unique, distinguishable profiles for Alice and Bob, but has nothing do to with their actual usage behavior. Later, one might found that Alice's and Bob's profiles are not that distinguishable when discarding OS-based activity.


\subsubsection{Network Information}

The second feature engineering trade-off we made was related to the network information, that is, the domains accessed by the users during the study period. Following the same idea adopted for the process information, we employed an  approach aimed at minimizing information loss in user profiles while streamlining the development of the learning models. We noticed in our dataset that some participants accessed websites from countries other than the United States, which alerted us to the importance of considering both US and foreign (e.g., China, Brazil, United Kingdom) domains.

Our network features set comprised the 200 most popular US websites (e.g., google.com, amazon.com, facebook.com) according to the Alexa list along with 253 country-level domains (e.g., .cn, .br, .uk) that a user might visit~\cite{countryDomains}. All these features were binary, where '0' means 'inactive' while '1' means 'active'. For example, if at a given minute the user was accessing only "amazon.com", which is a popular US domain, and "sina.com.cn", which is a foreign domain, the two respective features would contain '1', while the features related to the other popular US domains and foreign domains would contain '0'. We also included another feature called "other websites" to capture any activity other than the previous ones, such as US websites not included in the top 200 list. Table~\ref{tab:matrix_template} illustrates the situation where the user accessed two popular US websites and one foreign domain at a given minute. In order to get the network information accurately, we first converted the raw IP addressed and port numbers into domains. This was because, for instance, an access to "amazon.com" could be recorded under two different IP addresses as the DNS might direct requests to different Amazon servers.

We acknowledge that, for both process and network information, our feature engineering approach can lead to information loss as we grouped - and not discriminated - less popular applications and websites, thus loosing their identities. But, as discussed before, we decided to err on this side than sacrifice power and feasibility of the machine learning models by using sparse matrices with one feature for each possible process and website. \hl{Moreover, we decided to not look at our dataset when choosing the features because, in most real-world applications, there is no prior knowledge about which processes the user could use, so such a practice would be unrealistic and unfair. Also, we preferred to perform our analysis in a more generalized fashion instead of restricting it to our dataset, which reflects our sample and study period. As a result, we found that 10\% of our process features and 44\% of our network features were not used by any participant over the study period, while the rest of the features were used by at least one participant at some point of the study period.}
\todo[inline]{Fabricio/Daniela, que acha dessa justificativa em amarelo? Te convenceria, se voce fosse um reviewer? Lembre que, na primeira versao do paper, foi usada uma heuristica para escolher as features de modo a cobrir X\% dos nossos participantes. So que, alem de isso nao soar muito feasible/realistic pra mim, eu descobri que muitas dessas features sequer foram utilizadas pelos users, o que nao faz muito sentido (usamos uma heuristica para escolher features que nao sao usadas). Por isso decidi mudar o discurso.}
\todo[inline, backgroundcolor=blue!50]{Fabricio: parece bom pra mim, acho que ficou melhor que antes!}


% ===========================
% Machine Learning Analysis
% ===========================
\subsection{Machine Learning Analysis}

As mentioned at the beginning of this section, our machine learning experiments aimed at testing the uniqueness of the user profiles as well as their consistency over weeks. In our view, these investigations may produce useful findings under two different situations, so we designed two experimental scenarios accordingly: 

\begin{itemize}

  \item \textbf{Experimental Scenario 1:} considering the original feature matrices. As the process features showed some level of variability among our participants, we considered that this scenario could simulate large departments or even different departments in corporate settings, where users are more likely to use different applications, depending on their occupation and duties.
  
  \item \textbf{Experimental Scenario 2:} removing process features unused by all participants from the feature matrices. In other words, we kept only process features that were used by every single participant at some point of the study period. We considered that this scenario could simulate small departments in corporate environments, where users often have limited access to a standard set of applications. Like in the previous scenario, we did not perform any modification in the temporal or network features.
  
\end{itemize}
\todo[inline]{Guys, the description of the scenarios is very important, so can you please review it?}

\todo[inline, backgroundcolor=blue!50]{Fabricio: Do we need to include the number of features used in each scenario?}

% This part below was moved to the discussion section.
%We hypothesized that the profiles of our participants were more unique for the first scenario compared to the second one. For example, consider the situation where Bob, from the marketing department of a tech startup, uses Adobe Photoshop every day from 8:00 AM to 2:00 PM, which Alice, from the software engineering department, never uses. In this case, the simple fact of using Adobe Photoshop can distinguish between the two employees. However, it would not be that simple to distinguish Bob from Megan, also from the marketing department, which uses Adobe Photoshop every day as well, but from 1:00 PM to 5:00 PM. The temporal patterns in the profiles would need to be examined in cases like this.

In our experiments, which we describe in the following subsections, we decided not to submit the feature matrices to feature selection techniques, which would allow us to obtain the most discriminating subset of features for each participant. We believe that this practice is infeasible and unrealistic since such information is not available \textit{a priori} in real applications. \hl{Besides, the most discriminating features are possibly sensitive to the observation time, so the use of feature selection tools might not be suitable to CA mechanisms.}
\todo[inline]{Maybe we should remove this sentence. It is possible that some studies have successfully used feature selection for continuous authentications... I'm not familiar with this literature}

\todo[inline, backgroundcolor=blue!50]{Fabricio: Can't we include the concept drift as a reason for that too? I.e., user behaviour change as time goes by, we would need to make use of feature selection tools every time the concept change or something similar.}

\subsubsection{Testing Profile Uniqueness}

The goal of the first experiment was to examine whether the user profiles are unique/distinguishable. We decided to perform this investigation in two different ways, so we included two machine learning approaches, and then we compared them both in terms of feasibility and performance for CA mechanisms. \hl{The first approach was the multi-class classification, where a single predictive model is created based on the data of all users, and then used to distinguish among each other. The second approach was the one-class classification, where one predictive model is created for each user based on their data and regardless of the other users}. Although we believe that the one-class approach is more suitable for a CA tool, given that it would not require the model to be retrained every time a new user appears, the multi-class approach might achieve better results in terms of accurate predictions, given that it has access to all classes when building the model, creating better decision boundaries~\cite{Tax2001}. In addition, multi-class is better than one-class classification when a  large number of non-target classes (in our case, the data from other users) is available~\cite{10.1007/978-3-540-89378-3_32}. Therefore we decided to include both in this study. 
% In this study, 
We also aimed at examining whether the uniqueness of the user profiles is sensitive to the observation time. Therefore, for each experimental scenario, we included three experimental conditions: (i) using the first week of data only, (ii) using the two first weeks of data, and (iii) using all the three weeks of data. 

\todo[inline]{Fabricio, voce poderia melhorar essa explicação em amarelo e, se possível, incluir uma referência? Acho que seria legal detalhar a diferença das duas abordagens, talvez um exemplo ajude. Só pra embasar um pouco do pq achamos que one-class é mais feasible que multi-class para continuous authentication. A introdução desse paper aqui pode ajudar com algumas ideias: https://www.cs.waikato.ac.nz/~ml/publications/2008/hf08-domainsForOCC.pdf. Fique a vontade para reescrever qualquer coisa da forma que achar melhor!}
\todo[inline, backgroundcolor=blue!50]{Fabricio: adicionei uma referência e comentei sobre a criação de uma melhor fronteira de decisão. Adicionei também um pequeno texto comentando os resultados do artigo que você comentou.}

\textbf{Multi-Class Classification.} For the multi-class experiments, we chose four well-known machine learning models, in which three of them are traditional (SVM, Random Forest, and Decision Tree~\cite{scikit-learn}) and one is a deep model (LSTM \hl{[Include Reference]+}). \hl{[Include SVM parameters]}. 
We used the same parameters as the authors~\cite{scikit-learn} in both Random Forest and Decision Tree. \hl{[Include LSTM parameters and/or details if needed]}. To train these models, we split the data in two sets: the first $2/3$ used for training and the remaining $1/3$, for testing. We consider these proportions valid given that, when using all the data, we would have approximately two weeks of users behaviours to train the models and the remaining to test \hl{[check this explanation]}. Before training and testing the models, all the features werer normalized using min-max~\cite{scikit-learn} (applied separately to the training and test sets). It is important to note that this is an offline setting, that is, we did not update the model but trained it only once. To evaluate this experiment, we used the accuracy of each model. 
\todo[inline, backgroundcolor=blue!50]{Aokun, please include SVM parameters and/or model reference if you used SGD (which is an "approximation" of SVM)}
\todo[inline, backgroundcolor=blue!50]{Heng, please include LSTM parameters and/or model reference}
\todo[inline, backgroundcolor=blue!50]{I included a new explanation for our data split, but I'm not sure if this is enough}
\hl{Furthermore, we tested SVM and LSTM with different user group sizes of 3, 7, 10, and 17 users, with users randomly assigned to these different groups. For each group size, we analyzed classification accuracy for each of the following window sizes: 1, 5, 15, 30, and 60 minutes. (explain why)}
\todo[inline, backgroundcolor=blue!50]{Will we include these experiments? To do so, we need to include the sliding window figure again and explain it before reporting the experiment}



\textbf{One-class Classification.} For the one-class experiments, we chose two models widely used for outlier detection: One-Class SVM and Isolation Forest~\cite{scikit-learn}. \hl{[Include One-Class SVM and Isolation Forest parameters and/or details if needed]}. We also used the same training and test sets as before (the only difference is that we took the last $N/16$ instances of the $16$ other users to compose an outlier set with the same size of the test set, to ensure a more accurate accuracy value), the same normalization technique (min-max~\cite{scikit-learn}) as same metric (accuracy of each model).
\todo[inline, backgroundcolor=blue!50]{Luiz, please include One-Class SVM and Isolation Forest parameters and/or model reference}


\subsubsection{Testing Profile Consistency}

The aim of the second experiment was to investigate whether the user profiles exhibited concept drift over weeks within the study period. This phenomenon refers to changes in the user behavior that can occur due to several different reasons (e.g., travel, days off, change of responsibilities within the organization, etc.), so it varies from one user to another \hl{[reference]}. Therefore, to perform this investigation for each user in an independent fashion, we opted for using one-class classification only, together with visualizations generated by a Self-Organizing Map (SOM), an architecture of unsupervised Artificial Neural Network (ANN) which maps high dimensional data into low-dimensional space using fully connected neurons, grouping similar neurons and creating similarity clusters that reflect attribute relationships of input data, which are represented in light areas of the image~\cite{umatrix}. First, we computed SOM for weeks one, two, and three separately to check whether the usage profiles changed over the weeks. We chose one week intervals because, in general, computer usage profiles are expected to recur on a weekly basis. Then, we computed the classification curves using one-class classification (it exhibited better results than Isolation Forest in previous experiments) because we wanted to examine concept drift for each user independently. To do so, for each user, we used data from week one to train the classifier and then we slide a window over the data from weeks two and three to extract multiple test sets (they were used one by one, generating one accuracy per set), as shown in Figure~\ref{fig:q2_methodology}. The window has one week length and one hour step. We chose one week because, in general, usage profiles are expected to reoccur on a weekly basis. The results were used to plot an accuracy curve, any variability in the curve may indicate presence of concept drift, which can be categorized into one of the four types presented in Figure~\ref{fig:drift_types}: sudden drift, when a concept is suddenly replaced by a new one; gradual drift, when the probability of finding the previous concept decreases and the new one increases until it is completely replaced; incremental drift, when the difference between the old concept and the new one is very small and the difference is only noticed when looking at a longer period; and recurring concepts, when previous active concept reappears after some time~\cite{Lemaire2015}. 

Before actually testing the SOM visualizations and curves in real data, as a initial test we generated fake datasets to test whether they can properly detect the type of concept drift.

Finally, after generating both SOM visualizations and the accuracy curve for each user, we asked two independent reviews to answer the following questions: (i) Do SOM and classification curve both suggest the presence of some type of drift? (ii) If so, what is the type of drift suggested by the classification curve? Then, an inter-rater reliability analysis using the Kappa statistic was performed to determine consistency among raters. 
% . \hl{[Create Figure for Concept Drift types, including citation and explanation of every type]}.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figs/new_version/q2_methodology.pdf}
    \caption{One-class classification methodology for second experiment scenario using a fixed training set containing one week of data and a sliding window for the test sets.}
    \label{fig:q2_methodology}
\end{figure}

\todo[inline, backgroundcolor=blue!50]{Include figure for drift types and their explanations in the text.}

\begin{figure*}
    \centering
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\columnwidth]{figs/new_version/drift_types/sudden_drift.pdf}
        \caption{Sudden Drift.}
        \label{fig:sudden_drift}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\columnwidth]{figs/new_version/drift_types/gradual_drift.pdf}
        \caption{Gradual Drift.}
        \label{fig:gradual_drift}
    \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\columnwidth]{figs/new_version/drift_types/incremental_drift.pdf}
        \caption{Incremental Drift.}
        \label{fig:incremental_drift}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\columnwidth]{figs/new_version/drift_types/recurring_concepts.pdf}
        \caption{Recurring Concepts.}
        \label{fig:recurring_concepts}
    \end{subfigure}
    \caption{\hl{Drift types}.}
    \label{fig:drift_types}
\end{figure*}


\todo[inline] {Agora precisaria descrever todos os detalhes metodologicos, incluindo o SOM (talvez de para aproveitar o texto da primeira versao do paper). Essa secao vai ser bem importante, pois vamos apresentar a nossa abordagem de caracterizacao de concept drift (criterios, inspecao visual e kappa, etc.). Acho que seria bem importante explicar que testamos a abordagem com dados conhecidos para verificar a confiabilidade dos resultados. Os slides podem ajudar, esta tudo escrito neles. Tambem eh possivel usar figuras, se achar que ajuda.}

\todo[inline]{Ah, tambem precisaria explicar os tipos existentes de concept drift (quais sao e o que cada um significa). Podemos tentar fazer uma figura, se achar que ajuda, pra nao precisar usar figuras de outros papers.}

\hl{We need to include the procedure that raters followed to decide about presence and type of concept drift (i.e., the questionnaires).}
  
  
As far as we know, there is no clear measurement on how much similarity exists among SOM results. That’s why we examined drift through the visual inspection of the results (SOM and curves), but we involved two independent reviewers to reduce subjectivity effects. For future work, we can elaborate heuristics to categorize drift from the curves in a more deterministic fashion.



\subsubsection{Evaluation}

\todo[inline] {Fabricio, vejo duas opcoes: criar essa subsecao para detalhar a avaliacao dos modelos (treino/teste/etc), assim como foi feito na primeira versao do paper, OU incluir tais detalhes dentro das duas subsecoes anteriores, ja que cada experimento teve suas particularidades. Fique a vontade pra seguir da forma que achar que fica melhor/mais logica!}












% =====================================================================================
% OLD VERSION
% =====================================================================================

% We applied three distinct machine learning methods: (i) a newly developed BA-LSTM (detailed in Section \ref{subsec:BA-LSTM}), (ii) SVM, and (iii) Random Forest-V. We also used SOM  to visualize the uniqueness of computer usage profiles and their temporal consistency. This diverse set of machine learning approaches comprised both deep learning (BA-LSTM, SOM) and  traditional (SVM and Random Forest-V)  machine learning, including  supervised (BA-LSTM, SVM, Random Forest-V) and unsupervised (SOM) methods. 

% This section first presents our feature engineering approach to streamline the learning models. Then, it reports the application of sliding windows in our analysis. Next, it introduces our newly developed BA-LSTM  and provides  background on Random Forest-V and SOM. 

% \subsection{Feature Engineering}

% Feature engineering is the process of using domain knowledge  to determine the most appropriate features for machine learning analysis. This process usually involves making trade-offs regarding data representation.
% %Despite of collecting the complete set of system process and network events 
% %(process and network related) 
% % executed in the user’s desktop, we decided to perform feature engineering on the collected raw attributes. \textcolor{blue}{On the one hand, our feature engineering method refines the collected information, which helps machine learning analysis method to learn the difference between users. On the other hand, the feature set of different users remains constant, which simplifies the design of our machine learning analysis method.} 
% % %<Otherwise, each user would end up with different set of features in his profile model, which would render machine learning analysis rather complex.> 
% % Further, before machine learning analysis, 
% We converted the user’s data into vector matrices, where each vector represented one-minute of process and network information on a given study day. 
% %We streamline the development of the learning models we made tradeoffs regarding the representing of process and network information for the classifier.

% %In total we had 18 matrices representing the 21-day activities of each one of the 18 users, who successfully completed the study.  In total we collected an average of 59.94 MB per user (standard deviation 36.42 ). After feature engineering we had on average 127.56 MB of data in each matrix per user (standard deviation 56.33) 


% \subsubsection{Process Information}

% The first feature engineering trade-off we made related to the list of processes executed by a user. The list of processes exhibits a large commonality among users. However, at the same time, it  represents some variability, which is the crucial characteristic that make profiles unique.  For example, consider Mary and John who both work for the same corporation, but in separate departments. While they both use Chrome and MS Office, John uses Stata for statistical analysis, which Mary never uses. Mary, in contrast,  uses Adobe Photoshop, which John never uses. If we build feature vectors that consider all software used by all users, we would have to choose one of the following alternatives: (i) enumerate all software that a user could use and consider this complete list as features for all users or (ii) create personalized feature vectors for each user containing information about the specific software used by them. The first alternative is not feasible because there is a lack of  prior knowledge about  which applications could run on a user's machine at all points in time. Further, the use of an exhaustive list of applications would result in sparse matrices, which would impose memory and CPU overheads, while possibly resulting in overfitting of the learning models. The second alternative is not ideal either, as, under this condition, the learning model would need to be updated every time a new user enters the group (e.g., a new employee is hired) or a new software is executed. 
% %Option (iii) is also discouraged by our current methods. To prove our profiling hypothesis, we choose classification methods which requires training a single model using data from all of the users. This requirement cannot be fulfilled if each users has a unique feature representation. In our future work, however, to build a profile model for each of the users, we could consider using option (iii) combined with one-class classification methods. Therefore, we decided to adopt a heuristic approach to engineer process information.


% %Our method not only carefully selects and engineers the process and network information, but also associate them with timing information.

% \begin{figure}
%     \centering
%     \includegraphics[width=.50\textwidth]{figs/process_coverage_cropped.pdf}
%     \caption{Percentage of applications captured by the profile extractor (Coverage) as a function of the set of applications based on the Windows top 150 list.}
%     \label{fig:process_coverage}
% \end{figure}



% We, therefore, opted for a simplified, heuristic-based version of the first alternative with a finite set of commonly used Windows 10 applications as process features. These applications were selected based on publicly available lists of common Windows applications~\cite{fblq2018office,pcmagBackup2018,best23backup,valve2018,G2bestCS,fblq2018music,DT2018Media,fossMedia2017,G2bestIDE,quora10IDE,best13RA,bestRAS2018,BestAntiV,10antimalware,filehippo2018,CBS2018,muo2018,ninite2018,G2bestoffice}. In total, there are currently 150  Windows applications considered most popular.  We  determined the specific number of most popular  applications to consider as feature vectors in our approach based on  the function between the percentage  of applications captured by the  profile extractor from all 18 participants (Coverage) and the number of most popular Windows applications. As shown in  Figure~\ref{fig:process_coverage}, the top 100 Windows applications covered 80\% of  applications represented in our dataset. Inclusion of additional  applications would have resulted in little gain in  coverage.

% We also included a feature called “Other Applications”, to capture  usage of any other software not included in the top 100 list. For example, if Stata was not part of the Windows top 100, but was used by John, the information  would be captured via this “Other Applications” feature. We acknowledge that this heuristic-based approach can lead to information loss under some conditions  (e.g., John uses Stata). However, we decided to rather err on the side of possible information loss for specific profiles than sacrifice  power and feasibility of the machine learning models. 


% \begin{table}
% \centering
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Minute \\ in Day\end{tabular} & Sunday & … & Saturday & \begin{tabular}[c]{@{}l@{}}Other \\ App\end{tabular} & \begin{tabular}[c]{@{}l@{}}Popular\\  App 1\end{tabular} & … & \begin{tabular}[c]{@{}l@{}}Popular\\ App 100\end{tabular} \\ \hline
% 1 & 0 & ... & 0 & 0 & 0 & ... & 0 \\ \hline
% 2 & 0 & ... & 0 & 2 & 1 & ... & 0 \\ \hline
% 3 & 0 & ... & 0 & 5 & 1 & ... & 1 \\ \hline
% … & ... & ... & ... & … & … & ... & … \\ \hline
% N & 0 & ... & 1 & 1 & 0 & ... & 1 \\ \hline
% \end{tabular}
% }
% \caption{Example of process matrix, where each row corresponds to process activities for a particular user during a given minute per day.}
% \label{tab:process_matrix}
% \end{table}

% Table~\ref{tab:process_matrix} shows the feature vectors for process information. Each row in this matrix corresponds to process activities for a particular user during a given minute per day. This results in matrices with 1440 rows,  corresponding to every minute in a 24-hour period. That is, in total, each user was represented by a collection of up to 21 matrices, one for each day they were active in the study.  If the user was active in one particular popular application in a given minute, the respective cell would contain a 1. Otherwise, the cell would contain a zero. If, in a given minute,  the user accessed  software, which did not belong to the list of Windows top 100 applications, we would increase the counter on the cell corresponding to the feature “Other Applications”. 


% \subsubsection{Network Information}

% The second feature engineering trade-off we made related to network information, more specifically to the list of domains a user connected to during  the study. Our decisions regarding feature engineering of network information were  similar to those  for processes information. Similar to the execution of processes, the list of domains users connected both showed commonalities among users, as well as variability between users.  For example, while both Mary and John may connect regularly  to a set of popular U.S. sites  (e.g., Amazon, Facebook, CNN, etc.),  Mary being of Chinese descent, also frequently  connects to Chinese news websites (e.g., www.sina.com.cn), while John never does. 
% %Therefore, the same challenges faced for processes arise. On one hand, we want to capture the traits that distinguish Mary and John (e.g., Mary connecting to sites in China is usual, while for John this is an anomaly). On the other hand, attempting to determine and predict an exhaustive list of domains for machine learning feature representation is unfeasible. Further, a personal domain lists per user is not recommended for classification for the same reasons discussed for process information. 

% \begin{table}
% \centering
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Minute \\ in  Day\end{tabular} & Sun. & … & Sat. & \begin{tabular}[c]{@{}l@{}}Google\\ (Pop \\ site)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Amazon\\ (Pop\\ site)\end{tabular} & \begin{tabular}[c]{@{}l@{}}…\\ (Pop  \\ site) \end{tabular} & \begin{tabular}[c]{@{}l@{}}US\\   (Country)\end{tabular} & \begin{tabular}[c]{@{}l@{}}CN\\   (Country)\end{tabular} & \begin{tabular}[c]{@{}l@{}}…\\   (Country)\end{tabular} \\ \hline
% 1 & 0 &  & 0 & 0 & 0 & … & 0 & 1 & … \\ \hline
% 2 & 0 &  & 0 & 1 & 0 & … & 1 & 1 & … \\ \hline
% 3 & 0 &  & 0 & 0 & 1 & … & 1 & 1 & … \\ \hline
% … & … &  & … & … & … & … & … & … & … \\ \hline
% N & 0 &  & 1 & 0 & 0 & … & 1 & 1 & … \\ \hline
% \end{tabular}
% }
% \caption{Example of network matrix, where each row corresponds to network activities for a particular user during a given minute per day.}
% \label{tab:network_matrix}
% \end{table}

% We, therefore,  employed a heuristic-based approach, similar to that adopted for process feature representation to minimize  information loss in user profiles, while at the same time streamlining the development of the learning models. Features in our matrix were a list of the most popular network domains taken from the Alexa popular website list, along with a list of 255 country-level domains (e.g., .cn, .br, .uk, etc.)  a  user might visit~\cite{countryDomains}. These network features represented: (i) the frequency of access of  popular network domains  and (ii) the frequency of access of the selected country-level domains. %Commonly used domains are popular websites. 

% %In our log files, network information was recorded as raw IP addresses and port numbers. 
% Our feature engineering method first converted raw IP addresses and port numbers  into  domains (e.g., Amazon.com). This process is crucial to avoid introduction of noise in the feature vectors. For example, an access to Amazon.com could be logged under two different IP addresses because DNS might direct requests to different Amazon servers.
% %with different IP addresses. By considering the domain information (Amazon.com), we correctly capture that both Alice and Bob accessed Amazon.com. 

% %Popular network domains represent popular websites. Using a list of popular network domains improves our network information in the following aspects. First, it helps generate machine learning model focusing on network activities generated by the user. Second, it reduces the sparsity in the matrices. Using a list of domains, which are not widely used, will result in most features in the vectors having a zero value.

% %The country-specific features (247 in total) represent country-specific domains that, considering a cohort of users from an organization and living in the US, would be accessed by a subset of users.

% %\begin{figure}
% %    \centering
% %    \includegraphics[width=.45\textwidth]{figs/network_coverage_cropped.pdf}
% %    \caption{Percentage of domains captured by the profile extractor (Coverage) as a function of  the set of Alexa top 300 domains.}
% %    \label{fig:network_coverage}
% %\end{figure}

% %As shown in Figure ~\ref{fig:network_coverage} 
% We considered the first 300 top sites from Alexa (as of October 8, 2018). We found that the top 200 Alexa websites represented approximately 70\% of the captured domains in our user study and, thus, included these domains as network features. 
% %Further analysis into the remainder 80\% of domains accessed by our participants showed that over 77.6\% of these domains were servers that were not directly accessible by the user (e.g., email servers, advertising servers). Further, 6\% of these domains were web  servers not usually used for data exchange between user end applications. Another 5\% of the remaining IP addresses came from  servers hosting websites for other Internet content providers. On average, w 11.2\% of the remaining domains were user accessible websites. 
% %The composition of the domains that are not included in Alexa is shown in Figure~\ref{fig:network_ratio}. 
% %We, thus, decided to include as network features the  first 200 Alexa popular websites which covered more than 70\% of the user accessible domains.
% Figure 6 illustrates how we represented our feature engineering network information. 
% %We, therefore, representing each minute of network information for all days in the 21 days of the study with feature vectors in the form of a matrix (see Figure~\ref{tab:network_matrix}). First, we extracted the domain names of the remote servers and the countries in which the remote servers resided on for all the IP addresses in outgoing network connections made by the participants. This information is then used to create, for each participant, matrices representing vectors capturing one-minute of activity during a day for each one of the domains.
% For example, if in a given minute, Alice accessed Amazon.com, the feature ``Amazon.com'' would contain the value 1. If, in that minute, she also accessed www.sina.com.cn, the value of feature ``CN'' would contain the value 1. 
% %, meaning that Alice accessed a site in a Chinese domain. 
% We used 455 network features in our network matrices. %Each network feature vector is indexed with a timestamp that indicates the time it is recorded. %The network feature vectors also included timing information, specifically the time of the day the minute corresponds to (similarly to process, a number in the range [1-1440]) and the day of the week (a number in the range [1-7]).
% % \subsubsection{Feature Engineering Outcome}
% In total, each user was represented by a matrix with process and network information, containing a set of vectors with 564 features for each  minute in a maximum of 21 days.

% %(After having built the process and network feature vectors, we combined them to form the 18 matrices where each matrix represents 21 days of process and network information of the corresponding participants. Each vector of each matrix contains the concentration of one minute of process and network activities for a participant. The feature vectors also carry information about the time of the day and day of week, in which the minute of activity belonged to. Time of the day information is represented using a number from [0, 1439], representing one of the minutes of the 1440 minutes of a day. Day of the week information is represented using number from [0-6] representing one of the seven days in a week starting on Sunday. Each vector starts with time of the day and day of the week information of the represented minute followed by process and network features accordingly. In total, each vector has 556 features.


% \subsection{Sliding Window}
% \label{sec:sliding}

% Due to the temporal nature of our dataset, we used sliding windows of data for  classification, including windows of 1, 2, 5, 10, 15, and 50 minutes.

% For BA-LSTM and SVM, we created one classifier for each window size, where the training, testing, and validation data provided to the model was given according to the window size. For BA-LSTM training, test, and validation, each minute in a window was fed into the model consecutively. For example, for a window of 5 minutes, the model was first fed with data from the first minute, followed by data from the second minute, until the fifth minute. Because SVM cannot handle sequential data directly,  SVM training, test, and validation data from the entire window was fed into the model at once. For both BA-LSTM and SVM  we slid the previous window by one minute and repeated the process described above until  training, test, and validation was completed. The Random Forest-V classifier was trained individually with every minute of training data because the classification label of a given window was determined according to the most prevalent label found for every minute in the window. 
% %For example, if, for a window of five minutes, the classifier produced labels: User 1, User 1, User 2, User 1, User 2, the window would be classified as belonging to User 1.

% %\begin{figure}[!ht]
% %    \centering
%  %   \includegraphics[width=0.45\textwidth]{figs/sliding_window.pdf}
%   %  \caption{Sliding window mechanism.}
%   % \label{fig:sliding_window}
% %\end{figure}



% %(see Figure~\ref{fig:voting}).   

% %\begin{figure}[!ht]
% %    \centering
% %    \includegraphics[width=0.42\textwidth]{figs/voting.pdf}
% %    \caption{Voting mechanism.}
% %    \label{fig:voting}
% %\end{figure}


% \subsection{Bidirectional Attention Long Short-Term Memory}
% \label{subsec:BA-LSTM}

% For the analysis of the computer usage profiles, we augmented LSTM with a novel  bidirectional and attention mechanism. LSTM was chosen because it exhibits good performance in analyzing time series data, as  in our study. 

% %\subsubsection{Bi-directional LSTM}
% %One of the methods used in this project is based on long short-term memory or LSTM.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figs/data_sequnce-cropped.pdf}
%     \caption{Data sequence with time step of T.}
%     \label{fig:data_seq}
% \end{figure}

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=0.50\textwidth]{figs/LSTM_node.pdf}
% %     \caption{LSTM node showing LSTM($x_t$,$h_{t-1}$)}
% %     \label{fig:lstm_structure}
% % \end{figure}

% The original LSTM~\cite{Hochreiter1997LSTM} 
% %(structure shown in Figure~\ref{fig:lstm_structure}) 
% is well known for modeling sequences of information in one temporal direction (i.e., from the first minute of the input to later minutes).
% %The structure of a LSTM node is shown in Figure~\ref{fig:lstm_structure}. 
% Better performance is expected if the correlation information from both directions of the sequence is considered. For a given sequence with time step
% $x_t, t\in [0,T]$, where T is the time step length (Figure~\ref{fig:data_seq}), we use bidirectional LSTM~\cite{schuster1997bidirectional} to get 
% %annotations
% representations of time steps by summarizing information from both directions of the sequence. This allowed incorporation of  contextual information from both directions in the representation. Our bidirectional LSTM contains a forward LSTM $\overrightarrow{f}$, which reads the sequence $x$ from $x_0$ to $x_t$ and a backward LSTM $\overleftarrow{f}$, which reads from $x_t$ to $x_0$. Thus, for each hidden layer in bidirectional LSTM, we have the $t$th node :

% \begin{align}
% 	\overrightarrow{h_t} &= LSTM(x_t,h_{t-1}), t\in [0,T], \\
% 	\overleftarrow{h_t} &= LSTM(x_t,h_{t+1}), t\in [T,0].
% \end{align}
% Where $h_t$ is the $t$th hidden state of LSTM, and is also used to construct the representation for input $x_t$. $h_{-1}$ in forward LSTM and $h_{T+1}$ in backward LSTM are both 0. \\

% We obtained a final representation state $h_t$ for a given time step $x_t$ by
% concatenating the forward hidden state $\overrightarrow{h_t}$ and
% backward hidden state $\overleftarrow{h_t}$, i.e.,




% \begin{equation}
% 	h_t = 
% 	\begin{bmatrix}
% 	\overrightarrow{h_t} \\
% 	\overleftarrow{h_t}
% 	\end{bmatrix},
% \end{equation}
% which summarizes the information of the whole sequence centered around time step $x_t$.

% %\textcolor{blue}{Compared with original LSTM, Bi-directional LSTM learns more comprehensive representation of different computer users. In additional to be able of capturing the situations where usage activities at early time point triggers another activity later in the time sequence, bi-directional LSTM also considers a later usage activities as successor of former computer usage activities.}

% Compared to unidirectional LSTM, in which each hidden state is generated depending only on the past, bidirectional LSTM learns a more comprehensive representation of different computer users by modeling the behavior on each time step based on both past and future information. \\
% %a program in preparation for other activities, in which case the event happens later in time is in fact the cause of earlier event.}

% %Compared with original LSTM, Bi-directional LSTM learns more comprehensive representation of different computer users. It is able to model the relational information of a certain event at a certain time step from events both before and after that time step. For example, John would like to sign a document in word but does not want the contents to be accidentally changed afterwards. Thus, he decides to first convert the document to PDF before sign it electronically. For bidirectional LSTM, this event will be captured as the user needs Microsoft word before he uses PDF reader, which is more appropriate than regular LSTM representing it as the user would use PDF reader after using Microsoft word.

% \noindent
% {\bf Sequence Attention Layer.} Not all time steps in a sequence contribute equally to the representation of the sequence. Hence, we introduced an \emph{attention mechanism} to give more weight to time steps that are important to the characteristics of the sequence and aggregated the representation of those informative time steps to form a sequence. Specifically, we constructed  the attention layer  as:
% \begin{align}
% u_t &= \tanh (W_sh_t + b_s), \\
% \alpha_t &= \frac{\exp(u_t^T \mu_s)}{\sum_{t=0}^{T} \exp(u_t^T \mu_s)}, \label{eq:alpha_t} \\
% v &= \sum\limits_{t=0}^{T} \alpha_t h_t. \label{eq:v}
% \end{align}
% % The attention structure is shown in Figure~\ref{fig:attention_layer}.
% Where tanh is the hyperbolic tangent activation function and exp is the exponential function. \\
% That is, we first fed the time step annotation $h_t$ through
% a one-layer Multilayer Perceptron~\cite{rosenblatt1961principles} to get $u_t$ as a hidden representation of $h_t$. We then measured the importance of
% the sequence time step as the similarity of $u_t$ with a time step level
% context vector $\mu_s$ and got a normalized importance
% weight $\alpha_t$ through a softmax~\cite{nasrabadi2007pattern} function. After that,
% we computed the sequence vector $v$  as a weighted sum of the time step annotations based on the weights. The context vector $\mu_s$
% can be seen as a high-level representation of a fixed
% query (\emph{"what is the signature or informative time step''}) over the time steps
% like those used in memory networks~\cite{sukhbaatar2015end, kumar2016ask}. The time step context
% vector $\mu_s$ was randomly initialized and jointly learned
% during the training process.

% %\textcolor{blue}{In summary, attention mechanism estimated the distribution of the contribution of each time steps to distinguish the users and emphasize (given more weight in producing output) on those time steps that diverge among the computer users. More precisely, 
% In our approach, the attention mechanism improved the classification capability of LSTM by deciding which time steps displayed the difference among  users and by emphasizing this difference.   

% \subsection{Random Forest-V}

% One disadvantage of the sliding window approach used for BA-LSTM and SVM is its high requirement for computational resources. For example, the larger the window size, the more memory it will require, since the number of features will be multiplied by the window size. Thus, we  augmented  Random Forest with a voting mechanism. As discussed above (Section~\ref{sec:sliding}), we trained the Random Forest-V classifier with every minute of trained data individually and combined the classification results from these multiple one-minute data sequences  to produce the final prediction. Separate predictions were used in the voting process, where the majority class (the class with the highest number of votes) is considered  the final prediction. 
% %An example of this process is shown in Figure~\ref{fig:voting}, where the classification of a five-minute window of data is presented. Each minute in the window is classified individually and the classification label (e.g., User 1, User 2, etc.) is an input in the voting process, resulting in a single class (the most prevalent) output (e.g., Class 1, which was the most prevalent in this example - (voted on three different minutes) for a window of five minutes. 

% Random Forest-V does not require training a new classifier when the window size changes. Therefore, we just trained a single model for every minute individually and changed the window size in the prediction phase. This approach reduced memory usage as the original data was used only once. In addition, the window size can be changed on the fly, advancing the prediction in relation to the sliding window mechanism.

% \subsection{Self-Organizing Maps - SOM}

% We used SOM~\cite{SOM} to visualize individual profiles from each of our 18 participants. SOM is an architecture of unsupervised Artificial Neural Network (ANN), which maps high dimensional data (such as our participants' data)  into low-dimensional space (usually 2D or 3D) using fully connected neurons. During training, SOM groups similar neurons, creating similarity clusters that reflect attribute relationships of input data. We used  Unified Distance Matrix (U-Matrix), which visualizes the distances between  network neurons, whose clusters are represented in light areas of the image~\cite{umatrix}.

% % \subsection{Sliding Window}
% % To create sequences of user behaviors of different lengths, we adopted a sliding window mechanism for all machine learning methods used in our evaluation. In this approach our classifiers works on windows containing $x$ minutes of data for each user. 
% % This mechanism is illustrated in  Figure~\ref{fig:sliding_window}, where the classifier operates on windows of five minutes. After one window of five minutes of user data is processed and classified, the window is slided by one minute and this process repeats until all user data is processed. In this work we analyzed our classifiers when operating with the following window lengths: 1, 2, 5, 10, 15, and 50 min.


% % % \begin{figure*}
% % % \begin{multicols}{2}
% % %     \centering
% % %     \subcaptionbox{Sliding window mechanism.\label{fig:sliding_window}}[\linewidth][c]{
% % %     \includegraphics[width=.45\textwidth]{figs/sliding_window.pdf}}\par
% % %     \subcaptionbox{Voting mechanism.\label{fig:voting}}[\linewidth][c]{
% % %     \includegraphics[width=.29\textwidth]{figs/voting.pdf}}\par
% % % \end{multicols}
% % % \caption{Different time sequence creation method used in our work.}
% % % \label{fig:sequence_creation}
% % % \end{figure*}

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=0.45\textwidth]{figs/sliding_window.pdf}
% %     \caption{Sliding window mechanism.}
% %     \label{fig:sliding_window}
% % \end{figure}

% % \ToDo{Fabricio: TODO - Voting explanation}

% % It involves training the Random Forest classifier with every minute individually  and then, predict a window of N minutes individually with it. 

==> OLD/extract_and_feature_eng.tex <==
This section describes the design and implementation of our computer usage profiling collection module and the feature engineering methods we later employ on the collected dataset. 

\subsection{Data Extraction}

\begin{table*}[h]
\centering
\begin{tabular}{ccccc}
\hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Attributes}} & \multicolumn{4}{c|}{Process information} \\ \cline{2-5} 
\multicolumn{1}{|l|}{} & \multicolumn{1}{c|}{Process ID (PID)} & \multicolumn{1}{c|}{Parent PID (PPID)} & \multicolumn{1}{c|}{Executable pathname} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Active time\\ interval\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{Description} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Integer\\ representing\\ the process ID\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Integer\\ representing\\ the parent\\ process ID\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}The pathname\\ of the\\ process\\ executable file\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}List of\\ time intervals\\ when the process\\ is active\end{tabular}} \\ \hline
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Attributes\\ (continue)\end{tabular}}} & \multicolumn{4}{c|}{Network information} \\ \cline{2-5} 
\multicolumn{1}{|c|}{} & \multicolumn{2}{c|}{Connection information} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Network activity information\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Description\\ (continue)\end{tabular}} & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}Connection Information struct:\\ \{IP address (integer, source and destination),\\ Port number (integer, source and destination), \\ Connection start time (time stamp),\\ Connection end time (time stamp)\}\end{tabular}} & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}Network activity information struct:\\ \{Traffic direction \\ (0 for inbound, 1 for outbound),\\ Time the traffic is intercepted\\ (time stamp)\}\end{tabular}} \\ \hline
\end{tabular}
\caption{Data collection model. Each entry in this table corresponds to the summarized activity for one process in a period of 24 hours.}
\label{tab:datamodel}
\end{table*}

We design our extractor to monitor and record the user behavior by inspecting various process (e.g., Process ID of a process) and network traffic (e.g., source IP address of a network connection) information, hereafter called \textit{process} and \textit{network information}. The \textit{process} and \textit{network information} is acquired using Windows events, which are enumerations of system calls that Windows kernel driver interfaces exposes to the developers. Table~\ref{tab:datamodel} shows an overview of the \textit{process} and \textit{network information} we collect.

\subsubsection{Process Information}
\textit{Process Information} covers the identification information of the processes, e.g., process ID, and the period of time that it is in use. The upper sections of Table~\ref{tab:datamodel} presents the contents of process information. {\bf Process IDs} index each table entry on a given day. {\bf Parent Process IDs} track the relationship among the processes. {\bf Executable pathname} is the full pathname of the executable file of the process. {\bf Active time intervals} are time series corresponding to the time intervals when the processes are active. We consider processes to be active if they are triggering Windows events. In our design, if five minutes elapse after the last Windows event invocation from the process, the last period will be closed with the end time corresponding to the time of the last system events invocation. Table~\ref{tab:processRecordSample} shows an example of the summarized (i.e., showing only fields with general process information) daily activities for Microsoft Word.

\subsubsection{Network Information}
\textit{Network Information} represents network activities of a process. In Microsoft Windows, network activities are assorted into network connection sessions, and link to the correspond processes that initialize these activities. The network activities in the same connection sessions have the same internet sources and destinations. Our network information design reflects this mechanism. The lower section of Table~\ref{tab:datamodel} presents the collected network information. The connection session information is record in connection information, which includes {\bf source IP addresses}, {\bf destination IP addresses}, {\bf source ports}, {\bf destination ports}, and the time when the connection is created and terminated. The information network activities, which belongs to this connection session, are record with network activity information. As IP addresses and ports information are already recorded in connection information, network activity information includes only the time, which the activities are generated, and their direction, outbound or inbound, of the network activities. Table \ref{tab:networkRecordSample} shows the data for one network information for Chrome.

\subsection{Implementation of Data Extractor}
The data extractor is implemented as a kernel-mode driver for Microsoft Windows 10. As a kernel module, our data extractor is separated from the user space processes. This separation benefits our data extraction in the following two aspects. First, it obscures our data extractor, making the data extraction process non-intrusive. Second, it provides protection against user space malware. Figure~\ref{fig:data_extractor} presents the structure of our data extractor. The data extractor collects \textit{process} and \textit{network information} according to the following procedure. When the computer systems are used by the users, the processes in use will generate a series of system events. Windows kernel relays these system events to the data extractor which allows the data extractor to collect different information with different system events. Our extractor contains two sub-modules: process monitor and network monitor, which collect \textit{process} and \textit{network information} accordingly using system events.

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\textwidth]{figs/Data_extractor_structure.pdf}
    \caption{Structure of data extractor}
    \label{fig:data_extractor}
\end{figure}

\subsubsection{Process Monitor}
Process monitor utilizes two categories of systems events with Windows kernel APIs to capture \textit{process} information. The first set of system events covers the creation and termination of the processes. They are used to create per-process records across the lifespan of the processes. The second set of system events includes all process activities related to objects. These activities include memory access, child process/thread creation, handle duplication, and etc. These events incorporate most of the system events that processes generate during execution. They are used to distinguish process status between idle and active.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth,height=1\textwidth]{figs/Proc_mon-merged.pdf}
    \caption{Process monitor work flow}
    \label{fig:proc_mon_workflow}
\end{figure}

The control flow of process monitor recording the system events generated by a process is shown in Figure~\ref{fig:proc_mon_workflow}. First, when a process is created, the process monitor captures this event and records its PID, PPID, and the file path-name of its executable. Then, from the time the first system events gets generated by the process, process monitor creates and updates active intervals of the process. When the process becomes idle, the first active time interval ends. At last, after the process fulfill its task and gets terminated, the last active interval is concluded with the process termination time.

\subsubsection{Network Monitor}
Network monitor utilizes Windows filter platform (WFP) APIs to record \textit{network information}. To avoid introducing too much overhead, our network monitor performs online network traffic inspection. Two different categories of network system events are used to track network traffic. First, the creations and terminations of connection sessions are monitored. At the creation of network session, network monitor records the connection handle, which uniquely identifies the connection session, the process ID of the process that initializes or accepts this connection, along with all the connection information except the connection end time. At termination, network monitor labeled this connection session as closed to avoid confusion cased by Windows reusing the network handle. Second, the arrival of inbound IP packets and the departure of outbound IP packets are monitored. Using the network session handle, the direction of the IP packets and the time, which the packets are intercepted, are recorded and associated with a connection session.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth,height=0.75\textwidth]{figs/Net_mon-merged.pdf}
    \caption{Network monitor work flow}
    \label{fig:net_mon_workflow}
\end{figure}

The work-flow of our network monitor recording a connection session is shown in Figure \ref{fig:net_mon_workflow}. Starting from the creation of a connection session, our network monitor is invoked by Windows Filter manager. Our extractor then records all the presented connection features along with the connection handle and the process ID of it owner process. Since then, network monitor keeps identifying and recording the network traffic features of the network traffic related to this connection session using the connection session handle. At last, when the connection session is closed, the connection session close time is recorded.

\subsection{Feature Engineering}



==> OLD/feature.tex <==
%\subsection{Feature Engineering}
Feature engineering translates the collected information into more ideal features which enhances the collected computer usages behavioral information and transforms computer usage data into matrices composed of vectors describing user per-minute activities. Our method not only carefully selects and engineers the \textit{process} and \textit{network information}, but also associates them with the time when the process and network events happened. 
%Through feature engineering method, we convert computer usage behavior information into matrices composed of vectors describing user per-minute activities. 
Our feature engineering method first converts process and network information into process and network vectors representing user's process or network usage behavior of one minute. Then, we concatenate the process and network vectors representation the same minute and generate matrix.
Our feature engineering methods are discussed on process and network respectively. In following paragraphs, we describe our feature vectors and feature engineering procedures.

%\subsubsection{Time Features}

\subsubsection{Process Features}

Process features contains two sets of process information: (i) whether commonly used Windows applications are executed or not (active status), and (ii) the number of random applications are executed. 

We choose to use commonly used Windows applications instead of an exhaustive list of all applications because of the following reasons. First, we do not have pre-knowledge of the applications running in the computer systems of the users. As We do not limit the applications that the computer users would use, there is no. Second, it is challenging to include an exhaustive list of applications as the different applications accumulates over the time. Third, using an exhaustive list of application would result in sparse computer usage activity matrices, where most items in the matrix have the value of zero. The sparsity of matrices consumes excessive and unnecessary memory and computational power, while confuse machine learning/deep learning methods to overfitting the generated model.

We consider random applications as the specific applications used by few computer users. Thus, random applications represent the user-specific preference on application selection. We choose to categorize this information using the number of random applications rather than whether the random applications are executed or not. The number of random applications better preserves the user specific preference as users have different random applications running in their computer systems. 

\begin{figure}
\begin{multicols}{1}
    \centering
    \subcaptionbox{Coverage of process V.S. number of popular process\label{fig:process_coverage}}[0.45\textwidth][c]{
    \includegraphics[width=.45\textwidth]{figs/process_coverage_cropped.pdf}}\par
\end{multicols}
\begin{multicols}{1}
\centering
    \subcaptionbox{Coverage of websites V.S. number of popular websites\label{fig:network_coverage}}[ 0.45\textwidth][c]{
    \includegraphics[width=.45\textwidth]{figs/network_coverage_cropped.pdf}}\par

\end{multicols}
%\caption{}
\label{fig:feture_coverage}
\end{figure}

We choose the commonly used Windows applications from the a number of websites and forums~\cite{fblq2018office,pcmagBackup2018,best23backup,Google2018vm,Google2018ocs,valve2018,G2bestCS,fblq2018music,DT2018Media,fossMedia2017,G2bestIDE,quora10IDE,best13RA,bestRAS2018,BestAntiV,10antimalware,filehippo2018,CBS2018,muo2018,ninite2018,G2bestoffice}. In total, there are 150 different applications that these sites agree to be most commonly used. With these 150 popular applications, we determine the number of commonly used Windows applications with an experiment exploring the relation between the number commonly used applications, and the percentage of them showing in the behavior data of the 18 participants, namely the coverage. The results of our experiment is shown in Figure~\ref{fig:process_coverage} with the number commonly used applications in X-axis and the coverage in Y-axis. We choose 100 as the number for commonly used Windows applications as it covers 80\% of all the applications appearing in the data of the 18 participants, while including more popular applications yield little gain in the coverage.


%\begin{figure}
%    \centering
%    \includegraphics[width=0.40\textwidth]{figs/process_coverage.pdf}
%    \caption{Coverage of process V.S. number of popular process}
%    \label{fig:process_coverage}
%\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figs/Process_feature_engineering-cropped.pdf}
    \caption{Process feature engineering procedure}
    \label{fig:process_feature_eng}
\end{figure}

Using process features, we represent each minute of \textit{process information} with process feature vector. This procedure is shown in Figure~\ref{fig:process_feature_eng}. First, we enumerate process information into the applications using file pathname of the executable of each process. Second, for each application, we determine whether it is active using the active intervals of its processes. Third, we present the active status of commonly used applications and the number of active random applications in each minute with a vector. At last, we added time information to each vector by adding two features representing the time of the day and day of the week respectively. Time of the day information is represented using number i representing i-th minute of the 1440 minutes in a day. Day of the week information is represented using number i representing the i-th day of the 7 days in a week starting from Sunday.

%\includegraphics[]{figs/process_coverage.pdf}

\subsubsection{Network Features}

Network features contains two sets of network information: (i) whether the commonly used websites are accessed (access information), and (ii) how many random domains in different countries are accessed (random domain access frequency).

Commonly used websites are the popular websites where computer users access frequently. We choose to use commonly used websites because of the numerous IP addresses and domains recorded in \textit{network information}. Using commonly used websites improves our network information in the following aspects. First, it helps us focus on network activities generated by the user. Among the \textit{network information}, many are activities generated by applications. Commonly used websites help direct our attention to these domains that would be used by the user frequently. Second, it reduces the sparsity in the matrix we generated. Using a exhaustive list of websites, where most websites are not used by most users, will result in most features in the vectors having a value of zero. %Third, 

Similar with random applications, random domains are the domains that only accessed by few users. As the random domains for different users are different, we choose to represent the random domains with the countries where the domain servers resides. This design preserves user specific preference on network usage behavior in the following way. 
%First, As the random domains for different users are different. Random domains captures preserves this information. 
First, users have their own preferred websites from specific countries, e.g., Russian descendents are more likely to visit Russian websites. These differences will be recorded with the different counties where the domain servers reside. Second, the frequency where the random domains are used by different users could be different. The access frequency of random domains captured this information.

Similar with the commonly used processes, the commonly used websites are selected from the websites recorded in Alexa top sites on the web~\cite{Alexa}, hereby called Alexa. We experiment with the first 300 top sites from Alexa. Figure~\ref{fig:network_coverage} shows the measured relation between the number of popular websites (X-axis) and the percentage of them showing in the behavior data of the 18 participants, namely the coverage (Y-axis). We find that popular websites only account for around 22\% of all network IP addresses. However, after We further analyze the rest 80\% of domains and find that, on average, 11.2\% of the remaining domains are actual websites. In another word, commonly used websites include over 76\% of all the recorded websites. The composition of these domains are shown in Figure~\ref{fig:network_ratio}. Over 77.6\% of these domains are servers that are not directly accessible by the user. They are servers for email, marketing, advertising, and etc. 6\% of these domains are web service servers which are mainly used for data exchange with applications. Another 5\% of the remaining IP addresses come from website hosts. Based on our experiments, we choose to include the first 200 popular websites from the Alexa which covers over 70\% of the user accessible domains.

%\begin{figure}
%    \centering
%    \includegraphics[width=0.45\textwidth]{figs/network_coverage.pdf}
%    \caption{Coverage of websites V.S. number of popular websites}
%    \label{fig:network_coverage}
%\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figs/NetworkRatioMono.pdf}
    \caption{The composition of missed Domains}
    \label{fig:network_ratio}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.30\textwidth]{figs/Network_feature_engineering-cropped.pdf}
    \caption{Network feature engineering procedure}
    \label{fig:network_feature_eng}
\end{figure}

The procedure of applying our feature engineering method on network information is illustrated in Figure~\ref{fig:network_feature_eng}. First, we extract the domain names of the remote servers and the countries, which the remote servers reside in, using their IP addresses. 
Then, each minute of network information is represented with a vector. The access information of commonly accessed domains are recorded as whether the 200 Alexa popular websites are visited. The access frequency of random domains are recorded by the different countries where their servers reside. 
At last, we include time information into the vector by add two time features which represents time of the day and day of the week information respectively. Time of the day information is represented using number i representing i-th minute of the 1440 minutes in a day. Day of the week information is represented using number i representing the i-th day of the 7 days in a week starting from Sunday.
%In the case of engineering network information of popular websites, the number of network activities recorded during the minute are represented with the coordinate popular website features. In the case of engineering network information from other servers, the network activities are further batched using the countries where the remote servers reside in. The total number of network activities from different countries are recorded respectively using the country features. The generated network feature vectors are concatenated process and time feature vectors of the same minute to create the vectors describing user per-minute activities.

==> OLD/intro_backup.tex <==
% the definition of concept drift should appear somewhere

Continuous authentication (CA)~\cite{clarke2011transparent} relies on user profiling, the procedure of constructing a behavior-based digital identity of a person. Using behavior-based profiling for security applications involving anomaly detection and authentication is appealing because it requires adversaries to successfully mimic a target’s behavior to evade the security solution, which is arduous. When complemented with other forms of traditional authentication mechanisms (e.g., passwords and security keys), CA can be a game-changer for corporate security. Moreover, depending on the data used for determining user identity, CA has the potential to (i) operate in a non-intrusive fashion, (ii) improve security, as user identity is continuously determined (opposite to point-of-entry approaches), and (iii) provide a more effective measure of user identity  because decisions are not binary.

In this paper, we investigate the feasibility of using computer usage profiling (a form of behavioral biometrics) \cite{bleha1990computer,shepherd1995continuous,Hayashi1997PUISUM,Kim2010MAT} for CA. There are many factors that make computer usage behaviors well-suited for CA. First, personal computer usage profiles have the potential to uniquely characterize a user. This is because, today, it is common for a computer system to be used by a single user and not to be shared. Also, users likely have personalized and temporal consistent (e.g., repeating weekly) computer usage patterns. 
\textit{For example, Bob, middle-aged CEO from a Fortune 500 company, uses his computer very differently from Alice, a young software developer in a tech startup in California. While he mostly uses email reader, office software, browser, and customized company management software, Alice  mostly uses IDE, CAD, and software versioning tools, besides a browser and email reader. Being from Chinese descent, Alice also regularly accesses sites in China.}
Second, the automatic recording of computer usage profiles can be done in a transparent fashion without requiring user intervention, thus facilitating usability and acceptability. Third, in most corporate environments, the recording of computer level activities might not constitute a privacy violation, since most corporate users already have a very limited expectation of privacy \cite{privacy}.  
\todo[inline]{can we remove the example?}

In this paper, we particularly focus on the following research questions and hypotheses:

\textbf{RQ1}: Do individuals have unique computer usage profiles that can be distinguished from one another? 

\textbf{H1}: We hypothesize that computer users have unique usage profiles.

\textbf{RQ2}: Is profile uniqueness sensitive to the observation time?

\textbf{H2}: We hypothesize that profile uniqueness increases with observation time, as more computer usage data become available.

\textbf{RQ3}: Are computer usage profiles consistent over time?

\textbf{H3}: We hypothesized that computer usage profiles are consistent over weeks, since corporate users tend to repeat computer usage on a weekly basis.

To address these questions and test our hypotheses, we conducted an Institutional Review Board (IRB) approved user study to collect computer usage data that we submitted to comprehensive machine learning analysis. Our study enrolled 21 Windows-10 users ($M = 19.74$ yrs, $SD = 2.53$, range: 18-29, 43\% female), recruited via fliers and participant pools on campus. Participants installed a kernel module developed by our research team on their primary personal computers (not shared) to extract their computer usage profiles. Participants were instructed to use their computers naturally during the 21-day study period to assure an ecologically-valid test setting. With user consent, the extractor continuously recorded fine-grained information about system-level activities related to process and network (our definition of usage profile in this study) on the user's computer into log files, which were automatically and securely transferred to our research servers. Activities encompassed processes executed, periods of process activity and inactivity, including file system and network activity.

This data was submitted to machine learning analysis as follows. XXX
\todo[inline, backgroundcolor=blue!50]{Daniela: Luiz, We need here a paragraph summarizing what type of analyses were done.}


There are various proposals for CA tools in the literature using a variety of sensors \cite{bleha1990computer,shepherd1995continuous,Hayashi1997PUISUM,Frank2010AGR,Kim2010MAT,Yang2015Character}, such as mouse and keyboard dynamics, gait, touch, network traffic, etc. This paper does not propose yet another CA mechanism. Our novel contribution is a systematic investigation, based on ecologically-valid user data, and under consideration of the phenomenon of natural temporal changes in profile (concept drift), of the feasibility of computer usage profiling for CA systems. More specifically, compared to prior work, the novelty of our research is threefold. First, user profile data was collected naturally, with users leveraging their own devices in their daily lives, opposite to collection in a lab environment with users performing specific tasks on designed devices. Second, we introduced a novel approach to detect not only the presence, but also the type of concept drift in the usage profiles. Third, our study presents a systematic comparison between multi-class and one-class classification approaches for CA in terms of feasibility and performance, and under the consideration of concept drift aspects (not yet tackled by any of the proposed methods in the literature). We discuss the implications of our results for the development of CA tools and provide recommendations to overcome challenges that such tools may face regarding privacy, concept drift, and adversarial noise, among others. Furthermore, we are making publicly available (upon acceptance of the paper) a profile extracting tool for Windows OS and the de-identified dataset.

Our findings lead to three key conclusions for future behaviour-based CA research and development. First, {\bf computer usage profiles are not consistent over time}. Therefore, concept drift should be considered in the design, implementation and evaluation of CA tools. As discussed in this study, the recurrence of the usage behaviours in corporate environment can be individually influenced by several factors, such as the user’s occupation, occasional trips, days off, etc. For instance, while Alice’s usage profile repeats weekly, Bob’s can repeat biweekly or even monthly. This may suggest that CA  systems  should consider periodical updates  instead of relying on a single training, which points toward online classification for future investigations. Second, {\bf process activity is more relevant to distinguish among profiles than network flow}. Therefore, CA tools will likely experience challenges when users have access to the same applications set, which may happen to employees from the same department in corporate settings. Third, {\bf one-class classification (one independent predicting model per user) is more appropriate than multi-class (a single predicting model for all users) to perform CA in corporate environments}.  
\todo[inline, backgroundcolor=blue!50]{Daniela Oliveira: Luiz, briefly explain why}

In summary, our findings suggest promise for user-centric, behavior-based CA mechanisms by demonstrating that, in general, computer users have unique behaviors. Our results also suggest that CA tools could efficiently complement traditional security mechanisms in corporate environments to flag stealthy, long-duration threats, such as insider attacks and APTs (Advanced Persistent Threats), but further research is necessary to assess the effectiveness of such tools against short-duration threats like malware. Further, future research on handling concept drift in CA is warranted.

The remainder of the paper is organized as follows. Section 2 reviews related work in CA. Section 3 presents the methodology of our user study. Section 4 describes the design and implementation of the computer usage profile extraction tool used in our user study. Section 5 describes the methodology of our machine learning analysis. Section 6 summarizes the results obtained and discusses lessons learned and the study limitations. Finally, section 7 concludes this paper.


\todo[inline, backgroundcolor=blue!50]{Update with paper final structure}




%%% Recent old - 

%Today’s world is digital, people do almost everything using their computers and cellphones (e.g., payments, communication), therefore user authentication plays a key role in terms of security and privacy\todo{Daniela, help}. Most current authentication mechanisms are somehow intrusive and burdensome to users, such as increasingly complex passwords that must be remembered, RFID tokens that must be carried, etc.\todo{add reference}. Moreover, these mechanisms are usually employed in a point-of-entry fashion, that is, performed only once (e.g., entry login). This means that, upon successful authentication, the user has access to the system for unlimited time, which constitutes a potential security vulnerability since the device can be compromised after authenticated\todo{add reference}.

%User-transparent Continuous Authentication (CA) tools have the potential to overcome these limitations as they operate in a non-intrusive fashion and improve security by authenticating the user continuously, not just at the entry login point~\cite{clarke2011transparent}. In this scenario, behavior-based CA is a specific approach that uses the user's behavior to continuously verify their identity throughout a session, so it relies on the existence of unique computer usage profiles\todo{add reference}. Such an approach can be a game-changer for corporate security, complementing traditional mechanisms like passwords. However, despite all the advantages, CA tools have not yet been adopted widely in corporate environments. The major challenges for widespread adoption involve lack of consensus on some important points, such as: what type of data should constitute a user profile, whether profiles can be unique identifiers to users (like unique signatures able to distinguish among them and among malicious activities of the system), and whether profiles are subject to concept drift, which is defined as the phenomenon where the data distribution change over time, affecting the relation between the input data and labels~\cite{Gama:2014:SCD:2597757.2523813}. An example of concept drift in our context would be a change in the user profile related to travel or change of duties within the organization.

%Our long-term research goal is to design an effective behaviour-based CA tool to handle security in corporate environments. As a first step, in order to help inform future design, we conducted an ecologically-valid user study to investigate the feasibility of computer usage profiling. Based on the aforementioned gaps in the literature, this investigation aimed at answering two main research questions under the following hypotheses:

%\begin{itemize}
 % \item RQ1: Do individuals have unique computer usage profiles able to distinguish one another? Is this uniqueness sensitive to the observation time? %and type of corporate scenario?
  %\item H1: We hypothesized that computer users have unique usage profiles, which become more unique with the increase of the observation time, as more usage data become available. %Also, we assumed that profiles are more unique among users with access to different applications than among users with access to the same applications. While the former situation is more likely to happen for large or different departments of a company, the latter could be seen in small departments. For example, Bob, from the advertising department of a tech startup, uses Adobe Photoshop every day from 8am to 2pm, which Alice, from the software engineering department, never uses. Thus, the simple act of using Photoshop can distinguish between Bob and Alice. However, it is not that simple to distinguish Bob from Megan, also from the advertising department, which uses Photoshop every day as well but from 1pm to 5pm. In this case, the temporal patterns in their profiles must be considered.
  %\item RQ2: Are computer usage profiles consistent over time?
  %\item H2: We hypothesized that computer usage profiles are consistent over weeks, since regular users in corporate scenarios usually repeat their usage behaviors on a weekly basis.
%\end{itemize}

%Compared with prior work, the novelty of our research is threefold. First, we implemented an ecologically-valid setting by installing a profile extracting tool on the user's personal computer and recording their usage behavior remotely while they used the computer as they normally would. This allows one to obtain more realistic computer usage data and, therefore, achieve more reliable conclusions compared to classical approaches, such as bringing users to a laboratory \todo[inline]{Daniela, help...} Second, we introduced a novel approach to detect not only the presence but also the type of concept drift in the usage profiles. Third, our study presents a systematic comparison between multi-class and one-class classification approaches for CA in terms of feasibility and performance, and under the consideration of concept drift aspects (not yet tackled by any of the proposed methods in the literature). We discuss the implications of our results for the development of CA tools and provide recommendations to overcome challenges that such tools may face regarding privacy, concept drift, and adversarial noise, among others. Furthermore, we are making publicly available (upon acceptance of the paper) a profile extracting tool for Windows OS and a de-identified dataset.

%Our findings lead to three key conclusions for future behaviour-based CA research and design. First, \textit{computer usage profiles are not consistent over time, so the concept drift factor should be considered}. As discussed in this study, the recurrence of the usage behaviours in corporate environments can be individually influenced by several factors, such as the user’s occupation, occasional trips, days off, etc. For instance, while Alice’s usage profile repeats weekly, Bob’s can repeat biweekly or even monthly. This may suggest that CA systems should consider periodical updates instead of relying on a single training, which points toward online classification for future investigations. Second, \textit{process activity is more relevant to distinguish among profiles than network flow, so CA is more challenging when users have access to the same applications set, which may happen to employees from the same department in corporate settings}. **Discuss some useful insight from this finding**. Third, \textit{one-class classification (one independent predicting model per user) is more appropriate than multi-class (a single predicting model for all users) to perform CA in corporate environments}. **Discuss some useful insight from this finding.** 

%In summary, our findings suggest promise for user-centric, behavior-based CA mechanisms by demonstrating that, in general, computer users have unique behaviors. Our results also suggest that CA tools could efficiently complement traditional security mechanisms in corporate environments to flag stealthy, long-duration threats, such as insider attacks and APTs (Advanced Persistent Threats), but further research is necessary to assess the effectiveness of such tools against short-duration threats like malware \todo[inline]{Daniela, help}. Designing mechanisms to perform behavior-based CA in corporate environments while handling concept drift aspects is a worthwhile direction for future research.

%The remainder of the paper is organized as follows. Section~\ref{sec:related} reviews related work. Section~\ref{sec:user_study} presents the methodology of the user study. Section~\ref{sec:data_extrac} describes the design and implementation of our computer usage profile extraction tool. Section~\ref{sec:ml} describes the methodology of our machine learning analysis. Section~\ref{sec:eval} summarizes the results and discusses lessons learned and the study limitations. Lastly, section~\ref{sec:conclusions} concludes this paper.



% Old version:

% % =================================================================================
% It is common today for a computer system (e.g., desktop, laptop, tablet, or mobile phone) to be used by  a single user and not to be shared. Users of computer systems are diverse and  exhibit unique profiles in the usage of their  computer. 
% %For example, some users just use a browser for their computing needs, while others use computers as part of their work and run specific applications at specific times, including personal and task-oriented software. 
% For example, Bob, middle-aged  CEO from a Fortune 500 company, uses his computer very differently from Alice, a young software developer in a tech startup in California. While he mostly uses email reader, office software, browser, and customized company management software, Alice  mostly uses  IDE, CAD, and software versioning tools, besides a browser and email reader. Being from Chinese descent, Alice  also  regularly accesses sites in China. 
% %On some days, she works from home using VPN and VNC to access her company’s computational resources. 

% Behavior-based continuous authentication relies on the existence of behavioral user profiles. Such authentication method can be a game-changer for corporate security, effectively complementing traditional authentication mechanisms, such as passwords. Most current authentication mechanisms are employed in a point-of-entry fashion (e.g., performed once) and are  usually  intrusive and burdensome to users (e.g, passwords that have to be remembered, RFID tokens that can be lost, etc.). Moreover, upon successful point-of-entry authentication, the user has access to the system for unlimited time, without having to re-authenticate. This constitutes a potential security vulnerability, if the user device is compromised after successful point-of-entry authentication. Continuous and user-transparent authentication tools have the potential to address these vulnerabilities~\cite{clarke2011transparent} in the following ways:  (i) they operate in a non-intrusive fashion, (ii) they improve security, as users are continuously authenticated, and (iii) they provide a more effective measure of user identity  because the decisions are not binary. Despite these advantages, continuous authentication mechanisms have not yet been  adopted widely in corporate environments. The major challenges for widespread adoption are a lack of consensus on (i) what type of data should constitute a user profile, (ii) whether user behavior naturally changes overtime (concept drift), and (iii) how to record user data in a user-transparent, secure, and private fashion.

% %Major impedances for  adoption, of such mechanisms is the challenges in (i) determining  what type of data distinguishes a user from other users or other uses of the system (e.g., malware), (ii) whether user profiles are consistent overtime, and (iii) how to record user profile in user-transparently, secure and privacy-aware fashion.

% Based on these considerations, there are three pressing questions that the research and development community on behavior-based continuous authentication needs to answer: \textit{“(i) Do individuals have unique computer usage profiles?;  (ii) Are these profiles distinguishable (among users and malicious uses of the system)?, and (iii) Are these profiles consistent over time?''}

% % We hypothesize that computer usage behavior across all layers of abstraction that make up a computer system is unique to the user as if it constituted a \textit{signature}. Moreover, such unique profiles, if existent, could be potentially successfully leveraged in the development of the next generation of efficient and effective continuous authentication systems based on user behavior. 
% To address these questions, we conducted an Institutional Review Board (IRB) approved user study to collect computer usage data that we  submitted to comprehensive machine learning analysis to test the hypothesis that computer users have unique, distinguishable computer usage profiles, which are consistent overtime. Our study enrolled 21 Windows 10 users ($M = 19.74$ yrs, $SD = 2.53$, range: 18-29, 43\% female), recruited via fliers and participant pools on campus. Participants installed a kernel profile extractor developed by our research team on their primary personal computers (not shared). They were instructed to use their computers naturally during the 21-day study period to assure an ecologically-valid test setting. The extractor recorded  (with user consent)  in log files (on a continuous basis) fine-grained information about all system-level activities  on the user's desktop. This data was automatically and securely transferred to our research  servers. Activities encompassed processes executed, periods of process activity and inactivity, including  file system and network activity. 

% We conducted machine learning  analysis on this data to determine the  uniqueness of  user profiles, i.e., the extent to which a profile is distinguishable  from  other users' profiles.  In particular, we analyzed the data using three classification methods: (i) a newly proposed Bidirectional Attention Long Short-Term Memory (BA-LSTM), (ii) Support Vector Machine (SVM), and (iii) Random Forest combined with voting (Random Forest-V). For BA-LSTM, we included an attention mechanism to improve analysis of long input data sequences. %For Random Forest-V, we introduced a method to distinguish  users through voting.
% %, which allows us to predict a single user without having a fixed time window (we can also change it on the fly in the future), making faster decisions -- this method is classifier independent, i.e., it can be used with any classifier. 
% Our classification analysis considered different user group sizes and observation windows. We also used Self-Organizing Maps (SOM) for visualization of profile uniqueness  and for presentation of concept drift -- naturally occurring benign changes in user profile over the study period (e.g., travel or changes in responsibility in organization).  

% Results were highly consistent across all three classifiers. All methods reached over 90\% accuracy in determining user identify  for all user groups sizes with  observation windows longer than  10 minutes. For all group sizes, classification accuracy increased with longer observation windows. However, accuracy decreased slightly with greater group sizes. SOM provided visual indication of the uniqueness of the profiles and  suggested that some users exhibited concept drift over the study period. 
% %We found that the users for which the  classifier provided highest confidence in determining identity (almost 100\% confidence) usually presented usage profiles that did practically did not change week by week. On the other hand, the three users in our cohort for which the classifier presented lowest confidence (lower than 80\%) were those users whose usage profile during training and testing weeks differed considerably. 
% Our findings suggest promise for user-centric, behavior-based continuous  authentication  mechanisms by demonstrating that users exhibit, in general, distinct computer usage profiles, which are  robust over time (i.e., repeated weekly over the three-week study period). To the best of our knowledge, this is the first systematic investigation of  the feasibility of computer usage profiling for continuous authentication, using data generated in an ecologically-valid setting considering concept drift. 
% %While cross-layer, hyper-dimensional continuous authentication systems are promising in profiling users, they should always be part of a multi-factor authentication and anomaly-detection framework inside organizations, which also includes traditional mechanisms such, as passwords and antivirus. 
% Based on our findings, we propose that behavior-based continuous authentication tools could efficiently complement traditional security mechanisms in corporate environment to flag stealthy, long-duration threats, such as insider attacks, APTs (Advanced Persistent Threats). Our paper  contributes to scientific advancement and holds potential for practical impact in the following ways:



% %The BA-LSTM classifier achieve 92\% of accuracy at distinguishing 10 users using windows of 5 minutes. For any given amount of users, the accuracy will increase when longer window of time are analyzed with the accuracy ranging from 85\% to 99\%. In any given window of time, the accuracy will decrease as more people are considered with the accuracy ranges from 86\% to 98\%. 
% %Our RF-V classifier achieves 91\% of accuracy at distinguishing 10 users using windows of 5 minutes. For any given amount of users, the accuracy will increase when longer window of time are analyzed with the accuracy ranging from 87\% to 98\%. In any given window of time, the accuracy will decrease as more people are considered with the accuracy ranges from 89\% to 97\%. 
% %For SVM we found similar results as BA-LSTM and RF. SVM achieves 90\% of accuracy at distinguishing 10 users using windows of 5 minutes. For any given amount of users, the accuracy will increase when longer window of time are analyzed with the accuracy ranging from 86\% to 98\%. In any given window of time, the accuracy will decrease as more people are considered with the accuracy ranging from 87\% to 95\%.




% % This paper presents the following contributions: \ToDo{Nikos: contributions look ugly. You talk about ML in both i and iii. Normally, you start from the beginning in contribution i (for us extractor), and then you end up to the evaluation and discussion. }
% % \begin{enumerate}[label=\roman*]
% %     \item We describe the methodology and present results from a comprehensive analysis using machine learning and deep learning methods of an ecologically-valid user study testing the extent to which computer usage profiles are unique and can accurately identify computer users when leveraged in behavioral-based continuous authentication tools.
% %     \item We present a computer usage profile extracting tool\footnote{This extracting tool will be publicly available  at GitHub upon paper publication.} for Windows OS that can be leveraged in the development of continuous authentication tools based on users' computer usage profiles.
% %     \item We introduce a novel Bidirectional-Attention LSTM (BA-LSTM) that incorporates a  bidirectional architecture and an attention mechanism for analysis of long sequences of time series data, such as those encountered in user profiling.
% %     \item{ We discuss the implications of our findings for the next generation of user-centered continuous authentication tools and provide recommendations based on the lessons we learned, including a discussion of which features our methods found more relevant for distinguishing computer user behaviors.}
% % \end{enumerate}

% % This paper presents the following contributions:
% % \begin{enumerate}[label=\roman*]
% %     \item We describe a pioneering method of profiling the computer user using their per-minute computer usage information on process and network, which can be leveraged in behavioral-based continuous authentication tools.
% %     \item  We present a computer usage profile extracting tool\footnote{This extracting tool will be publicly available at GitHub upon paper publication.} for Windows OS and used it in ecologically-valid user study.
% %     \item We introduce a novel Bidirectional-Attention LSTM (BA-LSTM) that incorporates a  bidirectional architecture and an attention mechanism for analysis of long sequences of time series data, such as those encountered in user profiling.
% %     \item We testing the extent to which the user profiles generated from SOM, BA-LSTM, SVM and RF-V are unique and can accurately identify computer users when leveraged in behavior-based continuous authentication tools.
% %     \item We discuss the implications of our findings for the next generation of user-centered continuous authentication tools and provide recommendations based on the lessons we learned, including a discussion of which features our methods found more relevant for distinguishing computer user behaviors.
% % \end{enumerate}

% %In summary, in this paper we design a pioneering \textit{user profiling} framework that creates a multi-dimensional digital user signature based on various system level information and across different layers of abstractions. Further, we show that our framework can be leveraged in next generation behavioral-based continuous authentication tools. {To the best of our knowledge, this is the first work that does so, opening new horizons for user profilers and continuous authenticators}. 

% \begin{packed_enum}

% \item It describes the methodology of an ecologically-valid user study and presents results from  a comprehensive analysis using different machine learning methods showing that computer usage profiles \footnote{A de-identified dataset will be made publicly available upon acceptance of the paper.}  are unique, consistent overtime and allow accurate identification of  users  for behavior-based continuous authentication.

% \item It presents a computer usage profile extracting tool \footnote{To be made publicly available upon acceptance of the paper.}
% for Windows OS that extracts fine-grained information about process (including file-system) and network activities.

% \item  It introduces a novel BA-LSTM that incorporates a bidirectional architecture and an attention mechanism, for analysis of long sequences of time series data, such as  generated in our user study.

% \item  It discusses the implications of our findings for the development of the next generation of  behavior-based continuous authentication tools and provides recommendations for overcoming challenges such tools will face regarding privacy, concept drift, and adversarial noise introduced during generation of training data.

% \end{packed_enum}
%  %   \item \noindent We developed a computer usage profile extracting tool\footnote{This extracting tool will be publicly available at GitHub upon paper publication.} for Windows OS that collects various process-related, process-related, file-related information at the OS level with minimal overhead.
%   %  \noindent  \item We conduct an ecologically-valid user study using the computer usage profile extractor for 18 participants for a period of 21 days.
%   % \noindent  \item We introduce Bidirectional-Attention LSTM (BA-LSTM), a novel deep learning method, that incorporates a bidirectional architecture and an attention mechanism for analysis of long sequences of time series data, such as those encountered in our problem.
%   % \noindent  \item Using BA-LSTM, and three ML methods (OM, SVM and RF-V), we test to which extent the users of our study are distinguishable. We find that our framework can distinguish users with accuracy up to $98.3\%$.%We analyze to what extent the user profiles generated from SOM, BA-LSTM, SVM and RF-V are unique and can accurately identify computer users when leveraged in behavior-based continuous authentication tools. 
%     %\noindent   \item We discuss the implications of our findings for the next generation user-centric continuous authentication tools and shed some light on the involved dependencies and tradeoffs regarding the optimization on window length and selection of machine learning/deep learning methods.\ToDo{an example?}.%, e.g., different features contribute differently on the user profiling decision, following the data coming not only from that user but also the other ones. %We discuss the implications of our findings for the next generation user-centric continuous authentication tools and provide recommendations based on the lessons we learned, including a discussion of which features our methods found more relevant for distinguishing computer user behaviors.
% %\end{enumerate}


% The remainder of the paper is organized as follows. Section~\ref{sec:user_study} presents the methodology of the user study. Section~\ref{sec:data_extrac} describes the design and implementation of our computer usage profile extraction tool. Section~\ref{sec:ml} describes the methodology of our machine learning analysis. Section~\ref{sec:eval} summarizes the results and discusses lessons learned and the study limitations. Section~\ref{sec:related} reviews related work and Section~\ref{sec:conclusions} concludes this paper.



==> OLD/methods.tex <==
%\Todo{This section describes the Long Short-Term Memory (LSTM) for computer usage profile generation. LSTM RNN is designed to analyze data sequence with long term dependencies~\cite{Hochreiter1997LSTM}. This feature of LSTM RNN make it an ideal candidate for generating user profile from time sequence of user activities. To further improve its performance, we adopted the following optimization method in our LSTM RNN. }

%This section describes the feature engineering methods and Bidirectional Attention Long Short-Term Memory (BA-LSTM) used to analyze the computer usage behavior profiles. 





%\subsection{Time Features}

%Time features represent the daily schedule of computer users in using their computers. There are two set of time related features that we believe to have major impact on user activity: time of the day information and day of the week information. Time of the day information represents the time the event is recorded in 24 hour format. This set of features reflect the user’s daily schedule in using computer. Day of the week information represents the correspond weekday the event is recorded. This feature set tries to help the anomaly detector to discover users computer using routine on the different weekdays. 

%Time features are generated from the time stamps we collected in \textit{process} and \textit{network information}. When \textit{process} and \textit{network information} is engineered by minute, we extract the time of the day information and day of the week information from it, and store them in the form of time feature vectors. The generated time feature vectors are concatenated process and network feature vectors of the same minute to create the vectors describing user per-minute activities.

       
%\subsection{Bidirectional Attention Long Short-Term Memory}

We build Bidirectional Attention Long Short-Term Memory (BA-LSTM) to distinguish different computer users based on their computer usage information. We choose LSTM as it is designed to exploit long term correlation in the input sequences. This make LSTM robust in analyzing time series data. To further improve the capability of LSTM in modeling the user with long sequence of time series data, we implement bidirectional and attention mechanism in BA-LSTM.


\subsection{Bi-directional Mechanism}
%One of the methods used in this project is based on long short-term memory or LSTM.
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figs/data_sequnce-cropped.pdf}
    \caption{Data sequence with time step of T}
    \label{fig:data_seq}
\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=0.45\textwidth]{figs/LSTM_node-cropped.pdf}
%    \caption{LSTM node showing bidirectional LSTM}
%    \label{fig:lstm_structure}
%\end{figure}

The original LSTM~\cite{Hochreiter1997LSTM} is well known for modeling input sequence of information in one direction. 
%The structure of a LSTM node is shown in Figure~\ref{fig:lstm_structure}. 
If the correlation information from both directions of the sequence are considered, such models can be further improved. For a given sequence with time step
$x_t, t\in [0,T]$ (shown in Figure~\ref{fig:data_seq}), We use Bi-directional LSTM~\cite{schuster1997bidirectional} to get 
%annotations
representation of time steps by summarizing information from both directions of the sequence, and therefore the contextual information from both direction can be incorporated in the representation. Our bidirectional LSTM contains a forward LSTM $\overrightarrow{f}$ which reads the sequence $x$ from $x_0$ to $x_t$ and a backward LSTM $\overleftarrow{f}$ which reads from $x_t$ to $x_0$. 

Compared with original LSTM, Bi-directional LSTM learns more comprehensive representation of different computer users. In additional to be able of capturing the situations where usage activities at early time point triggers another activity later in the time sequence, bi-directional LSTM also considers a later usage activities as successor of former computer usage activities.

%Thus, for each hidden layer in bidirectional LSTM, we have representation of the $t$th node:
%\begin{align}
	%\overrightarrow{h_t} &= LSTM(x_t,h_{t-1}), t\in [0,T], \\
	%\overleftarrow{h_t} &= LSTM(x_t,h_{t+1}), t\in [T,0].
%\end{align}
%Where $h_t$ is the $t$th hidden state of LSTM, and is also used to construct the representation for input $x_t$. $h_{-1}$ in forward LSTM and $h_{T+1}$ in backward LSTM are both 0.\\
%The structure of bidirectional LSTM is shown in Figure~\ref{fig:lstm_structure}.\\
%We obtain an final representation state $h_t$ for a given time step $x_t$ by
%concatenating the forward hidden state $\overrightarrow{h_t}$ and
%backward hidden state $\overleftarrow{h_t}$, i.e.,


%\begin{equation}
	%h_t = 
	%\begin{bmatrix}
	%\overrightarrow{h_t} \\
	%\overleftarrow{h_t}
	%\end{bmatrix},
%\end{equation}
%which summarizes the information of the whole sequence centered around time step $x_t$.

\subsection{Attention Mechanism}

%\begin{figure}
%    \centering
%    \includegraphics[width=0.50\textwidth]{figs/attention_layer.pdf}
%    \caption{Attention layer of LSTM}
%    \label{fig:attention_layer}
%\end{figure}

Not all time steps in a sequence contribute equally to the representation of the sequence. Hence, we introduce attention mechanism to emphasize time steps (receiving more weight) that are important to the characteristics of the sequence and aggregate the representation of those informative time steps to form a sequence.

Attention mechanism estimated the distribution of the contribution of each time steps to distinguish the users and emphasize (given more weight in producing output) on those time steps that diverge among the computer users. More precisely, attention mechanism improve the classification capability of LSTM in the following two aspects. First, it helps filter out the time steps where most activities are generated by Windows OS. Second, attention mechanism improves classification accuracy by emphasize more on the time steps that display the difference among different users. 

%The attention structure is shown in Figure~\ref{fig:attention_layer}.
%Specifically, we have the attention layer constructed as:
%\begin{align}
%u_t &= \tanh (W_sh_t + b_s), \\
%\alpha_t &= \frac{\exp(u_t^T \mu_s)}{\sum_{t=0}^{T} \exp(u_t^T \mu_s)}, \label{eq:alpha_t} \\
%v &= \sum\limits_{t=0}^{T} \alpha_t h_t. \label{eq:v}
%\end{align}

%That is, we first feed the time step annotation $h_t$ through
%a one-layer Multilayer Perceptron~\cite{rosenblatt1961principles} to get $u_t$ as a hidden representation of $h_t$, then we measure the importance of the sequence time step as the similarity of $u_t$ with a time step level context vector $\mu_s$ and get a normalized importance weight $\alpha_t$ through a softmax~\cite{nasrabadi2007pattern} function. After that, we compute the sequence vector $v$ as a weighted sum of the time step annotations based on the weights. The context vector $\mu_s$ can be seen as a high level representation of a fixed query "what is the signature or informative time step" over the time steps like that used in memory networks~\cite{sukhbaatar2015end, kumar2016ask}. The time step context vector $\mu_s$ is randomly initialized and jointly learned during the training process.





==> _spine.tex <==

% =============== ESPINHA DORSAL DO PAPER ===============

Link aqui:
% https://docs.google.com/document/d/1eBgHcgATjljEYhNs_gcxKX1NkBtqmgDsDWoNMLNpC74/edit?usp=sharing


1. Coletamos os dados (ahh, jura?)
2. Tentamos diferenciar os users com ML pra ver se os nossos dados são bons pra computer usage profiling (i.e., são capazes de criar perfis únicos).
---> Usamos online ML porque <justifique aqui>
---> Testamos diferentes tamanhos de janela pra estimar quanto tempo um sistema de cont auth precisaria pra funcionar
- Usando o melhor tamanho de janela, tentamos investigar e explicar concept drift a partir de imagens SOM e top features

% ====================================================================
Solution Papers
JSys invites papers that present a new solution to a well-known problem. Solution papers are the closest to regular research papers in traditional conferences, and will be judged on how they improve the state-of-the-art.

Artifact Evaluation. Unlike regular conferences where artifact evaluation is optional, it is mandatory for solution papers. The solution must be realized in the form of an artifact, which must be publicly available and evaluated to be easily used by a third party. In this way, it will always be possible for someone else to build on, extend, or evaluate a JSys Solution paper.

Solution papers may be rejected for:
Not establishing how the solution improves the state-of-the-art
Not differentiating the solution from prior work attaching the same problem

Desk Rejections:
Not providing the artifact as open-source for Artifact Evaluation

Guideline for authors:
Prefix the title of these papers with “Solution:”
Check the Solution checkbox on the submission form to flag them for the review process

==> discussion-backup.tex <==

This section discusses study findings and limitations in testing computer usage profiles uniqueness (\textbf{RQ1}) and temporal consistency (\textbf{RQ3}), as well as top characteristics for determining unique profiles (\textbf{RQ2}). We also discuss challenges and opportunities of computer usage profiling for applications in CA.

%This section discusses study findings and limitations in testing computer usage profiling feasibility as well as profiles uniqueness (\textbf{RQ1}) and temporal consistency (\textbf{RQ2}). We also discuss future work.

%\subsubsection{Computer Usage Profiles Uniqueness}
%\label{sec:prof_uniqueness}
%\textbf{Computer Usage Profiles Uniqueness}
\subsection{Computer Usage Profiles Uniqueness}

%Our results partially supported \textbf{H1} in that unique computer usage profiles exist. More specifically, we found support only for Scenario 1 (all processes considered), which yielded promising accuracy rates with both classification approaches on average ($M = 86.3\%$ for multi-class and $M = 73.4\%$ for one-class). On the other hand, accuracy rates for Scenario 2 (only applications used by all users considered) did not suggest uniqueness in the computer usage profiles ($M = 39.5\%$ for multi-class and $M = 59.1\%$ for one-class). As prediction is more challenging in the presence of commonalities, we already expected worse results for Scenario 2.

%These findings suggest that computer users can be distinguished from one another as long as they show some variation in the types of applications used, that is, their applications are not restricted to predefined set. In other words, behavior-based CA systems are more likely to experience challenges in environments such as small departments or groups, where it is common for users to use systems with the same set of applications pre-installed, compared to large and diverse environments, where more diversity is expected in terms of software usage among computer users.  \linebreak

%This finding suggest that computer users can be distinguished from one another as long as they can use different applications, that is, not restricted to use a standard software set. In other words, behavior-based CA systems are more likely to experience challenges in environments like small departments of corporations, where is common for users to get a standard set of applications installed on their computers, compared to large or different departments, where more diversity is expected in terms of software usage among users. \hl{For example, Megan and John, from the marketing department of a company, use Adobe Photoshop every day, which Alice and Bob, from the software engineering department, never use}. \todo{keep or remove?}

%Our results partially supported the notion that computer usage profiles are unique. We found support only with % Scenario 1 with 
%the multi-class models, which resulted promising performances, but still below the expected for a CA solution. %The performances observed in all other experiments seem low for authentication systems and therefore do not suggest uniqueness in profiles. 
%Conversely, with the one-class models, we found an overall average F-score below 50\%, which means that tossing a coin would provide better chances of correctly classifying a given user. Such performance is significantly low for a CA system and therefore do not suggest uniqueness in profiles. %The performances observed for the one-class models are significantly low for a CA system and therefore do not suggest uniqueness in profiles. 


Our results from \textbf{RQ1} \emph{partially} supported the notion that computer usage profiles comprised of process- and network-related events plus \# of mouse clicks and keystrokes constitute an useful and feasible source of data to uniquely characterize computer users. This is because, while most of the tested machine learning classifiers yielded promising results (F-scores greater than 94\% with the offline models and greater than 99\% with the online models), the one-class models achieved poor results in both offline (maximum F-score of 66.23\%) and online (maximum F-score of 0.03\%) settings. The reason behind such a poor result for the online one-class model is that it works better when anomalous data are rare, which is the opposite of our scenario~\cite{10.5555/2283516.2283647}. In other words, our profiles can be considered unique depending on the learning model used for the recognition task. Importantly, our top feature analysis (\textbf{RQ2}) revealed that the websites accessed by the computer users was more relevant to distinguish them from one another compared to the processes that they used and the \# of mouse clicks and keystrokes that they performed. All these findings suggest that our definition of computer usage profile---specially the component related to network traffic--- has the potential to be leveraged by CA mechanisms based either on offline or online classifiers in both multi-class and binary settings to recognize computer users.

\medskip
\takeaway{Computer usage profiles encompassing process- and network-related events plus \# of mouse clicks and keystrokes have the potential to uniquely characterize computer users when analyzed with offline and online classifiers in both multi-class and binary settings, with network events constituting the most useful source of information to distinguish among users.}


%\commentario{In other words, the Half-Space Trees model did not seem suitable to handle computer usage profiles}.
%In other words, our findings suggest that our definition of computer usage profile has the potential to be leveraged by CA mechanisms based either on offline or online classifiers in both multi-class and binary settings.
%the websites visited by the computer users were more relevant to distinguish among them than 






%Our results partially supported the notion that computer usage profiles are unique. With the one-class models, we found an overall average F-score below 50\%, which do not suggest uniqueness in the profiles since tossing a coin would provide better chances of correctly classifying a given user. However, the multi-class models resulted promising performances (average F-score of 88.8\% in the best case), but still below the expected for a CA solution. These findings suggest that \textbf{our definition of computer usage profiling -- via process- and network-related events -- has the potential to uniquely characterize computer users and could be complemented with other types of events, such as mouse clicks and keystrokes, to improve profile uniqueness}.



% \luiz{These findings suggest that our definition of computer usage profiling has the potential to uniquely characterize computer users, but it is not feasible for CA when combined with either one-class or multi-class classification individually. On the one hand, the multi-class models outperformed the one-class models in terms of accurate predictions, but they are not practical because they need to be trained with data from all users. In this case, the learning model would need to be retrained every time a user is added or removed from the group (e.g., employee turnover). On the other hand, the one-class approach seems more realistic for applications in organizations because training occurs on a per-user basis, so there is no need to retrain all existing models when a user is added/removed. Also, one independent model for each user allows to handle temporal changes in profiles on a per-user basis, which is interesting given that these changes seem to be user specific (as discussed in the following), likely depending on factors like travel, role, etc. %On the other hand, the one-class approach seems more realistic for applications in corporate settings due to practical reasons, for example, no need to retrain all existing models every time a new user is added/removed from the group, and one independent model for each user which allows to handle temporal changes in profiles on a per-user basis. 
% Thus, it is possible to speculate that a hybrid solution combining aspects from the multi-class and one-class approaches could be able to deal with practical needs and also reach accurate predictions. Performance could also be improved if using other relevant information for computer usage profiling (e.g., keystrokes and mouse dynamics) along with process and network activity. }

%On the one hand, the one-class approach seems more realistic for applications in corporate settings due to practical reasons, such as no need to retrain existing models every time a new user is added/removed from the group, and one independent model for each user which allows to handle temporal changes in profiles on a per-user basis. On the other hand, multi-class classification outperformed one-class in terms of performance.
%has shown to be superior in terms of performance, but the results did not seem promising for a CA tool in any of the experiments. 
%Our findings point toward future research on hybrid approaches able to reach more accurate predictions while handle users in an individual and robust fashion. Future research on other useful information (e.g., keyboard and mouse dynamics) to be used along with process and network activity for computer usage profiling is also warranted

%Moreover, we found worse results for Scenario 2 (considering only common processes) compared to Scenario 1 (considering all processes) with both classification approaches. This was already expected since the use of only common processes among users brings more commonalities to the computer usage profiles, making predictions more challenging. These findings might suggest that behavior-based CA systems are more likely to experience challenges in environments such as small departments or groups, where it is common for users to use systems with the same set of applications pre-installed, compared to large and diverse environments, where more diversity is expected in terms of software usage among users. \\


%\subsubsection{Computer Usage Profiles Consistency}
%\label{sec:drift}
\subsection{Computer Usage Profiles Consistency}

%Our approach for the categorization of concept drift has shown to be accurate under artificial test data, as the SOM images and classification curves behaved as expected in all simulated situations (see Figure \ref{fig:fake_data}). As expected, while both methods were able to display presence of drift, only the curves proposed in this study allowed the identification of the drift type. Although these results are encouraging, our test data may not precisely reproduce the concept drifts found in real usage data, so it is more reasonable to assume that the approach can only infer -- and not securely determine -- type of drift in computer usage profiles. Moreover, the approach exhibited a few limitations under real data, as it was not able to categorize two participants in both experimental scenarios. In these cases, SOM suggested presence of drift over the weeks, while the curves did not, so it is possible to speculate that the former is more sensitive to the presence of concept drift than the latter.

%Our results suggest that most of our participants exhibited some type of concept drift during the study period in both experimental scenarios (see Table \ref{tab:drift_summary}), which did not support \textbf{H3} that computer users repeat usage behaviors weekly. These results likely reflect real corporate settings, where many factors can randomly affect the temporal consistency of usage behaviors, such as occasional business travels, days off, change of duties, among others. Furthermore, depending on the user's occupation, the usage profile can reoccur on a biweekly or even monthly basis, for example. Under this consideration, we might not have detected real concept drifts for certain users, but normal (benign) behavioral changes that may belong to a usage pattern if observed over a period longer than 1 week. 

Our approach for the categorization of temporal changes in computer usage profiles was accurate in our test with artificial data as the SOM results and classification curves behaved as expected for all simulations. However, as these datasets were artificially created by combining data from different participants, they may not precisely reproduce temporal changes found in real usage data. %Therefore, it might be more reasonable to presume that such approach can infer -- and not determine -- type of concept drift for computer users.


Under these considerations, \textbf{we found that profiles were not consistent over the study weeks for the better part of our sample (82.4\% of study participants)}.
%, with 82.4\% of the users experiencing concept drift. 
%for 82.4\% of our participants. 
Surprisingly, we observed that profile uniqueness did not increase with time as more usage data become available, but oscillate over time (Tables~\ref{tab:acc_multi_sc1} and \ref{tab:acc_one_sc1}). %, likely depending on the users’ activity. %(e.g., which processes were used and which network connections were made during a given period).
We also found that the pattern of temporal change is user-specific, since we observed all the four types of concept drift for the users (Table \ref{tab:drift_per_user}). These results might reflect real organizations and \commentario{corporate} settings, where many factors can affect profile temporal consistency such as travels, holidays, and change of role. %Interestingly, 23.5\% of the users were assigned different types of drift between the two Scenarios. This suggests that restricting the access of computer users may affect the temporal consistency of their usage patterns.

%In summary, our findings suggest that off-line learning approaches (training occurring once) may not be ideal for a behavior-based CA system. Alternatively, online approaches may reach better results, as the learning model can be periodically updated, thus capturing changes in usage behavior. Indeed, the literature discusses online supervised methods to handle concept drift, such as the Drift Detection Method~\cite{gama2004} and the Early Drift Detection Method~\cite{baena2006}. They are both based on sequential error monitoring, that is, if the model starts misclassifying, it is assumed that a concept drift might be taking place, which is the same logic that we adopted to analyze our classification curves.

%Our findings also suggest that CA tools with mechanisms to handle temporal changes in profiles should be prepared to experience different patterns of change, which may be influenced by restrictions in software usage imposed to users. So, as a practical recommendation, such systems might need to be adjusted or fine-tuned for the environment in which they operate for better results. For example, while incremental drifts occur slowly/gradually, the other types of drift involve abrupt changes that need to be quickly handled. This poses a major challenge because such abrupt switches can also be caused by outliers or noise in the data, which do not refer to concept drift, but to a once-off random change or anomaly~\cite{gama2014survey}.\linebreak

In summary, our findings led to two main conclusions. First, off-line learning approaches (training occurring once) may not be ideal for a behavior-based CA system. Alternatively, online approaches may reach better results, as the learning model can be periodically updated, thus capturing changes in usage behavior. Indeed, the literature discusses online supervised methods to handle concept drift, such as the Drift Detection Method~\cite{gama2004} and the Early Drift Detection Method~\cite{baena2006}. They are both based on sequential error monitoring, that is, if the model starts misclassifying, it is assumed that a concept drift might be taking place, which is the same logic that we adopted to analyze our classification curves. Second, CA tools with mechanisms to handle temporal changes in profiles should be prepared to experience different patterns of change. %, which may be influenced by restrictions in software usage imposed to users. 
So, as a practical recommendation, such systems might need to be adjusted or fine-tuned for the environment in which they operate for better results. For example, while incremental drifts occur slowly/gradually, the other types of drift involve abrupt changes that need to be quickly handled. %This poses a major challenge because such abrupt switches can also be caused by outliers or noise in the data, which do not refer to concept drift, but to a once-off random change or anomaly~\cite{gama2014survey}.\linebreak




%\subsubsection{Computer Usage Profiling Feasibility}
%\textbf{Computer Usage Profiling Feasibility}

%\luiz{Our results indicate that our definition of computer usage profiling is not feasible when analyzed via either one-class or multi-class classification individually. On the one hand, the one-class approach seems more realistic for applications in corporate settings due to its robustness to changes compared to multi-class as follows: no need to retrain existing models every time a new user is added/removed from the group, and one independent model for each user which allows to handle temporal changes in profiles on a per-user basis. On the other hand, multi-class classification has shown to be superior in terms of performance, but the results did not seem promising for a CA tool in any of the test scenarios. These findings point toward future research on hybrid approaches able to reach more accurate predictions while handling users in a robust and individual fashion. Future research on other useful information (e.g., keyboard and mouse dynamics) to be used along with process and network activity for computer usage profiling is also warranted}. \\


%Our results indicate that one-class classification is more feasible than multi-class for behavior-based CA. First, the one-class models performed slightly worse than the multi-class models for Scenario 1 (all processes considered), but moderately better for Scenario 2 (only applications used by all users considered). Second, the one-class approach is more realistic for applications in corporate settings as it provides one independent model for each user, therefore being more robust to changes (no need to retrain existing models every time a new user is added/removed from the group) and more suitable to handle temporal changes in profiles in a per-user basis. \linebreak
%individually, considering the particularities of each user. Such things are not possible with regular multi-class classifiers.

%Compared to related work, our profiling approach seems promising. A similar study reported an equal error rate of around 20\% with the use of one-class SVM, replicator neural network, and probabilistic similarity under system-level events collected from seven computer users in a controlled environment~\cite{Payne2013SEMAA}. Their solution is potentially resource hungry, as each user generated two to four GB of data in two hours. Compared to that study, our proposal of computer usage profiling seems more feasible, as we achieved competitive results with participants generating only 0.17 to 8.03 MB of data over a 21-days period (see Appendix~\ref{sec:appendix_amountdata}). The lack of other similar studies -- with a similar design of computer usage profiling -- prevented us from making further comparisons of our results.


% %\subsubsection{Privacy Aspects}
% \textbf{Privacy}

% One challenge of leveraging computer usage profiling for CA is that the recording and determination of profiles can be perceived as privacy-invasive. To address this concern, profile extracting tools should operate in the less invasive fashion, without recording personally identifiable information such as file contents or keys typed by users. Nevertheless, some users might still feel uncomfortable with having their system events being recorded. However, it is important to point out that, in corporate environments, expectations of privacy are very limited~\cite{privacy}. Often, employees are fully aware that nearly all their activities inside the organization perimeter are monitored and recorded. For example, many organizations have their employees agree on usage policies, such as %using corporate email only for business purposes, and 
% having their email and computer usage monitored~\cite{privacy}. 

\subsection{Computer Usage Profiling Feasibility}

In summary, our findings suggest that computer usage profiles comprised of user-initiated process and network events have the potential do uniquely characterize computer users (\textbf{RQ1}) and are not consistent over time (\textbf{RQ2}). On the one hand, the multi-class models outperformed the one-class models in terms of accurate predictions, but they are not practical because they need to be trained with data from all users. In this case, the learning model would need to be retrained every time a user is added or removed from the group (e.g., employee turnover). On the other hand, the one-class approach seems more realistic for applications in organizations because training occurs on a per-user basis, so there is no need to retrain all existing models when a user is added/removed. Also, one independent model for each user allows to handle temporal changes in profiles on a per-user basis, which is interesting given that these changes seem to be user specific (as discussed in the following), likely depending on factors like travel, role, etc. Even so, none of the approaches (multi-class or one-class) is suitable to properly handle temporal changes in profiles because both are off-line, that is, the learning model is trained only once, thus missing eventual behavioral changes that might take place over time.

We therefore concluded that, \textbf{if combined with either one-class or multi-class classification models individually, our definition of computer usage profiling is not feasible for CA}. We speculate that a hybrid solution combining aspects from multi-class and one-class approaches might be able to perform accurate predictions and also deal with practical needs of groups and organizations, such as independent models for users. As mentioned, online learning aspects could also be investigated to handle concept drift in the profiles via the periodical retraining of the model.


% These findings suggest that our definition of computer usage profiling has the potential to uniquely characterize computer users, but it is not feasible for CA when combined with either one-class or multi-class classification individually. 
% On the one hand, the multi-class models outperformed the one-class models in terms of accurate predictions, but they are not practical because they need to be trained with data from all users. In this case, the learning model would need to be retrained every time a user is added or removed from the group (e.g., employee turnover). On the other hand, the one-class approach seems more realistic for applications in organizations because training occurs on a per-user basis, so there is no need to retrain all existing models when a user is added/removed. Also, one independent model for each user allows to handle temporal changes in profiles on a per-user basis, which is interesting given that these changes seem to be user specific (as discussed in the following), likely depending on factors like travel, role, etc. %On the other hand, the one-class approach seems more realistic for applications in corporate settings due to practical reasons, for example, no need to retrain all existing models every time a new user is added/removed from the group, and one independent model for each user which allows to handle temporal changes in profiles on a per-user basis. 
% Thus, it is possible to speculate that a hybrid solution combining aspects from the multi-class and one-class approaches could be able to deal with practical needs and also reach accurate predictions. Performance could also be improved if using other relevant information for computer usage profiling (e.g., keystrokes and mouse dynamics) along with process and network activity.

% =======================================
% LIMITATIONS AND FUTURE WORK
% =======================================
\subsection{Limitations and Future Work}
\label{sec:limitations}

\mirelaehmuitoincrivel{@Luiz @Fabricio: this section is almost done; can you check the red font stuff here?}

% \ToDo{Limitation: sample was mainly college students from UF? Counterpoint: not atypical as several phishing user studies have similar hyper focused sample groups.}
% \ToDo{Limitation: collected during COVID, which has greatly changed how? users use the internet. Counterpoint: does this even matter? Is CEVERINO robust enough to adapt to different ``environments''?}
% \ToDo{Window size of 7+ days yields great results, but means this would be slow to catch an intruder.}

%Our study has four sets of limitations. We discuss actionable recommendation to address most of them in future research. \hl{The first set is related to our sample, which is small ($N = 17$) and not fully representative since all participants are young adults recruited in a particular metropolitan area, thus we do not know much about other age groups and regions. Moreover, our study was not conducted within a corporate environment as policies and rules make difficult to monitor activity in such places, so we used a home context (???). Yet, we attempted to simulate a corporate context in our experiments. These factors limit the generalizability of our findings. In future work, to bring more diversity to our sample, we plan to conduct data collection with a higher number of computer users from different age groups and places (cities or even countries). We also intend to focus on people who use computer for business activities (???)}. 

%One limitation of our study is the sample size, which is small ($N = 17$) and not fully representative of the general population since all participants are young adults from a large university. These factors limit the generalizability of our findings. Future studies with representative samples of a real corporate environment and teams are warranted.

The most glaring limitation of our study lies in our sample, which is small ($N = \samplesize$) and comprised mainly of young adults from a large university performing tasks on their personal computers; this is not representative of a large \commentario{corporate} setting. 
While a large university of nearly 50K students is a type of organizational environment, computer usage in corporations likely present different patterns of activity in terms of types of applications (often provided by the \commentario{corporation}) and websites (sometimes censored or limited) accessed, and times at which they are used. 
These factors thus limit the generalizability of our findings; nonetheless, our study's focus is on providing initial evidence of computer usage profiles in the context of concept drift, aware that future studies with representative samples of a real \commentario{corporate} setting and teams are warranted. 

%The second set of limitations refer to the integrity of the computer usage data that we recorded. We assumed that the users' systems were not compromised during the study period, but we did not monitor it as we collected data in an ecologically-valid setting. Presence of malware or any other malicious activities in the user's machine can adversely affect the learning models, as malicious behaviors would be considered part of the usage profile. In addition, although we debriefed all participants upon study completion to confirm that they did not share their computer while in study, some responses might not be accurate. For example, a participant may have forgotten about sharing the computer if this happened occasionally. Also, a participant who shared their password with others (e.g., relatives or friends) may have the computer used without their consent/knowledge.

Another limitation of our study concerns the integrity of the systems in which computer usage data was recorded: we assumed that the users' systems were not compromised by malware during the study period. 
Presence of malware could have adversely affected the learning models, as malicious behaviors would be considered part of the usage profile. 
In addition, although we debriefed all participants upon study completion to confirm that they did not share their computers during the study, some self-responses might not be accurate. 

Our feature engineering approach may also have been flawed, as the data representation that we used might not be robust over time because the lists of popular processes and websites that a user accesses change periodically.
%First, the determination of the most popular processes, websites, and country-level domains was time consuming, as well as the process of converting the recorded log files with the users' activities into such handcrafted features. Second, this representation of the data is not robust in the medium/long term because the popular processes and websites change over time. 
In future work, we plan to test automatic feature extractors able to provide more robust representations, which might be the case of TF-IDF~\cite{10.5555/553876}, Word2Vec~\cite{Mikolov2013EfficientEO} and BERT~\cite{DBLP:journals/corr/abs-1810-04805}, \ie 
considering users as documents in the context of information retrieval. %\todo[inline]{Will we include implementation details (algorithms used commented)?}
Additionally, due to the high number of processes \commentario{(100)} and websites \commentario{(454)} considered, and given that process and network activity varied among study participants, our approach was likely unable to reproduce patterns of computer usage observed, for example, for users working on the same project or belonging to the same teams in corporations, where it is common to use a standard set of software provided by the company. 
We believe that our approach was more suited to simulate computer usage activity in large or even different teams of \commentario{corporate} settings, where users are more likely to use different applications depending on their role. 
In future work, we plan to re-examine our dataset under different experimental conditions to investigate how restricting computer usage to common sets of processes and websites among users affects profile uniqueness and classification performance, thus gaining more understanding into how a CA tool would perform in different \commentario{corporate} scenarios.


Another set of limitations relate to our analysis of temporal consistency in computer usage profiles. 
First, our approaches exhibited a few limitations under real data since it could not to categorize two participants \commentario{(11.8\%)}. %in both Scenarios. 
In these cases, %the SOM suggested presence of concept drift over the weeks while the curves suggested absence of drift, so future research is necessary to investigate whether the former is more sensitive to drift than the latter. 
the SOM images suggested changes in the profiles while the curves suggested consistency, so future research is necessary to investigate whether the former is more sensitive to temporal behavior changes than the latter. 
Second, \commentario{we used a single learning model (one-class SVM) to compute the classification curves} \mirelaehmuitoincrivel{@Fabricio @Luiz: is this still true? If not, remove this and replace with: \textit{we found the best results when using window sizes of at least 7 days, which indicates that our approaches may be slow at catching an intruder.} 
}. 
For future work, we plan to assess other models in terms of accurate predictions and sensitivity to different levels of temporal changes. 
% Third, our approach relies on the visual inspection of the results, therefore needing different coders to address subjectivity issues. 
% Future work is advised to design metrics able to categorize type of temporal changes from SOM images and classification curves in a deterministic and automated fashion. 
Third, as shown in Figure~\ref{fig:drift_sensibility}, the categorization of drift is time-sensitive (the same user could be assigned different types of drift, depending on how much usage data was recorded from them), so our conclusions are limited to 8 weeks of data. 
We also collected data during the COVID-19 pandemic, which has greatly altered how users work, learn, socialize, and entertain themselves using their personal devices~\cite{Koeze2020-zm}; the yet unforeseeable changes to how our society may shift after the pandemic is resolved and how this may impact the user profiling analyses presented in this paper will require investigations from future work (\eg will there be more sparse personal computer usage as users return to work in offices and classrooms?). \ToDo{@Luiz or @Fabricio: can you check this sentence and make sure it... makes sense?}
Lastly, depending on the user's occupation, the usage profile can be consistent on different frequencies (\eg bi-weekly), thus for some participants what we may have detected were not real behavioral changes, but normal changes related to their usage pattern if observed over a period longer than one week. \mirelaehmuitoincrivel{@Fabricio: is this still true? Didn't you test several different window sizes?}
Therefore, future analysis with data collected over longer periods is warranted. %to allow investigation of temporal consistency not only weekly, but also biweekly and even monthly.


%Furthermore, depending on the user's occupation, the usage profile can reoccur on a basis other than weekly, thus we might not have detected real concept drifts for certain participants, but normal (benign) behavioral changes that may belong to a usage pattern if observed over a period longer than 1 week. Therefore, our conclusions are limited to our 3-weeks study period, and future analysis with longer periods of data collected is needed to allow investigation of temporal consistency not only weekly, but also biweekly and even monthly.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/new_version/drift_sensibility.pdf}
    \caption{Type of concept drift changing with the time.}
    \label{fig:drift_sensibility}
    \vspace{-1.5em}
\end{figure}

Finally, to evaluate the performance of our learning models, we only considered traditional metrics such as F-score and recall, which might not be ideal for CA systems~\cite{sugrim2019robust}. 
Future work is advised to consider more robust metrics, such as frequency count of scores along with receiver operating characteristics (ROC) curve, as discussed by Sugrim et al.~\cite{sugrim2019robust}.


We also identified some other opportunities for future research. 
% First, as \commentario{we found no evidence in this study that computer usage profiles are temporally consistent}, we plan to investigate online learning approaches for behavior-based CA in terms of feasibility, performance, and robustness against temporal changes in profiles. 
First, we intend to assess robustness against malicious activity (\eg insider attacks, APT, malware) by tampering real usage data with adversarial examples~\cite{christian2013DBLP}. 
Another aspect worth considering is the possibility of a user tampering with the classifier (\eg crafting noise to confuse the classifier and protect their privacy) or in malicious ways to disguise their actions.
% We also plan to extend our extractor to capture other information that can be useful for computer usage profiling, such as keystroke and mouse dynamics. 
Finally, we plan to test if including OS-based activity helps to increase profile uniqueness.



==> importante.tex <==
% sobre o classificador online

Talvez seja válido destacar que é necessário ter mais implementações para online learning, já que a gente teve que trocar as implementações até do multi-class e binary por conta disso. Mesmo se tratando de algo que possa tornar uma aplicação feasible, isso ainda é um problema na prática

% limitacoes

Outra coisa que tava pensando aqui é que, por usarmos uma janela de análise, talvez o conceito esteja em mudança e o classificador tenha dificuldade em detectar isso porque a janela vai gradualmente alterando isso com o tempo, sobretudo quando são janelas grandes, como 60 min. Talvez isso explique o resultado ruim de 60 min pro user 2, né?

==> tables/dns_info.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[h]
\centering
\caption{Example of a successful DNS session recording.}
\label{tab:dns_info}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}ccccc@{}}
\toprule
\textbf{PID} & \textbf{Event Time}      & \textbf{URL}    & \textbf{\begin{tabular}[c]{@{}c@{}}DNS Result\\for URL\end{tabular}}                                                                                                & \textbf{\begin{tabular}[c]{@{}c@{}}DNS Query\\Status\end{tabular}}                             \\ \midrule
1408        & \begin{tabular}[c]{@{}c@{}}09-23-2020\\18:23\end{tabular} & \url{sina.com.cn} & 35.51.247.37 & \begin{tabular}[c]{@{}c@{}}0\end{tabular}\\ \bottomrule
\end{tabular}%
}
\end{table}

% \begin{table}[h]
% \centering
% \caption{Example of DNS Session recording.}
% \label{tab:dns_info}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{@{}cccccc@{}}
% \toprule
% \textbf{PID} & \textbf{Event Time}                                        & \textbf{Executable Path}                               & \textbf{URL}    & \textbf{DNS Result for URL}                                                                                                & \textbf{DNS Query Status}                             \\ \midrule
% 11408        & \begin{tabular}[c]{@{}c@{}}09-23-2020\\ 18:23\end{tabular} & C:\textbackslash{}Application\textbackslash{}brave.exe & www.youtube.com & \begin{tabular}[c]{@{}c@{}}2607:f8b0:4002:c11::5b\\ 2607:f8b0:4002:c02::5b\\ 108.177.122.190\\ 108.177.122.93\end{tabular} & \begin{tabular}[c]{@{}c@{}}0\\ (Success)\end{tabular} \\ \bottomrule
% \end{tabular}%
% }
% \end{table}

==> tables/matrix_template.tex <==
\begin{table*}[ht]
\caption{Example of feature matrix, which contains temporal, process, and network features.}
\label{tab:matrix_template}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{6}{|c|}{Temporal features} & \multicolumn{7}{c|}{Process features} & \multicolumn{4}{c|}{Network features} \\ \hline
\begin{tabular}[c]{@{}c@{}}Minute\\ in day\end{tabular} & Sunday & ... & Saturday & Month & Day & \begin{tabular}[c]{@{}c@{}}Other\\ app\end{tabular} & \begin{tabular}[c]{@{}c@{}}Popular\\ app 1\end{tabular} & ... & \begin{tabular}[c]{@{}c@{}}Popular\\ app 99\end{tabular} & \begin{tabular}[c]{@{}c@{}}Popular\\ website 1\end{tabular} & ... & \begin{tabular}[c]{@{}c@{}}Popular\\ website 200\end{tabular} & \begin{tabular}[c]{@{}c@{}}Country level\\ domain 1\end{tabular} & ... & \begin{tabular}[c]{@{}c@{}}Country level\\ domain 253\end{tabular} & \begin{tabular}[c]{@{}c@{}}Other\\ website\end{tabular} \\ \hline
%0 & 0 & ... & 1 & 7 & 27 & 1 & 0 & ... & 0 & 0 & ... & 0 & 0 & ... & 0 & 0 \\
%... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
\begin{turn}{90}...\end{turn} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \begin{turn}{90}...\end{turn} \\ \hline
6 & 0 & ... & 1 & 7 & 27 & 3 & 1 & ... & 0 & 1 & ... & 1 & 1 & ... & 0 & 0 \\ \hline
\begin{turn}{90}...\end{turn} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \begin{turn}{90}...\end{turn} \\ \hline
%1436 & 0 & ... & 1 & 7 & 27 & 0 & 0 & ... & 1 & 1 & ... & 1 & 0 & ... & 0 & 2 \\
%... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
\end{tabular}
}
% \vspace{-3em}
\end{table*}

==> tables/process_info.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}

\begin{table}[ht]
\centering
\caption{Example of a recording log for process information.}
\label{tab:process_info}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}cccc@{}}
\toprule
\textbf{PID} & \textbf{Event Type} & \textbf{Executable Path}                                                                     & \textbf{Event Time}                                           \\ \midrule
1020         & Process Create      & C:\textbackslash{}...\textbackslash{}slack.exe & \begin{tabular}[c]{@{}c@{}}10-15-2020\\ 11:44:20\end{tabular} \\ \midrule
...          & ...                 & ...                                                                                          & ...                                                           \\ \midrule
1020         & Mouse               & C:\textbackslash{}...\textbackslash{}slack.exe & \begin{tabular}[c]{@{}c@{}}10-15-2020\\ 11:44:42\end{tabular} \\ \midrule
...          & ...                 & ...                                                                                          & ...                                                           \\ \midrule
1020         & Keyboard            & C:\textbackslash{}...\textbackslash{}slack.exe & \begin{tabular}[c]{@{}c@{}}10-15-2020\\ 11:45:27\end{tabular} \\ \bottomrule
\end{tabular}%
}
\end{table}



% \begin{table}[h]
% \centering
% \caption{Sample recording log showing a Slack process create event, followed by a mouse click and keyboard events in the same app.}
% \label{tab:process_info}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{@{}cccc@{}}
% \toprule
% \textbf{PID} & \textbf{Event Type} & \textbf{Executable Path}                                                                     & \textbf{Event Time}                                           \\ \midrule
% 1020         & Process Create      & C:\textbackslash{}..\textbackslash{}slack\textbackslash{}app-4.11.2\textbackslash{}slack.exe & \begin{tabular}[c]{@{}c@{}}10-15-2020\\ 11:44:20\end{tabular} \\ \midrule
% ...          & ...                 & ...                                                                                          & ...                                                           \\ \midrule
% 1020         & Mouse               & C:\textbackslash{}..\textbackslash{}slack\textbackslash{}app-4.11.2\textbackslash{}slack.exe & \begin{tabular}[c]{@{}c@{}}10-15-2020\\ 11:44:42\end{tabular} \\ \midrule
% ...          & ...                 & ...                                                                                          & ...                                                           \\ \midrule
% 1020         & Keyboard            & C:\textbackslash{}..\textbackslash{}slack\textbackslash{}app-4.11.2\textbackslash{}slack.exe & \begin{tabular}[c]{@{}c@{}}10-15-2020\\ 11:45:27\end{tabular} \\ \bottomrule
% \end{tabular}%
% }
% \end{table}

==> tables/profiles_period.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Period of the profiles in Condition 1 \& 2. N/A = Period not identified.}
\label{tab:period_profiles}
\resizebox{0.5\columnwidth}{!}{%
\begin{tabular}{@{}ccc@{}}
\toprule
\multirow{2}{*}{\textbf{User}}                                                         & \multicolumn{2}{c}{\textbf{Period (in hrs)}} \\ \cmidrule(l){2-3} 
                                                                                       & \textit{Condition 1}  & \textit{Condition 2} \\ \midrule
Remaining users & 24                    & 24                   \\
2  & N/A  & N/A \\
5  & 24   & 12  \\
8  & 89.6 & 7.6 \\
13 & 12   & N/A \\
19 & N/A  & 7.7 \\
30 & N/A  & 84  \\ \bottomrule
\end{tabular}%
}
\end{table}



% \begin{table}[]
% \centering
% \caption{\changed{Period of the profiles in Conditions 1 (with background activity) and 2 (without background activity).}}
% \label{tab:period_profiles}
% %\resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}ccc@{}}
% \toprule
% \multirow{2}{*}{\textbf{User}}     & \multicolumn{2}{c}{\textbf{Period}}                \\ \cmidrule(l){2-3} 
%                                   & \textbf{Condition 1}     & \textbf{Condition 2}    \\ \midrule
% 1*                                 & 24 hours                 & 24 hours                \\ \midrule
% u2                                  & Not identified                & Not identified               \\ \midrule
% 3--4*                             & 24 hours                 & 24 hours                \\ \midrule
% 5                                  & 24 hours                 & 12 hours                \\ \midrule
% 6--7*                             & 24 hours                 & 24 hours                \\ \midrule
% 8                                  & 89.6 hours               & 7.6 hours               \\ \midrule
% 9--12*                            & 24 hours                 & 24 hours                \\ \midrule
% 13                                 & 12 hours                 & Not identified               \\ \midrule
% 14--18*                           & 24 hours                 & 24 hours                \\ \midrule
% 19                                 & Not identified                & 7.7 hours               \\ \midrule
% 20--29*                           & 24 hours                 & 24 hours                \\ \midrule
% 30                                 & Not identified                & 84 hours                \\ \midrule
% 31*                                & 24 hours                 & 24 hours                \\ \midrule
% \multicolumn{3}{l}{* indicates user profiles with a same period in the two conditions.}
% \end{tabular}%
% %}
% \end{table}

==> tables/tab_network_record_sample.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{Example of network information recording.}
\label{tab:networkRecordSample}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccccccccc@{}}
\toprule
\multicolumn{9}{c}{\textbf{Connection Information}} &
   &
  \multicolumn{4}{c}{\textbf{Traffic Information}} \\ \cmidrule(r){1-9} \cmidrule(l){11-14} 
\textbf{PID} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Con.\\  hdl\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}IP \\ Prot.\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Local \\ IP addr \\ (hex)\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Local \\ port \\ \#\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Remote \\ IP addr \\ (hex)\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Remote \\ Port \#\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Con. \\ est. \\ time\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Con. \\ close \\ time\end{tabular}} &
  \textbf{} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Traffic\\ direct.\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Traffic\\ time\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Traffic\\ direct.\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Traffic\\ time\end{tabular}} \\ \midrule
\begin{tabular}[c]{@{}c@{}}3844\\ (Chrome)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}125-\\ 288\end{tabular} &
  V4 &
  \begin{tabular}[c]{@{}c@{}}10.255.\\ 48.22\end{tabular} &
  55321 &
  \begin{tabular}[c]{@{}c@{}}35.51.\\ 247.37\end{tabular} &
  443 &
  3:28 &
  3:30 &
   &
  0 &
  3:30 &
  1 &
  3:29 \\ \bottomrule
\end{tabular}%
}
\end{table*}


% \begin{table*}[t]
% \caption{Example of network information recording. %At 3:28 PM a new connection to 35.51.247.37 (sina.com.cn) was recorded. At 3:29 PM the extractor recorded traffic from the server to the user's machine and at 3:30 PM traffic from the user's machine to the server. The connection was closed at 3:30 PM.
% }
% \label{tab:networkRecordSample}
% \small
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multicolumn{9}{|c|}{Connection information} & \multicolumn{4}{c|}{Traffic information} \\ \hline
% PID & \begin{tabular}[c]{@{}c@{}}Con.\\  hdl\end{tabular} & \begin{tabular}[c]{@{}c@{}}IP \\ Prot.\end{tabular} & \begin{tabular}[c]{@{}c@{}}Local \\ IP addr \\ (hex)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Local \\ port \\ \#\end{tabular} & \begin{tabular}[c]{@{}c@{}}Remote \\ IP addr \\ (hex)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Remote \\ Port \#\end{tabular} & \begin{tabular}[c]{@{}c@{}}Con. \\ est. \\ time\end{tabular} & \begin{tabular}[c]{@{}c@{}}Con. \\ close \\ time\end{tabular} & \begin{tabular}[c]{@{}c@{}}Traffic\\ direct.\end{tabular} & \begin{tabular}[c]{@{}c@{}}Traffic\\ time\end{tabular} & \begin{tabular}[c]{@{}c@{}}Traffic\\ direct.\end{tabular} & \begin{tabular}[c]{@{}c@{}}Traffic\\ time\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}c@{}}3844\\ (Chrome)\end{tabular} & \begin{tabular}[c]{@{}c@{}}125-\\ 288\end{tabular} & V4 & \begin{tabular}[c]{@{}c@{}}10.255.\\ 48.22\end{tabular} & 55321 & \begin{tabular}[c]{@{}c@{}}35.51.\\ 247.37\end{tabular} & 443 & 3:28 & 3:30 & 0 & 3:30 & 1 & 3:29 \\ \hline
% \end{tabular}
% % \vspace{-2.75em}
% \end{table*}


==> tables/top_features.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\begin{longtable}[c]{@{}ccc@{}}
\caption{Top features by user.}
\label{tab:top-features}\\
\toprule
\textbf{Feature \#} & \textbf{User 1}                                        & \textbf{User 2}                            \\* \midrule
\endfirsthead
%
\endhead
%
\bottomrule
\endfoot
%
\endlastfoot
%
\textbf{1}         & mobile.pipe.aria.microsoft.com                         & ssl.gstatic.com                            \\
\textbf{2}         & login.microsoftonline.com                              & geo.prod.do.dsp.mp.microsoft.com           \\
\textbf{3}         & dm2306.storage.live.com                                & static-asm.secure.skypeassets.com          \\
\textbf{4}         & slack.com                                              & static.asm.skype.com                       \\
\textbf{5}         & tse3.mm.bing.net                                       & fpc.msedge.net                             \\
\textbf{6}         & roaming.officeapps.live.com                            & edge.skype.com                             \\
\textbf{7}         & assets.msn.com                                         & mail.google.com                            \\
\textbf{8}         & d27xxe7juh1us6.cloudfront.net                          & play.google.com                            \\
\textbf{9}         & contacts.google.com                                    & clients4.google.com                        \\
\textbf{10}        & img-s-msn-com.akamaized.net                            & browser.pipe.aria.microsoft.com            \\* \midrule
\textbf{Feature \#} & \textbf{User 3}                                        & \textbf{User 4}                            \\* \midrule
\textbf{1}         & mobile.pipe.aria.microsoft.com                         & v20.events.data.microsoft.com              \\
\textbf{2}         & presence.teams.microsoft.com                           & bl3301.storage.live.com                    \\
\textbf{3}         & d27xxe7juh1us6.cloudfront.net                          & outlook.office365.com                      \\
\textbf{4}         & chat-pa.clients6.google.com                            & edge.microsoft.com                         \\
\textbf{5}         & redirector.gvt1.com                                    & mobile.pipe.aria.microsoft.com             \\
\textbf{6}         & d29x207vrinatv.cloudfront.net                          & nleditor.osi.office.net                    \\
\textbf{7}         & teams.microsoft.com                                    & d27xxe7juh1us6.cloudfront.net              \\
\textbf{8}         & bolt.dropbox.com                                       & settings.data.microsoft.com                \\
\textbf{9}         & ping.citrix.com                                        & telemetry.dropbox.com                      \\
\textbf{10}        & www.gstatic.com                                        & android.clients.google.com                 \\* \midrule
\textbf{Feature \#} & \textbf{User 5}                                        & \textbf{User 6}                            \\* \midrule
\textbf{1}         & ncc.avast.com                                          & cloud.gastecnologia.com.br                 \\
\textbf{2}         & cdf505560e374ab9acea4cbc8dc632d9.fp.measure.office.com & 2.realtime.services.box.net                \\
\textbf{3}         & beacon.dropbox.com                                     & thunder.dropbox.com                        \\
\textbf{4}         & v20.events.data.microsoft.com                          & client.dropbox.com                         \\
\textbf{5}         & slack.com                                              & contacts.google.com                        \\
\textbf{6}         & platform-lookaside.fbsbx.com                           & d.dropbox.com                              \\
\textbf{7}         & gmail.com                                              & telemetry.dropbox.com                      \\
\textbf{8}         & outlook.office365.com                                  & www.msftconnecttest.com                    \\
\textbf{9}         & play.google.com                                        & feedbackws.icloud.com                      \\
\textbf{10}        & static.xx.fbcdn.net                                    & ssl.gstatic.com                            \\* \midrule
\textbf{Feature \#} & \textbf{User 7}                                        & \textbf{User 8}                            \\* \midrule
\textbf{1}         & osce120-en.fbs25.trendmicro.com                        & 4.bing.com                                 \\
\textbf{2}         & d27xxe7juh1us6.cloudfront.net                          & platform.bing.com                          \\
\textbf{3}         & osce120-sp1-en-b.trx.trendmicro.com                    & stats.g.doubleclick.net                    \\
\textbf{4}         & play.google.com                                        & content-autofill.googleapis.com            \\
\textbf{5}         & mobile.pipe.aria.microsoft.com                         & d27xxe7juh1us6.cloudfront.net              \\
\textbf{6}         & mail.google.com                                        & www.prolific.co                            \\
\textbf{7}         & calendar.google.com                                    & assets.msn.com                             \\
\textbf{8}         & clients6.google.com                                    & chrome                                     \\
\textbf{9}         & \_ldap.\_tcp.dc.\_msdcs.ad.ufl.edu.                       & array611.prod.do.dsp.mp.microsoft.com      \\
\textbf{10}        & self.events.data.microsoft.com                         & www.google.com                             \\* \midrule
\textbf{Feature \#} & \textbf{User 9}                                        & \textbf{User 10}                           \\* \midrule
\textbf{1}         & signaler-pa.clients6.google.com                        & browser.events.data.msn.com                \\
\textbf{2}         & ksn-file-geo.kaspersky-labs.com                        & bolt.dropbox.com                           \\
\textbf{3}         & v10.events.data.microsoft.com                          & telemetry.dropbox.com                      \\
\textbf{4}         & dc1-file.ksn.kaspersky-labs.com                        & ufl.instructure.com                        \\
\textbf{5}         & cdpcs.microsoft.com                                    & activity.windows.com                       \\
\textbf{6}         & 13.ucp-ntfy.kaspersky-labs.com                         & d.dropbox.com                              \\
\textbf{7}         & ksn-tcert-geo.kaspersky-labs.com                       & edge.microsoft.com                         \\
\textbf{8}         & android.clients.google.com                             & d27xxe7juh1us6.cloudfront.net              \\
\textbf{9}         & www.gmail.com                                          & checkappexec.microsoft.com                 \\
\textbf{10}        & clients1.google.com                                    & d.joinhoney.com                            \\* \midrule
\textbf{Feature \#} & \textbf{User 11}                                       & \textbf{User 12}                           \\* \midrule
\textbf{1}         & cloudflare-dns.com                                     & thunder.dropbox.com                        \\
\textbf{2}         & www.cloudflare.com                                     & substrate.office.com                       \\
\textbf{3}         & rum14.perf.linkedin.com                                & play.googleapis.com                        \\
\textbf{4}         & api.honeygain.com                                      & outlook.office365.com                      \\
\textbf{5}         & video-weaver.fra05.hls.ttvnw.net                       & mobile.pipe.aria.microsoft.com             \\
\textbf{6}         & update.avastbrowser.com                                & messages.google.com                        \\
\textbf{7}         & video-weaver.fra02.hls.ttvnw.net                       & telemetry.dropbox.com                      \\
\textbf{8}         & us10.freevpn.zone                                      & d.dropbox.com                              \\
\textbf{9}         & ieonlinews.microsoft.com                               & google.com                                 \\
\textbf{10}        & d27xxe7juh1us6.cloudfront.net                          & client-env.dropbox-dns.com                 \\* \midrule
\textbf{Feature \#} & \textbf{User 13}                                       & \textbf{User 14}                           \\* \midrule
\textbf{1}         & tconf2.cloud.360safe.com                               & datarouter.ol.epicgames.com                \\
\textbf{2}         & mmg-fna.whatsapp.net                                   & presence.teams.microsoft.com               \\
\textbf{3}         & us-atl.proxy.phantom.avira-vpn.com                     & aka.ms                                     \\
\textbf{4}         & cdn.content.prod.cms.msn.com                           & d27xxe7juh1us6.cloudfront.net              \\
\textbf{5}         & assets.msn.com                                         & self.events.data.microsoft.com             \\
\textbf{6}         & mobile.pipe.aria.microsoft.com                         & ufl.instructure.com                        \\
\textbf{7}         & play.google.com                                        & catalog.gamepass.com                       \\
\textbf{8}         & clientservices.googleapis.com                          & blitz-cdn.blitz.gg                         \\
\textbf{9}         & self.events.data.microsoft.com                         & go.microsoft.com                           \\
\textbf{10}        & d27xxe7juh1us6.cloudfront.net                          & telemetry.dropbox.com                      \\* \midrule
\textbf{Feature \#} & \textbf{User 15}                                       & \textbf{User 16}                           \\* \midrule
\textbf{1}         & ecs.office.com                                         & v10.events.data.microsoft.com              \\
\textbf{2}         & platform.bing.com                                      & d27xxe7juh1us6.cloudfront.net              \\
\textbf{3}         & www.google-analytics.com                               & play.google.com                            \\
\textbf{4}         & browser.pipe.aria.microsoft.com                        & mobile.pipe.aria.microsoft.com             \\
\textbf{5}         & update.googleapis.com                                  & v20.events.data.microsoft.com              \\
\textbf{6}         & d27xxe7juh1us6.cloudfront.net                          & settings.data.microsoft.com                \\
\textbf{7}         & ufl.instructure.com                                    & update.googleapis.com                      \\
\textbf{8}         & presence.teams.microsoft.com                           & login.microsoftonline.com                  \\
\textbf{9}         & login.microsoftonline.com                              & outlook.office365.com                      \\
\textbf{10}        & play.google.com                                        & redirector.gvt1.com                        \\* \midrule
\textbf{Feature \#} & \textbf{User 17}                                       & \textbf{User 18}                           \\* \midrule
\textbf{1}         & ws12.gti.mcafee.com                                    & hpnetworkcommunicatorcom                   \\
\textbf{2}         & self.events.data.microsoft.com                         & array805.prod.do.dsp.mp.microsoft.com      \\
\textbf{3}         & edge.microsoft.com                                     & background\_activity                        \\
\textbf{4}         & d27xxe7juh1us6.cloudfront.net                          & geo.prod.do.dsp.mp.microsoft.com           \\
\textbf{5}         & smartscreen-prod.microsoft.com                         & backgroundtaskhost                         \\
\textbf{6}         & ch3302.storage.live.com                                & www.yammer.com                             \\
\textbf{7}         & fbsbx.com                                              & runtimebroker                              \\
\textbf{8}         & update.googleapis.com                                  & settings.data.microsoft.com                \\
\textbf{9}         & blackboard.irsc.edu                                    & pipe.skype.com                             \\
\textbf{10}        & sadownload.mcafee.com                                  & d27xxe7juh1us6.cloudfront.net              \\* \midrule
\textbf{Feature \#} & \textbf{User 19}                                       & \textbf{User 20}                           \\* \midrule
\textbf{1}         & upload.analyzeme.net                                   & ksn-cinfo-geo.kaspersky-labs.com           \\
\textbf{2}         & aka.ms                                                 & v20.events.data.microsoft.com              \\
\textbf{3}         & ipv6detect.rmprod.zone                                 & ssl.bing.com                               \\
\textbf{4}         & smtp.gmail.com                                         & dc1.ksn.kaspersky-labs.com                 \\
\textbf{5}         & imap.gmail.com                                         & assets.msn.com                             \\
\textbf{6}         & ipv4detect.rmprod.zone                                 & uflorida.sharepoint.com                    \\
\textbf{7}         & http-intake.logs.datadoghq.com                         & api.onedrive.com                           \\
\textbf{8}         & catalog.gamepass.com                                   & ksn-crypto-wifiplus-geo.kaspersky-labs.com \\
\textbf{9}         & mobile.pipe.aria.microsoft.com                         & platform.bing.com                          \\
\textbf{10}        & chat-pa.clients6.google.com                            & ksn-stat-geo.kaspersky-labs.com            \\* \midrule
\textbf{Feature \#} & \textbf{User 21}                                       & \textbf{User 22}                           \\* \midrule
\textbf{1}         & addons-pa.clients6.google.com                          & presence.teams.microsoft.com               \\
\textbf{2}         & beacons.gcp.gvt2.com                                   & sn.webrootcloudav.com                      \\
\textbf{3}         & gcdn.2mdn.net                                          & snu.webrootcloudav.com                     \\
\textbf{4}         & mobile.pipe.aria.microsoft.com                         & skyversion.webrootcloudav.com              \\
\textbf{5}         & fundingchoicesmessages.google.com                      & r.bing.com                                 \\
\textbf{6}         & clients4.google.com                                    & beacons.gvt2.com                           \\
\textbf{7}         & clients2.google.com                                    & platform.bing.com                          \\
\textbf{8}         & fcmatch.google.com                                     & d27xxe7juh1us6.cloudfront.net              \\
\textbf{9}         & d27xxe7juh1us6.cloudfront.net                          & slack.com                                  \\
\textbf{10}        & oauthaccountmanager.googleapis.com                     & ssl.gstatic.com                            \\* \midrule
\textbf{Feature \#} & \textbf{User 23}                                       & \textbf{User 24}                           \\* \midrule
\textbf{1}         & scontent.cdninstagram.com                              & cc-api-behance.adobe.io                    \\
\textbf{2}         & cloud.gastecnologia.com.br                             & cc-api-data.adobe.io                       \\
\textbf{3}         & ssl.bing.com                                           & dev2.apps.ufl.edu                          \\
\textbf{4}         & platform.bing.com                                      & polka.typekit.com                          \\
\textbf{5}         & update.googleapis.com                                  & ping.citrix.com                            \\
\textbf{6}         & v10.events.data.microsoft.com                          & acp-ss-ue1.adobe.io                        \\
\textbf{7}         & redirector.gvt1.com                                    & notify.adobe.io                            \\
\textbf{8}         & dm2306files.storage.live.com                           & ocsp.pki.goog                              \\
\textbf{9}         & www.googleapis.com                                     & www.google-analytics.com                   \\
\textbf{10}        & array604.prod.do.dsp.mp.microsoft.com                  & api.onedrive.com                           \\* \midrule
\textbf{Feature \#} & \textbf{User 25}                                       & \textbf{User 26}                           \\* \midrule
\textbf{1}         & platform.bing.com                                      & aka.ms                                     \\
\textbf{2}         & ieonline.microsoft.com                                 & catalog.gamepass.com                       \\
\textbf{3}         & bing.com                                               & incoming.telemetry.mozilla.org             \\
\textbf{4}         & v10.events.data.microsoft.com                          & noahupdate.himsa.dk                        \\
\textbf{5}         & tile-service.weather.microsoft.com                     & self.events.data.microsoft.com             \\
\textbf{6}         & 9e77f29e93f64c0e8171ff52e41e0526.fp.measure.office.com & ocspx.digicert.com                         \\
\textbf{7}         & settings.data.microsoft.com                            & www.twitch.tv                              \\
\textbf{8}         & d27xxe7juh1us6.cloudfront.net                          & mobile.pipe.aria.microsoft.com             \\
\textbf{9}         & s.symcb.com                                            & ajax.googleapis.com                        \\
\textbf{10}        & mobile.pipe.aria.microsoft.com                         & spocs.getpocket.com                        \\* \midrule
\textbf{Feature \#} & \textbf{User 27}                                       & \textbf{User 28}                           \\* \midrule
\textbf{1}         & ocws.officeapps.live.com                               & background\_activity                        \\
\textbf{2}         & category.blocksite.co                                  & opera                                      \\
\textbf{3}         & www.onenote.com                                        & v10.events.data.microsoft.com              \\
\textbf{4}         & calendar.google.com                                    & mouse                                      \\
\textbf{5}         & datbooster.com                                         & ncc.avast.com                              \\
\textbf{6}         & www.google-analytics.com                               & d27xxe7juh1us6.cloudfront.net              \\
\textbf{7}         & googleads.g.doubleclick.net                            & keyboard                                   \\
\textbf{8}         & d27xxe7juh1us6.cloudfront.net                          & weather.opera-api.com                      \\
\textbf{9}         & uflorida.sharepoint.com                                & www.googletagservices.com                  \\
\textbf{10}        & play.google.com                                        & www.messenger.com                          \\* \midrule
\textbf{Feature \#} & \textbf{User 29}                                       & \textbf{User 30}                           \\* \midrule
\textbf{1}         & ocsp.pki.goog                                          & dns.google                                 \\
\textbf{2}         & mobile.pipe.aria.microsoft.com                         & update.googleapis.com                      \\
\textbf{3}         & fonts.googleapis.com                                   & datarouter.ol.epicgames.com                \\
\textbf{4}         & updatekeepalive.mcafee.com                             & clients2.google.com                        \\
\textbf{5}         & us.mcafee.com                                          & redirector.gvt1.com                        \\
\textbf{6}         & telemetry.dropbox.com                                  & cdn.content.prod.cms.msn.com               \\
\textbf{7}         & clients2.google.com                                    & d27xxe7juh1us6.cloudfront.net              \\
\textbf{8}         & docs.google.com                                        & settings.data.microsoft.com                \\
\textbf{9}         & d.dropbox.com                                          & assets.msn.com                             \\
\textbf{10}        & webadvisorc.rest.gti.mcafee.com                        & datarouter-prod.ak.epicgames.com           \\* \midrule
\textbf{Feature \#} & \textbf{User 31}                                       &                                            \\* \midrule
\textbf{1}         & browser.pipe.aria.microsoft.com                        &                                            \\
\textbf{2}         & presence.teams.microsoft.com                           &                                            \\
\textbf{3}         & sadownload.mcafee.com                                  &                                            \\
\textbf{4}         & d.docs.live.net                                        &                                            \\
\textbf{5}         & login.windows.net                                      &                                            \\
\textbf{6}         & d27xxe7juh1us6.cloudfront.net                          &                                            \\
\textbf{7}         & config.teams.microsoft.com                             &                                            \\
\textbf{8}         & d.dropbox.com                                          &                                            \\
\textbf{9}         & bolt.dropbox.com                                       &                                            \\
\textbf{10}        & teams.events.data.microsoft.com                        &                                            \\* \bottomrule
\end{longtable}



==> tables/usage_hours.tex <==
% -----------------------
% STATS ONLY TABLE
% -----------------------
\begin{table}[h] 
\centering
\caption{Summary of users' computer usage time.}
\label{tab:usage-hours}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccccc@{}}
\toprule
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}User \\ (De-Identified)\end{tabular}}} &
\multicolumn{5}{c}{\textbf{Statistics}} \\ 
\cmidrule(l){2-6} & 
% \multicolumn{1}{c}{} & 
% \multicolumn{1}{c}{} & 
\textit{Mean}   & \textit{Std}   & \textit{Min}   & \textit{Max}    & \textit{CV} \\ \toprule
1	& 17.77  & 5.00  & 9.53  & 27.40  & 28.16\%  \\ \midrule
2	& 11.43  & 27.97 & 1.05  & 80.65  & 244.64\% \\ \midrule
3	& 107.42 & 22.21 & 72.52 & 129.18 & 20.67\%  \\ \midrule
4	& 40.61  & 20.99 & 8.88  & 77.20  & 51.70\%  \\ \midrule
5	& 35.39  & 5.88  & 28.92 & 46.98  & 16.62\%  \\ \midrule
6	& 17.47  & 9.77  & 7.45  & 32.17  & 55.91\%  \\ \midrule
7	& 49.01  & 19.09 & 29.43 & 76.60  & 38.95\%  \\ \midrule
8	& 4.23   & 4.78  & 0.00  & 14.40  & 112.99\% \\ \midrule
9	& 47.37  & 3.84  & 38.30 & 50.45  & 8.10\%   \\ \midrule
10	& 21.98  & 6.48  & 15.25 & 36.47  & 29.47\%  \\ \midrule
11	& 31.85  & 17.56 & 15.80 & 59.02  & 55.13\%  \\ \midrule
12	& 25.40  & 34.90 & 0.00  & 82.15  & 137.43\% \\ \midrule
13	& 33.68  & 21.04 & 4.47  & 59.43  & 62.47\%  \\ \midrule
14	& 28.30  & 11.68 & 10.07 & 43.97  & 41.27\%  \\ \midrule
15	& 23.58  & 16.54 & 3.42  & 46.63  & 70.13\%  \\ \midrule
16	& 27.82  & 23.70 & 0.00  & 53.52  & 85.20\%  \\ \midrule
17	& 10.77  & 12.68 & 0.00  & 27.32  & 117.75\% \\ \midrule
18	& 3.93   & 2.39  & 0.35  & 7.90   & 60.90\%  \\ \midrule
19	& 76.62  & 49.73 & 14.20 & 152.33 & 64.90\%  \\ \midrule
20	& 41.04  & 16.00 & 19.97 & 61.87  & 38.98\%  \\ \midrule
21	& 8.23   & 7.63  & 0.00  & 20.57  & 92.71\%  \\ \midrule
22	& 31.26  & 27.82 & 0.00  & 63.08  & 88.99\%  \\ \midrule
23	& 30.79  & 11.71 & 14.00 & 52.10  & 38.03\%  \\ \midrule
24	& 76.30  & 14.36 & 56.52 & 95.60  & 18.82\%  \\ \midrule
25	& 11.06  & 4.39  & 4.57  & 16.12  & 39.69\%  \\ \midrule
26	& 34.24  & 7.38  & 18.00 & 40.75  & 21.54\%  \\ \midrule
27	& 52.07  & 13.29 & 25.47 & 67.88  & 25.53\%  \\ \midrule
28	& 53.93  & 9.11  & 39.15 & 64.58  & 16.90\%  \\ \bottomrule
\end{tabular}%
}
\end{table}



% -------------------------
% UPDATED FULL TABLE
% -------------------------
% \begin{table*}[ht] 
% \centering
% \caption{Computer users' computer usage time per study week.}
% \label{tab:usage-hours}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}ccccccccccccccc@{}}
% \toprule
% \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}User \\ (De-Identified)\end{tabular}}} &
% \multicolumn{8}{c}{\textbf{Weekly Usage Hours}} &
% \phantom{abc} &
% \multicolumn{5}{c}{\textbf{Statistics}} \\ 
% \cmidrule(l){2-9} \cmidrule(l){11-15} & 
% % \multicolumn{1}{c}{} & 
% % \multicolumn{1}{c}{} & 
% \textit{Week 1}  & \textit{Week 2}  & \textit{Week 3}  & \textit{Week 4} & \textit{Week 5}  & \textit{Week 6}  & \textit{Week 7}  & \textit{Week 8}  && \textit{Mean}   & \textit{Std}   & \textit{Min}   & \textit{Max}    & \textit{CV}       \\ 
%   \toprule
% 1               & 16.17  & 19.63  & 15.37  & 17.40 & 19.37  & 17.32  & 9.53   & 27.40  && 17.77  & 5.00  & 9.53  & 27.40  & 28.16\%  \\ \midrule
% 2               & 80.65  & 1.93   & 1.45   & 1.08  & 1.27   & 1.05   & 1.88   & 2.15   && 11.43  & 27.97 & 1.05  & 80.65  & 244.64\% \\ \midrule
% 3               & 72.52  & 112.08 & 129.18 & 74.80 & 106.45 & 125.35 & 125.02 & 113.98 && 107.42 & 22.21 & 72.52 & 129.18 & 20.67\%  \\ \midrule
% 4               & 51.10  & 32.47  & 38.27  & 77.20 & 39.88  & 8.88   & 21.97  & 55.08  && 40.61  & 20.99 & 8.88  & 77.20  & 51.70\%  \\ \midrule
% 5               & 34.37  & 28.92  & 35.45  & 30.98 & 46.98  & 37.98  & 38.43  & 29.98  && 35.39  & 5.88  & 28.92 & 46.98  & 16.62\%  \\ \midrule
% 6               & 10.22  & 32.17  & 7.85   & 25.42 & 17.65  & 11.30  & 7.45   & 27.72  && 17.47  & 9.77  & 7.45  & 32.17  & 55.91\%  \\ \midrule
% 7               & 72.83  & 76.60  & 35.53  & 36.85 & 64.20  & 33.25  & 43.42  & 29.43  && 49.01  & 19.09 & 29.43 & 76.60  & 38.95\%  \\ \midrule
% 8               & 6.67   & 1.57   & 14.40  & 5.52  & 1.87   & 3.80   & 0.00   & 0.00   && 4.23   & 4.78  & 0.00  & 14.40  & 112.99\% \\ \midrule
% 9               & 47.72  & 49.37  & 46.90  & 49.43 & 48.97  & 38.30  & 50.45  & 47.85  && 47.37  & 3.84  & 38.30 & 50.45  & 8.10\%   \\ \midrule
% 10              & 23.88  & 20.37  & 16.92  & 21.02 & 36.47  & 22.38  & 15.25  & 19.58  && 21.98  & 6.48  & 15.25 & 36.47  & 29.47\%  \\ \toprule
% 11              & 21.13  & 59.00  & 59.02  & 32.52 & 19.37  & 20.15  & 15.80  & 27.78  && 31.85  & 17.56 & 15.80 & 59.02  & 55.13\%  \\ \midrule
% 12              & 82.15  & 56.00  & 61.60  & 0.92  & 0.00   & 2.50   & 0.00   & 0.00   && 25.40  & 34.90 & 0.00  & 82.15  & 137.43\% \\ \midrule
% 13              & 37.82  & 44.12  & 55.37  & 42.98 & 15.08  & 4.47   & 59.43  & 10.17  && 33.68  & 21.04 & 4.47  & 59.43  & 62.47\%  \\ \midrule
% 14              & 42.28  & 43.97  & 27.77  & 21.78 & 35.77  & 19.87  & 10.07  & 24.88  && 28.30  & 11.68 & 10.07 & 43.97  & 41.27\%  \\ \midrule
% 15              & 10.27  & 45.17  & 22.83  & 46.63 & 15.25  & 33.95  & 11.12  & 3.42   && 23.58  & 16.54 & 3.42  & 46.63  & 70.13\%  \\ \midrule
% 16              & 41.20  & 29.72  & 50.62  & 53.52 & 45.98  & 1.52   & 0.00   & 0.00   && 27.82  & 23.70 & 0.00  & 53.52  & 85.20\%  \\ \midrule
% 17              & 9.32   & 27.32  & 23.23  & 26.08 & 0.20   & 0.00   & 0.00   & 0.00   && 10.77  & 12.68 & 0.00  & 27.32  & 117.75\% \\ \midrule
% 18              & 4.03   & 0.35   & 2.52   & 3.63  & 4.33   & 2.22   & 7.90   & 6.43   && 3.93   & 2.39  & 0.35  & 7.90   & 60.90\%  \\ \midrule
% 19              & 133.73 & 93.62  & 39.02  & 48.67 & 94.85  & 152.33 & 36.57  & 14.20  && 76.62  & 49.73 & 14.20 & 152.33 & 64.90\%  \\ \midrule
% 20              & 49.85  & 61.87  & 61.07  & 46.88 & 30.45  & 19.97  & 30.75  & 27.52  && 41.04  & 16.00 & 19.97 & 61.87  & 38.98\%  \\ \toprule
% 21              & 20.57  & 14.05  & 14.52  & 8.55  & 1.65   & 0.00   & 0.00   & 6.50   && 8.23   & 7.63  & 0.00  & 20.57  & 92.71\%  \\ \midrule
% 22              & 63.08  & 46.70  & 56.87  & 55.15 & 28.30  & 0.00   & 0.00   & 0.00   && 31.26  & 27.82 & 0.00  & 63.08  & 88.99\%  \\ \midrule
% 23              & 52.10  & 30.67  & 27.93  & 19.10 & 36.07  & 37.67  & 14.00  & 28.82  && 30.79  & 11.71 & 14.00 & 52.10  & 38.03\%  \\ \midrule
% 24              & 95.60  & 56.52  & 74.42  & 79.62 & 94.02  & 78.57  & 57.87  & 73.80  && 76.30  & 14.36 & 56.52 & 95.60  & 18.82\%  \\ \midrule
% 25              & 12.58  & 16.12  & 9.50   & 14.55 & 7.67   & 4.57   & 7.42   & 16.12  && 11.06  & 4.39  & 4.57  & 16.12  & 39.69\%  \\ \toprule
% 26              & 31.48  & 18.00  & 32.70  & 37.12 & 40.75  & 34.87  & 39.95  & 39.08  && 34.24  & 7.38  & 18.00 & 40.75  & 21.54\%  \\ \midrule
% 27              & 67.88  & 60.33  & 49.43  & 62.18 & 54.35  & 54.38  & 42.53  & 25.47  && 52.07  & 13.29 & 25.47 & 67.88  & 25.53\%  \\ \midrule
% 28              & 39.15  & 59.95  & 40.60  & 55.80 & 58.00  & 56.23  & 64.58  & 57.12  && 53.93  & 9.11  & 39.15 & 64.58  & 16.90\%  \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}



% -------------------------
% ORIGINAL TABLE
% -------------------------
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{multirow}
% % \usepackage{graphicx}
% \begin{table*}[ht]
% \centering
% %\caption{Computer users' employment status, field, and computer usage time per study week.}
% \caption{Computer users' computer usage time per study week.}
% \label{tab:usage-hours}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}cllccccccccccccc@{}}
% \toprule
% \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}User \\ (De-Identified)\end{tabular}}} &
%   \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Employment\\ Status\end{tabular}}}} &
%   \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Primary Type \\ of Field\end{tabular}}}} &
%   \multicolumn{8}{c}{\textbf{Weekly Usage Hours}} &
%   \multicolumn{5}{c}{\textbf{Statistics}} \\ \cmidrule(l){4-16} 
%   & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}     & week1  & week2  & week3  & week4 & week5  & week6  & week7  & week8  & Mean   & Std   & Min   & Max    & CV       \\ \midrule
% 1  & Unemployed           & Marketing                & 16.17  & 19.63  & 15.37  & 17.40 & 19.37  & 17.32  & 9.53   & 27.40  & 17.77  & 5.00  & 9.53  & 27.40  & 28.16\%  \\ \midrule
% 2  & Employed             & Insurance                & 80.65  & 1.93   & 1.45   & 1.08  & 1.27   & 1.05   & 1.88   & 2.15   & 11.43  & 27.97 & 1.05  & 80.65  & 244.64\% \\ \midrule
% 3  & Employed             & Research                 & 72.52  & 112.08 & 129.18 & 74.80 & 106.45 & 125.35 & 125.02 & 113.98 & 107.42 & 22.21 & 72.52 & 129.18 & 20.67\%  \\ \midrule
% 4  & Unemployed           & N/A                      & 51.10  & 32.47  & 38.27  & 77.20 & 39.88  & 8.88   & 21.97  & 55.08  & 40.61  & 20.99 & 8.88  & 77.20  & 51.70\%  \\ \midrule
% 5  & Employed             & Student                  & 34.37  & 28.92  & 35.45  & 30.98 & 46.98  & 37.98  & 38.43  & 29.98  & 35.39  & 5.88  & 28.92 & 46.98  & 16.62\%  \\ \midrule
% 6  & Employed             & Research                 & 10.22  & 32.17  & 7.85   & 25.42 & 17.65  & 11.30  & 7.45   & 27.72  & 17.47  & 9.77  & 7.45  & 32.17  & 55.91\%  \\ \midrule
% 7  & Employed             & Research                 & 72.83  & 76.60  & 35.53  & 36.85 & 64.20  & 33.25  & 43.42  & 29.43  & 49.01  & 19.09 & 29.43 & 76.60  & 38.95\%  \\ \midrule
% 8  & Unemployed           & N/A                      & 6.67   & 1.57   & 14.40  & 5.52  & 1.87   & 3.80   & 0.00   & 0.00   & 4.23   & 4.78  & 0.00  & 14.40  & 112.99\% \\ \midrule
% 9  & Employed             & Research and Educational & 47.72  & 49.37  & 46.90  & 49.43 & 48.97  & 38.30  & 50.45  & 47.85  & 47.37  & 3.84  & 38.30 & 50.45  & 8.10\%   \\ \midrule
% 10 & Unemployed           & Student                  & 23.88  & 20.37  & 16.92  & 21.02 & 36.47  & 22.38  & 15.25  & 19.58  & 21.98  & 6.48  & 15.25 & 36.47  & 29.47\%  \\ \midrule
% 11 & Employed             & Legal                    & 21.13  & 59.00  & 59.02  & 32.52 & 19.37  & 20.15  & 15.80  & 27.78  & 31.85  & 17.56 & 15.80 & 59.02  & 55.13\%  \\ \midrule
% 12 & Employed             & Computer technology      & 82.15  & 56.00  & 61.60  & 0.92  & 0.00   & 2.50   & 0.00   & 0.00   & 25.40  & 34.90 & 0.00  & 82.15  & 137.43\% \\ \midrule
% 13 & Employed             & Software Development     & 37.82  & 44.12  & 55.37  & 42.98 & 15.08  & 4.47   & 59.43  & 10.17  & 33.68  & 21.04 & 4.47  & 59.43  & 62.47\%  \\ \midrule
% 14 & Unemployed           & Studying                 & 42.28  & 43.97  & 27.77  & 21.78 & 35.77  & 19.87  & 10.07  & 24.88  & 28.30  & 11.68 & 10.07 & 43.97  & 41.27\%  \\ \midrule
% 15 & Unemployed           & N/A                      & 10.27  & 45.17  & 22.83  & 46.63 & 15.25  & 33.95  & 11.12  & 3.42   & 23.58  & 16.54 & 3.42  & 46.63  & 70.13\%  \\ \midrule
% 16 & Employed             & Design                   & 41.20  & 29.72  & 50.62  & 53.52 & 45.98  & 1.52   & 0.00   & 0.00   & 27.82  & 23.70 & 0.00  & 53.52  & 85.20\%  \\ \midrule
% 17 & Unemployed           & Administration           & 9.32   & 27.32  & 23.23  & 26.08 & 0.20   & 0.00   & 0.00   & 0.00   & 10.77  & 12.68 & 0.00  & 27.32  & 117.75\% \\ \midrule
% 18 & Unemployed           & Finance                  & 4.03   & 0.35   & 2.52   & 3.63  & 4.33   & 2.22   & 7.90   & 6.43   & 3.93   & 2.39  & 0.35  & 7.90   & 60.90\%  \\ \midrule
% 19 & Employed             & Cruise Entertainment     & 133.73 & 93.62  & 39.02  & 48.67 & 94.85  & 152.33 & 36.57  & 14.20  & 76.62  & 49.73 & 14.20 & 152.33 & 64.90\%  \\ \midrule
% 20 & Employed             & Chemistry                & 49.85  & 61.87  & 61.07  & 46.88 & 30.45  & 19.97  & 30.75  & 27.52  & 41.04  & 16.00 & 19.97 & 61.87  & 38.98\%  \\ \midrule
% 21 & Unemployed           & Student                  & 20.57  & 14.05  & 14.52  & 8.55  & 1.65   & 0.00   & 0.00   & 6.50   & 8.23   & 7.63  & 0.00  & 20.57  & 92.71\%  \\ \midrule
% 22 & Unemployed           & Education                & 63.08  & 46.70  & 56.87  & 55.15 & 28.30  & 0.00   & 0.00   & 0.00   & 31.26  & 27.82 & 0.00  & 63.08  & 88.99\%  \\ \midrule
% 23 & Unemployed           & Environmental Sciences   & 52.10  & 30.67  & 27.93  & 19.10 & 36.07  & 37.67  & 14.00  & 28.82  & 30.79  & 11.71 & 14.00 & 52.10  & 38.03\%  \\ \midrule
% 24 & Employed             & Customer service         & 95.60  & 56.52  & 74.42  & 79.62 & 94.02  & 78.57  & 57.87  & 73.80  & 76.30  & 14.36 & 56.52 & 95.60  & 18.82\%  \\ \midrule
% 25 & Unemployed           & Children cares           & 12.58  & 16.12  & 9.50   & 14.55 & 7.67   & 4.57   & 7.42   & 16.12  & 11.06  & 4.39  & 4.57  & 16.12  & 39.69\%  \\ \midrule
% 26 & Unemployed           & Food Service             & 31.48  & 18.00  & 32.70  & 37.12 & 40.75  & 34.87  & 39.95  & 39.08  & 34.24  & 7.38  & 18.00 & 40.75  & 21.54\%  \\ \midrule
% 27 & Employed             & Student                  & 67.88  & 60.33  & 49.43  & 62.18 & 54.35  & 54.38  & 42.53  & 25.47  & 52.07  & 13.29 & 25.47 & 67.88  & 25.53\%  \\ \midrule
% 28 & Employed             & Student assistant        & 39.15  & 59.95  & 40.60  & 55.80 & 58.00  & 56.23  & 64.58  & 57.12  & 53.93  & 9.11  & 39.15 & 64.58  & 16.90\%  \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}

==> tables/user_info.tex <==
\begin{table*}[]
\caption{Overview of active time over the 8-week study period per participant.
\centering 
}
\label{tab:user_info}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccccccc@{}}
% \begin{tabular}{|c|c|c|c|}
\toprule
\textbf{\begin{tabular}[c]{@{}c@{}}User \\ (De-Identified)\end{tabular}} &
  \multicolumn{8}{c}{\textbf{Weekly Usage Hours}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Total Active \\ Days\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Total Active \\ Hours\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Average \\ Hours/Day\end{tabular}} \\
  \cmidrule(l){2-9} &
  \textit{Week 1}  & \textit{Week 2}  & \textit{Week 3}  & \textit{Week 4} & \textit{Week 5}  & \textit{Week 6}  & \textit{Week 7}  & \textit{Week 8}
  \\ 
  \midrule
1  & 16.17  & 19.63  & 15.37  & 17.40 & 19.37  & 17.32  & 9.53   & 27.40 & 48 (86\%)  & 142 & 2.5  \\ \midrule
2  & 80.65  & 1.93   & 1.45   & 1.08  & 1.27   & 1.05   & 1.88   & 2.15 & 54 (96\%)  & 91  & 1.6  \\ \midrule
3  & 72.52  & 112.08 & 129.18 & 74.80 & 106.45 & 125.35 & 125.02 & 113.98  & 56 (100\%) & 859 & 15.3 \\ \midrule
4 & 51.10  & 32.47  & 38.27  & 77.20 & 39.88  & 8.88   & 21.97  & 55.08  & 56 (100\%) & 325 & 5.8  \\ \midrule
5  & 34.37  & 28.92  & 35.45  & 30.98 & 46.98  & 37.98  & 38.43  & 29.98 & 56 (100\%) & 283 & 5.1  \\ \midrule
6   & 10.22  & 32.17  & 7.85   & 25.42 & 17.65  & 11.30  & 7.45   & 27.72 & 37 (66\%)  & 140 & 2.5  \\ \midrule
7 & 72.83  & 76.60  & 35.53  & 36.85 & 64.20  & 33.25  & 43.42  & 29.43 & 53 (95\%)  & 392 & 7.0  \\ \midrule
8   & 6.67   & 1.57   & 14.40  & 5.52  & 1.87   & 3.80   & 0.00   & 0.00 & 29 (52\%)  & 34  & 0.6  \\ \midrule
9  & 47.72  & 49.37  & 46.90  & 49.43 & 48.97  & 38.30  & 50.45  & 47.85 & 56 (100\%) & 379 & 6.8  \\ \midrule
10 & 23.88  & 20.37  & 16.92  & 21.02 & 36.47  & 22.38  & 15.25  & 19.58 & 54 (96\%)  & 176 & 3.1  \\ \midrule
11 & 21.13  & 59.00  & 59.02  & 32.52 & 19.37  & 20.15  & 15.80  & 27.78 & 55 (98\%)  & 255 & 4.5  \\ \midrule
12  & 82.15  & 56.00  & 61.60  & 0.92  & 0.00   & 2.50   & 0.00   & 0.00 & 24 (43\%)  & 203 & 3.6  \\ \midrule
13 & 37.82  & 44.12  & 55.37  & 42.98 & 15.08  & 4.47   & 59.43  & 10.17 & 55 (98\%)  & 269 & 4.8  \\ \midrule
14 & 42.28  & 43.97  & 27.77  & 21.78 & 35.77  & 19.87  & 10.07  & 24.88 & 53 (95\%)  & 226 & 4.0  \\ \midrule
15  & 10.27  & 45.17  & 22.83  & 46.63 & 15.25  & 33.95  & 11.12  & 3.42 & 48 (86\%)  & 189 & 3.4  \\ \midrule
16  & 41.20  & 29.72  & 50.62  & 53.52 & 45.98  & 1.52   & 0.00   & 0.00 & 37 (66\%)  & 223 & 4.0  \\ \midrule
17 & 9.32   & 27.32  & 23.23  & 26.08 & 0.20   & 0.00   & 0.00   & 0.00 & 24 (43\%)  & 86  & 1.5  \\ \midrule
18 & 4.03   & 0.35   & 2.52   & 3.63  & 4.33   & 2.22   & 7.90   & 6.43 & 47 (84\%)  & 31  & 0.6  \\ \midrule
19  & 133.73 & 93.62  & 39.02  & 48.67 & 94.85  & 152.33 & 36.57  & 14.20 & 49 (88\%)  & 613 & 10.9 \\ \midrule
20 & 49.85  & 61.87  & 61.07  & 46.88 & 30.45  & 19.97  & 30.75  & 27.52 & 56 (100\%) & 328 & 5.9  \\ \midrule
21 & 20.57  & 14.05  & 14.52  & 8.55  & 1.65   & 0.00   & 0.00   & 6.50 & 34 (61\%)  & 66  & 1.2  \\ \midrule
22  & 63.08  & 46.70  & 56.87  & 55.15 & 28.30  & 0.00   & 0.00   & 0.00 & 31 (55\%)  & 250 & 4.5  \\ \midrule
23 & 52.10  & 30.67  & 27.93  & 19.10 & 36.07  & 37.67  & 14.00  & 28.82 & 50 (89\%)  & 246 & 4.4  \\ \midrule
24 & 95.60  & 56.52  & 74.42  & 79.62 & 94.02  & 78.57  & 57.87  & 73.80 & 56 (100\%) & 610 & 10.9 \\ \midrule
25 & 12.58  & 16.12  & 9.50   & 14.55 & 7.67   & 4.57   & 7.42   & 16.12 & 50 (89\%)  & 89  & 1.6  \\ \midrule
26  & 31.48  & 18.00  & 32.70  & 37.12 & 40.75  & 34.87  & 39.95  & 39.08 & 55 (98\%)  & 274 & 4.9  \\ \midrule
27 & 67.88  & 60.33  & 49.43  & 62.18 & 54.35  & 54.38  & 42.53  & 25.47 & 56 (100\%) & 417 & 7.4  \\ \midrule
28 & 39.15  & 59.95  & 40.60  & 55.80 & 58.00  & 56.23  & 64.58  & 57.12 & 56 (100\%) & 431 & 7.7  \\ \toprule 
  &&&&&&&& \textbf{Average} &
  \textbf{47.7 (85.2\%)} &
  \textbf{272} &
  \textbf{4.9} 
\end{tabular}%
}
\end{table*}



%\begin{table}[H]
% \caption{Overview of active time over the 8-week study period per participant. \ToDo{Make sure this table isn't being cut off in the final version of paper.}}
% \label{tab:user_info}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}cccc@{}}
% % \begin{tabular}{|c|c|c|c|}
% \toprule
% \textbf{\begin{tabular}[c]{@{}c@{}}User \\ (De-Identified)\end{tabular}} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}Total Active \\ Days\end{tabular}} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}Total Active \\ Hours\end{tabular}} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}Average \\ Hours/Day\end{tabular}} \\ \midrule
% 1  & 48 (86\%)  & 142 & 2.5  \\ \midrule
% 2  & 54 (96\%)  & 91  & 1.6  \\ \midrule
% 3  & 56 (100\%) & 859 & 15.3 \\ \midrule
% 4  & 56 (100\%) & 325 & 5.8  \\ \midrule
% 5  & 56 (100\%) & 283 & 5.1  \\ \midrule
% 6  & 37 (66\%)  & 140 & 2.5  \\ \midrule
% 7  & 53 (95\%)  & 392 & 7.0  \\ \midrule
% 8  & 29 (52\%)  & 34  & 0.6  \\ \midrule
% 9  & 56 (100\%) & 379 & 6.8  \\ \midrule
% 10 & 54 (96\%)  & 176 & 3.1  \\ \midrule
% 11 & 55 (98\%)  & 255 & 4.5  \\ \midrule
% 12 & 24 (43\%)  & 203 & 3.6  \\ \midrule
% 13 & 55 (98\%)  & 269 & 4.8  \\ \midrule
% 14 & 53 (95\%)  & 226 & 4.0  \\ \midrule
% 15 & 48 (86\%)  & 189 & 3.4  \\ \midrule
% 16 & 37 (66\%)  & 223 & 4.0  \\ \midrule
% 17 & 24 (43\%)  & 86  & 1.5  \\ \midrule
% 18 & 47 (84\%)  & 31  & 0.6  \\ \midrule
% 19 & 49 (88\%)  & 613 & 10.9 \\ \midrule
% 20 & 56 (100\%) & 328 & 5.9  \\ \midrule
% 21 & 34 (61\%)  & 66  & 1.2  \\ \midrule
% 22 & 31 (55\%)  & 250 & 4.5  \\ \midrule
% 23 & 50 (89\%)  & 246 & 4.4  \\ \midrule
% 24 & 56 (100\%) & 610 & 10.9 \\ \midrule
% 25 & 50 (89\%)  & 89  & 1.6  \\ \midrule
% 26 & 55 (98\%)  & 274 & 4.9  \\ \midrule
% 27 & 56 (100\%) & 417 & 7.4  \\ \midrule
% 28 & 56 (100\%) & 431 & 7.7  \\ \midrule
% \textbf{Average} &
%   \textbf{47.7 (85.2\%)} &
%   \textbf{272} &
%   \textbf{4.9} \\ \bottomrule
% \end{tabular}%
% }
% \end{table}

% ========================
% OUTDATED
% ========================
% \begin{table}[htb]
% \caption{Number of active days over the 21-day study period, total amount of usage hours, and data size collected per participant.\commentario{OUTDATED}}
% \label{tab:user_info}
% \centering
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|c|c|c|c|}
% \midrule
% \begin{tabular}[c]{@{}c@{}}User \\(De-identified)\end{tabular} & Active Days & \begin{tabular}[c]{@{}c@{}}Total Usage \\Hours\end{tabular} & \begin{tabular}[c]{@{}c@{}}Data Size \\(MB) \end{tabular} \\ \midrule
% 01 & 17 (81\%) & 235.8 & 1.24 \\ \midrule
% 02 & 11 (52.4\%) & 132.3 & 2.73 \\ \midrule
% 03 & 21 (100\%) & 448.1 & 2.59\\ \midrule
% 04 & 21 (100\%) & 420.9 & 0.17\\ \midrule
% 05 & 15 (71.4\%) & 175.3 & 3.96\\ \midrule
% 06 & 13 (61.9\%) & 122.2 & 1.27\\ \midrule
% 07 & 20 (95.2\%) & 179.4 & 1.43\\ \midrule
% 08 & 21 (100\%) & 370.3 & 4.91\\ \midrule
% 09 & 21 (100\%) & 374.2 & 0.44\\ \midrule
% 10 & 12 (57.1\%) & 154 & 0.48\\ \midrule
% 11 & 20 (95.2\%) & 424.8 & 2.38\\ \midrule
% 12 & 20 (95.2\%) & 400 & 0.22\\ \midrule
% 13 & 20 (95.2\%) & 386.4 & 1.71\\ \midrule
% 14 & 15 (71.4\%) & 176.3 & 0.83\\ \midrule
% 15 & 21 (100\%) & 416.7 & 8.03\\ \midrule
% 16 & 15 (71.4\%) & 139.9 & 1.24\\ \midrule
% 17 & 20 (95.2\%) & 382.8 & 3.95\\ \midrule
% Average & 17.8 (84.9\%) & 290.6 & 2.20\\ \midrule 
% \end{tabular}
% }
% \end{table}
